Isogeometric Analysis of Acoustic Scattering using Infinite Elements

Isogeometric analysis (IGA) has proven to be an improvement on the classical finite element method (FEM) in several fields, including structural mechanics and fluid dynamics. In this paper, the performance of IGA coupled with the infinite element method (IEM) for some acoustic scattering problems is investigated. In particular, the simple problem of acoustic scattering by a rigid sphere, and the scattering of acoustic waves by an elastic spherical shell with fluid domains both inside and outside, representing a full acoustic-structure interaction (ASI) problem. Finally, a mock shell and a simplified submarine benchmark are investigated. The numerical examples include comparisons between IGA and the FEM. Our main finding is that the usage of IGA significantly increases the accuracy compared to the usage of $C^0$ FEM due to increased inter-element continuity of the spline basis functions.

==> contents/NURBSgeometries.tex <==
%\newpage
\section{NURBS parametrization}
\subsection{Spherical shell}
\label{Sec2:NURBSdata}
A spherical shell with outer radius $R_0$ and inner radius $R_1$ may be represented by NURBS with knot vectors tabulated in \Cref{tab:sphericalShellKnotvectors} and control points tabulated in \Cref{tab:sphericalShellControlPoints}. The singularity points (of the mapping) is placed on the $z$-axis such that $\xi$ traverses around this $z$-axis.
\begin{table}
	\centering
	\caption{\textbf{Spherical shell}: Knot vectors.}
	\label{tab:sphericalShellKnotvectors}
	\begin{tabular}{l l l}
		\toprule
		Direction	& 	Order	& 	Knot vector\\
		\hline
		$\xi$		&	$\check{p}_\upxi=2$	&	$\Xi = \{0, 0, 0, 1, 1, 2, 2, 3, 3, 4, 4, 4\}$	\\
		$\eta$		&	$\check{p}_\upeta=2$	&	$\Eta = \{0, 0, 0, 1, 1, 2, 2, 2\}$					\\
		$\zeta$		&	$\check{p}_\upzeta=1$	&	$\Zeta = \{0, 0, 1, 1\}$						\\
		\bottomrule
	\end{tabular}
\end{table}
\begin{center}
\begin{longtable}{c c c c c c}
	\caption{\textbf{Spherical shell}: Control points and weights.}
	\label{tab:sphericalShellControlPoints}\\

\toprule $i$		& 	$j$	& 	$\vec{P}_{i,j,1}$ 	& 	$\vec{P}_{i,j,2}$ 		& 	$w_{i,j,1}$ & 	$w_{i,j,2}$ \\ \hline 
\endfirsthead
		\multicolumn{6}{c}%
		{{\textcolor{black}{\footnotesize \tablename\ \thetable{} -- continued from previous page}}} \\	
\toprule $i$		& 	$j$	& 	$\vec{P}_{i,j,1}$ 	& 	$\vec{P}_{i,j,2}$ 		& 	$w_{i,j,1}$ & 	$w_{i,j,2}$ \\ \hline 
\endhead

\hline \multicolumn{6}{r}{{Continued on next page}} \\
\endfoot

\hline
\endlastfoot
	$1$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$2$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$4$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$6$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$8$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$1$	&	$(0, 0, -R_1)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	
	$1$		&	$2$	&	$( R_1, 0  ,-R_1)$		&	$( R_0, 0  ,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$2$		&	$2$	&	$( R_1, R_1,-R_1)$		&	$( R_0, R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$3$		&	$2$	&	$( 0  , R_1,-R_1)$		&	$(-R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$4$		&	$2$	&	$(-R_1, R_1,-R_1)$		&	$( 0  , R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$5$		&	$2$	&	$(-R_1, 0  ,-R_1)$		&	$(-R_0, 0  ,-R_0)$		& $1/\sqrt{2}$	& $1/\sqrt{2}$	\\
	$6$		&	$2$	&	$(-R_1,-R_1,-R_1)$		&	$(-R_0,-R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$7$		&	$2$	&	$( 0  ,-R_1,-R_1)$		&	$( 0  ,-R_0,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$8$		&	$2$	&	$( R_1,-R_1,-R_1)$		&	$( R_0,-R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$9$		&	$2$	&	$( R_1, 0  ,-R_1)$		&	$( R_0, 0  ,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	
	$1$		&	$3$	&	$( R_1, 0  , 0)$		&	$( R_0, 0  , 0)$		& 1 			& 1				\\
	$2$		&	$3$	&	$( R_1, R_1, 0)$		&	$( R_0, R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$3$	&	$( 0  , R_1, 0)$		&	$( 0  , R_0, 0)$		& 1 			& 1				\\
	$4$		&	$3$	&	$(-R_1, R_1, 0)$		&	$(-R_0, R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$3$	&	$(-R_1, 0  , 0)$		&	$(-R_0, 0  , 0)$		& 1 			& 1				\\
	$6$		&	$3$	&	$(-R_1,-R_1, 0)$		&	$(-R_0,-R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$3$	&	$( 0  ,-R_1, 0)$		&	$( 0  ,-R_0, 0)$		& 1 			& 1				\\
	$8$		&	$3$	&	$( R_1,-R_1, 0)$		&	$( R_0,-R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$3$	&	$( R_1, 0  , 0)$		&	$( R_0, 0  , 0)$		& 1 			& 1				\\
	
	$1$		&	$4$	&	$( R_1, 0  , R_1)$		&	$( R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$2$		&	$4$	&	$( R_1, R_1, R_1)$		&	$( R_0, R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$3$		&	$4$	&	$( 0  , R_1, R_1)$		&	$( 0  , R_0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$4$		&	$4$	&	$(-R_1, R_1, R_1)$		&	$(-R_0, R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$5$		&	$4$	&	$(-R_1, 0  , R_1)$		&	$(-R_0, 0  , R_0)$		& $1/\sqrt{2}$	& $1/\sqrt{2}$	\\
	$6$		&	$4$	&	$(-R_1,-R_1, R_1)$		&	$(-R_0,-R_0, R_0)$  		& $1/2$ 		& $1/2$ 		\\
	$7$		&	$4$	&	$( 0  ,-R_1, R_1)$		&	$( 0  ,-R_0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$8$		&	$4$	&	$( R_1,-R_1, R_1)$		&	$( R_0,-R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$9$		&	$4$	&	$( R_1, 0  , R_1)$		&	$( R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	
	$1$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$2$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$ 		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$4$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$6$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$8$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$5$	&	$(0, 0, R_1)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
\end{longtable}
\end{center}

\subsection{Sphere}
\label{Sec2:NURBSdataSphere}
A sphere with radius $R_0$ may be represented by NURBS with knot vectors tabulated in \Cref{tab:sphereKnotvectors} and control points tabulated in \Cref{tab:sphereControlPoints}. The singularity points (of the mapping) is again placed on the $z$-axis such that $\xi$ traverses around this $z$-axis.
\begin{table}
	\centering
	\caption{\textbf{Sphere}: Knot vectors.}
	\label{tab:sphereKnotvectors}
	\begin{tabular}{l l l}
		\toprule
		Direction	& 	Order	& 	Knot vector\\
		\hline
		$\xi$		&	$\check{p}_\upxi=2$	&	$\Xi = \{0, 0, 0, 1, 1, 2, 2, 3, 3, 4, 4, 4\}$	\\
		$\eta$		&	$\check{p}_\upeta=2$	&	$\Eta = \{0, 0, 0, 1, 1, 2, 2, 2\}$					\\
		$\zeta$		&	$\check{p}_\upzeta=1$	&	$\Zeta = \{0, 0, 1, 1\}$						\\
		\bottomrule
	\end{tabular}
\end{table}
\begin{center}
\begin{longtable}{c c c c c c}
	\caption{\textbf{Sphere}: Control points and weights.}
	\label{tab:sphereControlPoints}\\

\toprule $i$		& 	$j$	& 	$\vec{P}_{i,j,1}$ 	& 	$\vec{P}_{i,j,2}$ 		& 	$w_{i,j,1}$ & 	$w_{i,j,2}$ \\ \hline 
\endfirsthead
		\multicolumn{6}{c}%
		{{\textcolor{black}{\footnotesize \tablename\ \thetable{} -- continued from previous page}}} \\	
\toprule $i$		& 	$j$	& 	$\vec{P}_{i,j,1}$ 	& 	$\vec{P}_{i,j,2}$ 		& 	$w_{i,j,1}$ & 	$w_{i,j,2}$ \\ \hline 
\endhead

\hline \multicolumn{6}{r}{{Continued on next page}} \\
\endfoot

\hline
\endlastfoot
	$1$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$2$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$4$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$6$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	$8$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$1$	&	$(0, 0, 0)$		&	$(0, 0, -R_0)$		& 1 			& 1				\\
	
	$1$		&	$2$	&	$(0, 0, 0)$		&	$( R_0, 0  ,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$2$		&	$2$	&	$(0, 0, 0)$		&	$( R_0, R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$3$		&	$2$	&	$(0, 0, 0)$		&	$(-R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$4$		&	$2$	&	$(0, 0, 0)$		&	$( 0  , R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$5$		&	$2$	&	$(0, 0, 0)$		&	$(-R_0, 0  ,-R_0)$		& $1/\sqrt{2}$	& $1/\sqrt{2}$	\\
	$6$		&	$2$	&	$(0, 0, 0)$		&	$(-R_0,-R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$7$		&	$2$	&	$(0, 0, 0)$		&	$( 0  ,-R_0,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$8$		&	$2$	&	$(0, 0, 0)$		&	$( R_0,-R_0,-R_0)$		& $1/2$ 		& $1/2$ 		\\
	$9$		&	$2$	&	$(0, 0, 0)$		&	$( R_0, 0  ,-R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	
	$1$		&	$3$	&	$(0, 0, 0)$		&	$( R_0, 0  , 0)$		& 1 			& 1				\\
	$2$		&	$3$	&	$(0, 0, 0)$		&	$( R_0, R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$3$	&	$(0, 0, 0)$		&	$( 0  , R_0, 0)$		& 1 			& 1				\\
	$4$		&	$3$	&	$(0, 0, 0)$		&	$(-R_0, R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$3$	&	$(0, 0, 0)$		&	$(-R_0, 0  , 0)$		& 1 			& 1				\\
	$6$		&	$3$	&	$(0, 0, 0)$		&	$(-R_0,-R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$3$	&	$(0, 0, 0)$		&	$( 0  ,-R_0, 0)$		& 1 			& 1				\\
	$8$		&	$3$	&	$(0, 0, 0)$		&	$( R_0,-R_0, 0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$3$	&	$(0, 0, 0)$		&	$( R_0, 0  , 0)$		& 1 			& 1				\\
	
	$1$		&	$4$	&	$(0, 0, 0)$		&	$( R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$2$		&	$4$	&	$(0, 0, 0)$		&	$( R_0, R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$3$		&	$4$	&	$(0, 0, 0)$		&	$( 0  , R_0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$4$		&	$4$	&	$(0, 0, 0)$		&	$(-R_0, R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$5$		&	$4$	&	$(0, 0, 0)$		&	$(-R_0, 0  , R_0)$		& $1/\sqrt{2}$	& $1/\sqrt{2}$	\\
	$6$		&	$4$	&	$(0, 0, 0)$		&	$(-R_0,-R_0, R_0)$  		& $1/2$ 		& $1/2$ 		\\
	$7$		&	$4$	&	$(0, 0, 0)$		&	$( 0  ,-R_0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	$8$		&	$4$	&	$(0, 0, 0)$		&	$( R_0,-R_0, R_0)$		& $1/2$ 		& $1/2$ 		\\
	$9$		&	$4$	&	$(0, 0, 0)$		&	$( R_0, 0  , R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$	\\
	
	$1$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$2$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$ 		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$3$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$4$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$5$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$6$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$7$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
	$8$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& $1/\sqrt{2}$ 	& $1/\sqrt{2}$ 	\\
	$9$		&	$5$	&	$(0, 0, 0)$		&	$(0, 0, R_0)$		& 1 			& 1				\\
\end{longtable}
\end{center}
%\thispagestyle{empty}

==> contents/analyticSolution.tex <==
\section{Analytic solution for spherical shell}
\label{Sec2:analyticSolution}
There are few known analytic solution to full 3D scattering problems, but for the spherical shell, the exact solution is known (the exact solution is also known for a solid sphere, but this case will not be considered). Whenever the spherical shell is analyzed, we shall mainly use the parameters found in \Cref{Tab2:sphericalShellParameters}. It is typically also possible to construct analytic solution to an in homogeneous Helmholtz equation by inserting an arbitrary smooth solution and calculate the resulting right hand side. Correspondingly for elasticity problems with body forces. However, for the homogeneous equations one does not have this liberty. Elastic scattering on a spherical shell thus serves as a valuable test problem before geometries with higher complexity may be analyzed.
\begin{table}
	\centering
	\caption[Parameters for spherical shell]{Parameters for spherical shell.}
	\label{Tab2:sphericalShellParameters}
	\begin{tabular}{l l}
		\toprule
		Parameter & Description\\
		\midrule
		$E = 2.07\cdot 10^{11}\unit{Pa}$ & Young's modulus\\
		$\rho_s = 7669\unit{kg/m^3}$ & Density of solid\\
		$\rho_{\mathrm{f}} = 1000\unit{kg/m^3}$ & Density of fluid\\
		$\nu = 0.3$ & Poisson's ratio\\
		$c_{\mathrm{f}} = 1524\unit{m/s}$ & Fluid speed of sound\\
		$t = 0.15\unit{m}$ & Thickness of the shell\\
		$R = 5\unit{m}$ & Radius of the midsurface of the shell\\
		$R_0 = 5.075\unit{m}$ & Outer radius of the shell\\
		$P_0 = 1$ & Amplitude of incident wave\\
		\bottomrule
	\end{tabular}
\end{table}

\subsection{Fundamental functions}
Exact solutions for the spherical shell are heavily based on the spherical coordinate system defined in \Cref{Sec2:sphericalCoordinates}. Some fundamental functions then naturally arise, and we shall briefly present their notation in the following.

As the \textit{Bessel functions} (or \textit{cylindrical harmonics}) are implemented in MATLAB, we shall use these functions as a starting point. 

\subsubsection{Legendre polynomials}
The Legendre polynomials are defined recursively by (cf.~\cite[p. 332]{Abramovitz1964ham})
\begin{equation*}
	(n+1)P_{n+1}(x)=(2n+1)xP_n(x)-nP_{n-1}(x)
\end{equation*}
starting with $P_0(x) = 1$ and $P_1(x) = x$. The first five of these two sets of functions are illustrated in \Cref{Fig2:legendrePolynomials}. The solutions presented involving these functions appears as $P_n(\cos\vartheta)$, so we also plot these functions in \Cref{Fig2:legendrePolynomials2}.
\tikzsetnextfilename{legendrePolynomials}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			legend style={
				at={(0.97,0.03)},
				anchor=south east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$x$,
			ylabel=$P_n$,
%			ymax=19,
			ymin=-1.4,	
			ymax=1.4,		
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n0.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n1.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n2.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n3.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n4.dat};
			\addlegendentry{$P_0$}
			\addlegendentry{$P_1$}
			\addlegendentry{$P_2$}
			\addlegendentry{$P_3$}
			\addlegendentry{$P_4$}
		\end{axis}
	\end{tikzpicture}
	\caption[Legendre polynomials]{\textbf{Legendre polynomials}: The first 5 Legendre polynomials $P_n(x)$.}
\label{Fig2:legendrePolynomials}
\vspace{2cm}
	\tikzsetnextfilename{legendrePolynomials2}
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			legend style={
				at={(0.03,0.03)},
				anchor=south west
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$\vartheta$,
			ylabel=$P_n(\cos\vartheta)$,
%			ymax=19,
%			ymin=-4,		
			ymin=-1.4,	
			ymax=1.4,	
		    xtick={0,0.785398163397448, 1.570796326794897,2.356194490192345, 3.141592653589793},
		    xticklabels={$0$,$\frac{\pi}{4}$,$\frac{\pi}{2}$,$\frac{3\pi}{4}$,$\pi$},
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n0_cosTheta.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n1_cosTheta.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n2_cosTheta.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n3_cosTheta.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/legendre_n4_cosTheta.dat};
			\addlegendentry{$P_0(\cos\vartheta)$}
			\addlegendentry{$P_1(\cos\vartheta)$}
			\addlegendentry{$P_2(\cos\vartheta)$}
			\addlegendentry{$P_3(\cos\vartheta)$}
			\addlegendentry{$P_4(\cos\vartheta)$}
		\end{axis}
	\end{tikzpicture}
	\caption[Legendre polynomials as a function of the polar angle]{\textbf{Legendre polynomials}: The first 5 Legendre polynomials $P_n$ evaluated at $\cos\vartheta$ for $\vartheta\in[0, \pi]$.}
\label{Fig2:legendrePolynomials2}
\end{figure}

\subsubsection{Bessel functions}
The Bessel functions of the first kind are defined by
\begin{equation*}
	J_\alpha(x) = \sum_{m=0}^\infty \frac{(-1)^m}{m! \Gamma(m+\alpha+1)}\left(\frac{x}{2}\right)^{2m+\alpha},
\end{equation*}
while the Bessel functions of the second kind are defined by
\begin{equation*}
	Y_\alpha(x) = \frac{J_\alpha \cos(\alpha\pi)-J_{-\alpha}(x)}{\sin(\alpha\pi)},
\end{equation*}
where
\begin{equation*}
	Y_n(x) = \lim_{\alpha\to n} Y_\alpha(x)
\end{equation*}
whenever $n\in\Z$ (cf.~\cite[p. 358]{Abramovitz1964ham}). The derivatives of these functions are given by
\begin{equation*}
	J_\alpha'(x) = \begin{cases}
		\frac{1}{2}\left(J_{\alpha-1}-J_{\alpha+1}\right)\quad&\alpha\neq 0\\
		-J_1(x) \quad &\alpha=0
	\end{cases}
\end{equation*}
and
\begin{equation*}
	Y_\alpha'(x) = \begin{cases}
		\frac{1}{2}\left(Y_{\alpha-1}-Y_{\alpha+1}\right)\quad&\alpha\neq 0\\
		-Y_1(x) \quad &\alpha=0.
	\end{cases}
\end{equation*}
The first five functions of these two sets of functions are illustrated in \Cref{Fig2:besselFunctions1} and \Cref{Fig2:besselFunctions2}, respectively.
\tikzsetnextfilename{besselFunctions1}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$x$,
			ylabel=$J_n$,
			ymin=-0.55,	
			ymax=1.15,	
%			ymax=19,
%			ymin=-1,		
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel1_n0.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel1_n1.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel1_n2.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel1_n3.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel1_n4.dat};
			\addlegendentry{$J_0$}
			\addlegendentry{$J_1$}
			\addlegendentry{$J_2$}
			\addlegendentry{$J_3$}
			\addlegendentry{$J_4$}
		\end{axis}
	\end{tikzpicture}
	\caption[Bessel function of first kind]{\textbf{Bessel function of first kind}: The first 5 Bessel functions of first kind $J_n(x)$.}
\label{Fig2:besselFunctions1}
\vspace{2cm}
	\tikzsetnextfilename{besselFunctions2}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			%width=0.45*350pt,
			%height=0.5*250pt,
			legend style={
				at={(0.97,0.03)},
				anchor=south east
			},
			xlabel=$x$,
			ylabel=$Y_n$,
			ymax=0.6,
			ymin=-1,	
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel2_n0.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel2_n1.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel2_n2.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel2_n3.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/bessel2_n4.dat};
			\addlegendentry{$Y_0$}
			\addlegendentry{$Y_1$}
			\addlegendentry{$Y_2$}
			\addlegendentry{$Y_3$}
			\addlegendentry{$Y_4$}
		\end{axis}
	\end{tikzpicture}
	\caption[Bessel function of second kind]{\textbf{Bessel function of second kind}: The first 5 Bessel functions of second kind $Y_n(x)$.}
\label{Fig2:besselFunctions2}
\end{figure}

We may now use these definitions to define the \textit{spherical Bessel functions}. The spherical Bessel functions of the first kind are defined by (cf.~\cite[p. 437]{Abramovitz1964ham})
\begin{equation*}
	j_n(x) = \sqrt{\frac{\pi}{2x}}J_{n+\frac{1}{2}}(x)
\end{equation*}
and the second kind are defined by
\begin{equation*}
	y_n(x) = \sqrt{\frac{\pi}{2x}}Y_{n+\frac{1}{2}}(x).
\end{equation*}
The first five functions of these two sets of functions are illustrated in \Cref{Fig2:sphericalBesselFunctions1} and \Cref{Fig2:sphericalBesselFunctions2}. The derivatives of these functions are simply found by the product rule
\begin{equation*}
	j_n'(x) = \sqrt{\frac{\pi}{2x}}J_{n+\frac{1}{2}}'(x) -\frac{1}{2} \sqrt{\frac{\pi}{2}}\frac{1}{x^{3/2}}J_{n+\frac{1}{2}}(x)
\end{equation*}
and
\begin{equation*}
	y_n'(x) = \sqrt{\frac{\pi}{2x}}Y_{n+\frac{1}{2}}'(x) -\frac{1}{2} \sqrt{\frac{\pi}{2}}\frac{1}{x^{3/2}}Y_{n+\frac{1}{2}}(x).
\end{equation*}

\tikzsetnextfilename{sphericalBesselFunctions1}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$x$,
			ylabel=$j_n$,
%			ymax=19,
%			ymin=-1,	
			ymin=-0.55,	
			ymax=1.15,		
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel1_n0.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel1_n1.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel1_n2.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel1_n3.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel1_n4.dat};
			\addlegendentry{$j_0$}
			\addlegendentry{$j_1$}
			\addlegendentry{$j_2$}
			\addlegendentry{$j_3$}
			\addlegendentry{$j_4$}
		\end{axis}
	\end{tikzpicture}
	\caption[Spherical Bessel function of first kind]{\textbf{Spherical Bessel function of first kind}: The first 5 Spherical Bessel functions of first kind $j_n(x)$.}
\label{Fig2:sphericalBesselFunctions1}
\vspace{2cm}
	\tikzsetnextfilename{sphericalBesselFunctions2}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			%width=0.45*350pt,
			%height=0.5*250pt,
			legend style={
				at={(0.97,0.03)},
				anchor=south east
			},
			xlabel=$x$,
			ylabel=$y_n$,
			ymax=0.6,
			ymin=-1,	
%			xmin = 0.2,
%			xmax = 0.72
			]
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel2_n0.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel2_n1.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel2_n2.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel2_n3.dat};
			\addplot table[x=x,y=y] {../../data/plotData/fundamentalFunctions/sphericalBessel2_n4.dat};
			\addlegendentry{$y_0$}
			\addlegendentry{$y_1$}
			\addlegendentry{$y_2$}
			\addlegendentry{$y_3$}
			\addlegendentry{$y_4$}
		\end{axis}
	\end{tikzpicture}
	\caption[Spherical Bessel function of second kind]{\textbf{Spherical Bessel function of second kind}: The first 5 Spherical Bessel function of second kind $y_n(x)$.}
\label{Fig2:sphericalBesselFunctions2}
\end{figure}

\subsubsection{Spherical Hankel functions}
The spherical Hankel functions of the first kind are now given by
\begin{equation*}
	h_n(x) = j_n(x) +  \imag y_n(x)
\end{equation*}
with a derivative given by
\begin{equation*}
	h_n'(x) = j_n'(x) +  \imag y_n'(x).
\end{equation*}
The spherical Hankel functions of the second kind are simply defined by
\begin{equation*}
	h_n^{(2)}(x) = j_n(x) -  \imag y_n(x).
\end{equation*}
As these solution will represent in-going waves in scattering problems, they will not be used (They will be eliminated by the Sommerfield condition, which we will come back to).

\subsection{Simplifying notations}
In~\cite[pp. 12-20]{Chang1994voa} the exact 3D elasticity solution for the spherical shell is presented. We shall repeat the final formulas here, but will adopt them to the notation of the thesis and do some simplifications in the expressions. As the formulas involved are quite comprehensive, we shall start by defining some simplifying notation. For convenience, we define
\begin{equation*}
	Z_{n}^{(1)}(x) = j_n(x),\quad\text{and}\quad Z_{n}^{(2)}(x) = y_n(x),
\end{equation*}
such that we can define
\begin{align*}
	U_1^{(i)}(x) &= nZ_n^{(i)}(x)-xZ_{n+1}^{(i)}(x)\\
	U_3^{(i)}(x) &= n(n+1)Z_n^{(i)}(x)\\
	T_{11}^{(i)}(x) &= \left[n^2-n-\frac{1}{2}\left(\frac{\beta}{\alpha}\right)^2 x^2\right] Z_n^{(i)}(x) + 2xZ_{n+1}^{(i)}(x)\\
	T_{13}^{(i)}(x) &= n(n+1)\left[(n-1)Z_n^{(i)}(x) - xZ_{n+1}^{(i)}(x)\right]\\
	T_{21}^{(i)}(x) &= \left[-n^2-\frac{1}{2}\left(\frac{\beta}{\alpha}\right)^2 x^2+x^2\right] Z_n^{(i)}(x) - xZ_{n+1}^{(i)}(x)\\
	T_{23}^{(i)}(x) &= -(n^2+n)\left[n Z_n^{(i)}(x) - xZ_{n+1}^{(i)}(x)\right] \\
	T_{31}^{(i)}(x) &= \left[n-\frac{1}{2}x^2+\left(\frac{\alpha}{\beta}\right)^2 x^2\right] Z_n^{(i)}\left(\frac{\alpha}{\beta}x\right) - \frac{\alpha}{\beta}x Z_{n+1}^{(i)}\left(\frac{\alpha}{\beta}x\right)\\
	T_{33}^{(i)}(x) &= n(n+1)Z_n^{(i)}(x)\\
	T_{41}^{(i)}(x) &= (n-1) Z_n^{(i)}(x) - xZ_{n+1}^{(i)}(x)\\
	T_{43}^{(i)}(x) &= \left(n^2-1-\frac{1}{2}x^2\right) Z_n^{(i)}(x) + xZ_{n+1}^{(i)}(x)
\end{align*}
where
\begin{equation*}
	\alpha=\frac{\omega}{c_1},\quad \beta=\frac{\omega}{c_2},\quad c_1 = \sqrt{\frac{\lambda+2\mu}{\rho_s}},\quad c_2 = \sqrt{\frac{\mu}{\rho_s}}.
\end{equation*}
Moreover, we define the coefficients $A_n$, $B_n$, $C_n$ and $D_n$ by
\begin{equation*}
	A_0 = \frac{\frac{R_0^2}{2\mu}T_{11}^{(2)}(\alpha R_1)}{\nabla^2_0},\quad B_0=0,\quad
	C_0 = -\frac{\frac{R_0^2}{2\mu}T_{11}^{(1)}(\alpha R_1)}{\nabla^2_0},\quad D_0=0
\end{equation*}
for $n=0$ where
\begin{equation*}
	\nabla^2_0=\begin{vmatrix}
		T_{11}^{(1)}(\alpha R_0) & T_{11}^{(2)}(\alpha R_0)\\
		T_{11}^{(1)}(\alpha R_1) & T_{11}^{(2)}(\alpha R_1)
	\end{vmatrix},
\end{equation*}
and for $n>0$ we have
\begin{equation*}
	A_n = \frac{\nabla^2_{n1}}{\nabla^2_n},\quad B_n = \frac{\nabla^2_{n2}}{\nabla^2_n},\quad C_n = \frac{\nabla^2_{n3}}{\nabla^2_n},\quad D_n = \frac{\nabla^2_{n4}}{\nabla^2_n}
\end{equation*}
where
\begin{equation}\label{Eq2:DeterminantForSphericalShell}
	\nabla^2_n = \begin{vmatrix}
		T_{11}^{(1)}(\alpha R_0) & T_{13}^{(1)}(\beta R_0) & T_{11}^{(2)}(\alpha R_0) & T_{13}^{(2)}(\beta R_0)\\
		T_{11}^{(1)}(\alpha R_1) & T_{13}^{(1)}(\beta R_1) & T_{11}^{(2)}(\alpha R_1) & T_{13}^{(2)}(\beta R_1)\\
		T_{41}^{(1)}(\alpha R_0) & T_{43}^{(1)}(\beta R_0) & T_{41}^{(2)}(\alpha R_0) & T_{43}^{(2)}(\beta R_0)\\
		T_{41}^{(1)}(\alpha R_1) & T_{43}^{(1)}(\beta R_1) & T_{41}^{(2)}(\alpha R_1) & T_{43}^{(2)}(\beta R_1)
	\end{vmatrix}
\end{equation}
\begin{equation*}
	\nabla^2_{n1} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		T_{13}^{(1)}(\beta R_1) & T_{11}^{(2)}(\alpha R_1) & T_{13}^{(2)}(\beta R_1)\\
		T_{43}^{(1)}(\beta R_0) & T_{41}^{(2)}(\alpha R_0) & T_{43}^{(2)}(\beta R_0)\\
		T_{43}^{(1)}(\beta R_1) & T_{41}^{(2)}(\alpha R_1) & T_{43}^{(2)}(\beta R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{n2} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		T_{11}^{(1)}(\alpha R_1) & T_{11}^{(2)}(\alpha R_1) & T_{13}^{(2)}(\beta R_1)\\
		T_{41}^{(1)}(\alpha R_0) & T_{41}^{(2)}(\alpha R_0) & T_{43}^{(2)}(\beta R_0)\\
		T_{41}^{(1)}(\alpha R_1) & T_{41}^{(2)}(\alpha R_1) & T_{43}^{(2)}(\beta R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{n3} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		T_{11}^{(1)}(\alpha R_1) & T_{13}^{(1)}(\beta R_1) & T_{13}^{(2)}(\beta R_1)\\
		T_{41}^{(1)}(\alpha R_0) & T_{43}^{(1)}(\beta R_0) & T_{43}^{(2)}(\beta R_0)\\
		T_{41}^{(1)}(\alpha R_1) & T_{43}^{(1)}(\beta R_1) & T_{43}^{(2)}(\beta R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{n4} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		T_{11}^{(1)}(\alpha R_1) & T_{13}^{(1)}(\beta R_1) & T_{11}^{(2)}(\alpha R_1)\\
		T_{41}^{(1)}(\alpha R_0) & T_{43}^{(1)}(\beta R_0) & T_{41}^{(2)}(\alpha R_0)\\
		T_{41}^{(1)}(\alpha R_1) & T_{43}^{(1)}(\beta R_1) & T_{41}^{(2)}(\alpha R_1)
	\end{vmatrix}.
\end{equation*}
The \textit{mechanical impedance} is now defined by
\begin{equation*}
	Z_n=\frac{R_0}{-\imag\omega\left[A_n U_1^{(1)}(\alpha R_0) + C_n U_1^{(2)}(\alpha R_0) + B_n U_3^{(1)}(\beta R_0) + D_n U_3^{(2)}(\beta R_0)\right]}
\end{equation*}
and the \textit{specific acoustic impedance} is given by
\begin{equation*}
	z_n = \imag\rho_{\mathrm{f}} c_{\mathrm{f}}\frac{h_n(kR_0)}{h_n'(kR_0)}.
\end{equation*}

\subsection{Vibration of spherical shell in vacuum}
The eigenvalues of a spherical elastic shell in vacuum is found by solving $\nabla^2_n=0$ (given by \Cref{Eq2:DeterminantForSphericalShell}) for all \textit{modes} $n$. For each mode $n$ there will be infinitely many eigenvalues. For a given $n$, we denote by $\omega_{nm}$ the eigenvalue corresponding to the $\mathrm{m}^\mathrm{th}$ zero of $\nabla^2_n$. The resulting eigenvalues seems to grow as $n$ grows for large $n$ (as shown in \Cref{Fig2:vibrationsOfSphericalShellInVacuumEigenvalues}). In \Cref{Tab2:sphericalShellFirstEigenValues} we show the first 4 zeros of $\nabla^2_n$ for $n$ from 0 to 20. The first four (lowest) eigenvalues are found to be $\omega_{21} = 764.12055$, $\omega_{31} = 907.96676$, $\omega_{41} = 972.16922$ and $\omega_{51} = 1017.829$.
\begin{table}
	\centering
	\caption[Eigenvalues for spherical shell]{\textbf{Vibration of spherical shell in vacuum}: Eigenvalues.}
	\label{Tab2:sphericalShellFirstEigenValues}
	\pgfplotstableset{% global config, for example in the preamble
	% these columns/<colname>/.style={<options>} things define a style
	% which applies to <colname> only.
	columns/n/.style={int detect,column type=r,column name=\textsc{$n$}}, 
	columns/omega_n_0/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n1}$}},
	columns/omega_n_1/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n2}$}},
	columns/omega_n_2/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n3}$}},
	columns/omega_n_3/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n4}$}},
	every head row/.style={before row=\toprule,after row=\midrule},
	every last row/.style={after row=\bottomrule}
	}
	\pgfplotstabletypeset[fixed zerofill,precision=6, 1000 sep={\,},1000 sep in fractionals]{../../data/plotData/analyticEigenValuesSphericalShell/sortedEigenvalues.dat}
\end{table}

\begin{figure}
	\centering
	\ifplotData
	\tikzset{every mark/.append style={scale=0.3}}
\tikzsetnextfilename{vibrationsOfSphericalShellInVacuumEigenvalues1}
	\begin{subfigure}[b]{0.75\textwidth}
		\begin{tikzpicture}
			\begin{axis}[
				width = 0.95\textwidth,
				height = 0.25\paperheight,
				% xtick={100, 1000, 10000,100000},
				%xticklabels={100, 1000, 10000,100000},
				%ytick={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
				%yticklabels={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
				enlarge x limits = true,
				cycle list={%
					{myYellow, mark=*}, 
					{mycolor, mark=*}, 
					{myGreen, mark=*}, 
					{myCyan, mark=*}, 
					{myRed, mark=*},
				},
				legend style={
					at={(0.97,0.03)},
					anchor=south east,
				},
				%xticklabels={0.2, 0.15, 0.1, 0.05, 0},
				%xmin=80, 
				ymin=-19000,
				ymax=220000,
				% xmax=200000, 
				xlabel=$n$,
				ylabel=$\omega_{nm}$]
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/0.dat};
				\addlegendentry{$1^\mathrm{st}$ zero of $\nabla^2_n$}
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/1.dat};
				\addlegendentry{$2^\mathrm{nd}$ zero of $\nabla^2_n$}
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/2.dat};
				\addlegendentry{$3^\mathrm{rd}$ zero of $\nabla^2_n$}
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/3.dat};
				\addlegendentry{$4^\mathrm{th}$ zero of $\nabla^2_n$}					
				\addplot [black, dotted] coordinates{(-1, -19000) (10, -19000) (10, 150000) (-1, 150000) (-1, -19000)};
			\end{axis}
		\end{tikzpicture}
	\end{subfigure}
	\tikzsetnextfilename{vibrationsOfSphericalShellInVacuumEigenvalues2}
	\begin{subfigure}[b]{0.23\textwidth}
		\begin{tikzpicture}
			\begin{axis}[
				width = \textwidth,
				height = 0.25\paperheight,
				% xtick={100, 1000, 10000,100000},
				%xticklabels={100, 1000, 10000,100000},
				%ytick={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
				%yticklabels={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
				enlarge x limits = true,
				cycle list={%
					{myYellow, mark=*}, 
					{mycolor, mark=*}, 
					{myGreen, mark=*}, 
					{myCyan, mark=*}, 
					{myRed, mark=*},
				},
				%xticklabels={0.2, 0.15, 0.1, 0.05, 0},
				%xmin=80, 
				% ymin=0.0007,
				% xmax=200000, 
				xlabel=$n$,
				xmin=-1, 
				xmax=10, 
				ymin=-19000,
				ymax=150000,
				%ylabel=$\omega_{nm}$,
	%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
				%yticklabels={},
				]
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/0.dat};
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/1.dat};
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/2.dat};
				\addplot table[x=n,y=Eigenvalues] {../../data/plotData/analyticEigenValuesSphericalShell/3.dat};
			\end{axis}
		\end{tikzpicture} 
	\end{subfigure}
	\fi
	\caption[Plot of eigenvalues for spherical shell in vacuum]{\textbf{Vibrations of spherical shell in vacuum:} All eigenvalues below $2\cdot 10^5$, which results in 1186 eigenvalues. The plot on the right shows a magnification of the domain inside the dotted lines.}\label{Fig2:vibrationsOfSphericalShellInVacuumEigenvalues}
\end{figure}

\subsection{Scattering on a rigid sphere}
\label{Subsubsec:scatteringOnRigidSphere}
Let the plane wave
\begin{equation*}
	p_{\textrm{inc}}(r,\vartheta) = P_0\euler^{\imag kz} = P_0\euler^{\imag kr\cos\vartheta}
\end{equation*}
be scattered on a sphere with radius $R$. The resulting scattered wave is then
\begin{equation*}
	p_{\mathrm{s}\infty} (r,\vartheta) = -P_0\sum_{n=0}^\infty \imag^n (2n+1) P_n(\cos\vartheta)\frac{j_n'(kR)}{h_n'(kR)} h_n(kr).
\end{equation*}
For details of this solution see~\cite[p. 28]{Ihlenburg1998fea}.
%such that the total pressure is given by
%\begin{equation*}
%	p(r,\vartheta) = p_{\textrm{inc}}(r,\vartheta) + p_{s\infty} (r,\vartheta).
%\end{equation*}

\subsection{Scattering on elastic spherical shell}
\tikzsetnextfilename{IllustrationOfScattering}
\begin{figure}
	\centering
	\begin{tikzpicture}[scale=0.9]
		\def\a{5}		% Radius of the midsurface of the shell
		\def\aa{6}		% Radius of the midsurface of the shell
		\def\rOuter{5.075}		% Ending iteration (if no overlap is wanted set this to be \D-1)
		\def\t{0.25} 		% Starting angle of characteristics in fan	
		\def\axisScale{8} 		% Scale length of the axis
		\def\arrowScale{0.7} 		% Scale length of the axis
		\def\sqrtTwo{1.414213562373095}
		
		\draw[->] (-\a-\axisScale*\t/2,0) -- (\a+\axisScale*\t/2,0) node[right] {$z$};
		\draw[->] (0,-\a-\axisScale*\t/2) -- (0,\a+\axisScale*\t/2) node[above] {$x$};
		
		\filldraw[fill=solid] (0,0) circle (\a+\t/2);
		\filldraw[fill=white] (0,0) circle (\a-\t/2);
		\draw[dotted] (0,0) circle (\a);
		
		\draw[-] (-\a+\t/2,0) -- (\a-\t/2,0);
		\draw[-] (0,-\a+\t/2) -- (0,\a-\t/2);
		\draw[dashed] (0,0) -- (-\aa,\aa) node[above left]{$\vec{P}_{\mathrm{s}}(r_{\mathrm{s}},\alpha_{\mathrm{s}},\beta_{\mathrm{s}})$};
		
		\draw[->] (180+45:\a+1) node[above, left] {$t$}  -- (180+45:\a+\t/2);
		\draw[->] (180+45:\a-1) -- (180+45:\a-\t/2);
		
		\draw[->] (0,0) -- node[above=0.1cm, left] {$R$} (180+30:\a);
		\draw[->] (0,0) -- node[above, left] {$R_1$} (180+45+15:\a-\t/2);
		\draw[->] (0,0) -- node[below=0.5cm, right=-0.2cm] {$R_0$} (180+45+30:\a+\t/2);
		
		\draw[->] (0.5,0) arc (0:135:0.5);
		\draw (0.3, 0.7) node{$\alpha_{\mathrm{s}}$};
		
		\draw[dashed] (0,0) -- (\aa,\aa) node{$\bullet$} node[above]{$\vec{P}_{\mathrm{f}}(r_{\mathrm{f}},\alpha_{\mathrm{f}},\beta_{\mathrm{f}})$};
		\draw[->] (1,0) arc (0:45:1);
		\draw (1.2, 0.4) node{$\alpha_{\mathrm{f}}$};
		
		\draw[->] (-\aa,\aa) -- (-\aa+1.5,\aa-1.5);
		\def\dx{2};
		\def\dy{2};
		\def\x{-0.95*\aa-\dx/2};
		\def\y{0.95*\aa-\dy/2};
		\draw (\x,\y) -- (\x+\dx,\y+\dy);
		\def\x{-0.9*\aa-\dx/2};
		\def\y{0.9*\aa-\dy/2};
		\draw (\x,\y) -- (\x+\dx,\y+\dy);
		\def\x{-0.85*\aa-\dx/2};
		\def\y{0.85*\aa-\dy/2};
		\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\end{tikzpicture}
	\caption[The spherical shell in the $xz$-plane]{\textbf{Scattering on elastic spherical shell}: The spherical shell in the $xz$-plane. Here with $R=5$ and $t=0.25$ (the calculations uses $t=0.15$ and are here set to 0.25 only for visualization purposes).}
	\label{Fig2:IllustrationOfScattering}
\end{figure}
The full 3D exact solution to the elastic scattering problem is given by
\begin{equation}\label{Eq2:exact3DscatteringSphericalShellSol}
	p(r,\vartheta) = p_{\mathrm{s},\infty}(r,\vartheta) + p_{\mathrm{s},\mathrm{r}}(r,\vartheta)
\end{equation}
where
\begin{equation*}
	p_{\mathrm{s},\infty}(r,\vartheta) = -P_0\sum_{n=0}^\infty (2n+1)\imag^n P_n(\cos\vartheta) \frac{j_n'(kR_0)}{h_n'(kR_0)}h_n(kr)
\end{equation*}
and
\begin{equation*}
	p_{\mathrm{s},\mathrm{r}}(r,\vartheta) = \frac{P_0\rho_{\mathrm{f}} c_{\mathrm{f}}}{(kR_0)^2}\sum_{n=0}^\infty \frac{\imag^n(2n+1)P_n(\cos\vartheta)h_n(kr)}{[h_n'(kR_0)]^2(Z_n+z_n)}.
\end{equation*}
Here, $p_{\mathrm{s},\infty}$ represent a scattered wave from a rigid body, and $p_{\mathrm{s},\mathrm{r}}$ represent the pressure corresponding to the forced vibrations of the elastic body in fluid (loaded with the sum of incident pressure $p_{\mathrm{inc}}$ and the rigid body scattered pressure $p_{\mathrm{s},\infty}$) (see~\cite[p. 2]{Chang1994voa} for more details). Note that we do not include the incident pressure field $p_{\mathrm{inc}}$ in $p$, as this field is not present in the numerical solution. However, to compute the total physical pressure at the wet surface this field must be included (in addition to the constant background pressure).
\begin{figure}
	\centering
	\ifplotData
	\tikzsetnextfilename{BackScatteredPressure1}
	\begin{subfigure}[b]{0.75\textwidth}
		\begin{tikzpicture}
			\begin{axis}[
				cycle list={%
					{mycolor}
				},
				width = 0.95\textwidth,
				height = 0.25\paperheight,
				%width=0.45*350pt,
				%height=0.5*250pt,
				xlabel=$k$,
				ylabel=$|F(k)|$,
				ymax=30,
				ymin=-4,
				]
				\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_fine2.dat};
				\addplot [black, dotted] coordinates{(1.362, -4) (1.38, -4) (1.38, 30) (1.362, 30) (1.362, -4)};
			\end{axis}
		\end{tikzpicture}
	\end{subfigure}
	\tikzsetnextfilename{BackScatteredPressure2}
	\begin{subfigure}[b]{0.23\textwidth}
		\begin{tikzpicture}
			\begin{axis}[
				width =\textwidth,
				height = 0.25\paperheight,
				cycle list={%
					{mycolor}
				},				
%xticklabel style={
%rotate 90,
%/pgf/number format/precision=12,
%},
				xtick={8.7431},
				xticklabels={1.3715},
	%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
				yticklabels={},
				%xmin=80, 
				%xmax=100000, 
				xlabel=$k$,
				%ylabel=$|F(k)|$,
				ymax=30,
				ymin=-4,
				]
				\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_specialCase.dat};
			\end{axis}
		\end{tikzpicture} 
	\end{subfigure}
	\fi
	\caption[Far-field pattern of backscattered pressure for elastic spherical shell]{\textbf{Scattering on elastic spherical shell}: Far-field pattern of backscattered pressure (we set $\alpha_{\mathrm{s}} = \alpha_{\mathrm{f}} = \pi$) for elastic spherical shell (monostatic calculation). The plot on the right shows a magnification (in $x$-direction) of the domain inside the dotted lines. The length of the domain of this plot is $\nabla^2 k = 10^{-6}$.}
\label{Fig2:BackScatteredPressure}
\end{figure} 

In \Cref{Fig2:BackScatteredPressure} we plot the modulus of the function
\begin{equation*}
	F(k) = r_{\mathrm{f}}\euler^{\imag k r_{\mathrm{f}}} p(r_{\mathrm{f}},\alpha_{\mathrm{f}},\beta_{\mathrm{f}})
\end{equation*}
where $\vec{P}_{\mathrm{f}}$ is the far field point which depends on $r_{\mathrm{f}}$, $\alpha_{\mathrm{f}}$ and $\beta_{\mathrm{f}}$ (cf. \Cref{Fig2:IllustrationOfScattering}). This plot illustrates the complexity of the exact solution at hand. It seems to be discontinuous at the eigenmodes (with wave numbers found in \Cref{Tab2:comparisons}), but if zoomed in enough, we observe the spikes to be smooth as well. As \Cref{Fig2:BackScatteredPressure} illustrates, we must magnify a lot to show details of the higher eigenmodes. If such a detailed plot was to be illustrated using uniform sampling, we would need several millions of samples. Due to the complexity of the functions involved, this would be very time consuming, so it is more practical to use non uniform sampling. Needless to say, to find these higher eigenmodes using a numerical approximation will be very hard, even though we know a priori the exact location of the analytic eigenmodes. 
\tikzsetnextfilename{BackScatteredPressureDensities}
\begin{figure}
	\centering
	\ifplotData
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed}, 
				{mycolor}, 
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$k$,
			ylabel=$|F(k)|$,
			ymax=19,
			ymin=-4,		
			xmin = 0.2,
			xmax = 0.72
			]
			\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_air_fine2.dat};
			\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_fine2.dat};
			\addlegendentry{Air: $\rho_{\mathrm{f}}=1$}
			\addlegendentry{Water: $\rho_{\mathrm{f}}=1000$}
		\end{axis}
	\end{tikzpicture}
	\fi
	\caption[Scattering from elastic shell with different fluid densities]{\textbf{Scattering on elastic spherical shell}: Scattering from elastic shell with different fluid densities.}
\label{Fig2:BackScatteredPressureDensities}
\end{figure}

In \Cref{Fig2:BackScatteredPressureDensities} we also show the effect of low density of the fluid. As we can see from \Cref{Tab2:comparisons}, the eigenmodes of a spherical shell surrounded by air (with low density) comes close to the corresponding wave numbers for a spherical shell in vacuum. As Ihlenburg points out, an increase in the density of the acoustic medium around the spherical shell results in a larger shift to the left of the eigenmodes.
\begin{table}
	\centering
	\caption[Comparison of wave number of modes]{\textbf{Spherical shell:} Comparison of wave number of modes in the case of air and water ($\rho_{\mathrm{f}}=1$ and $\rho_{\mathrm{f}}=1000$ respectively) and shall theory solution (for water) versus the values for spherical shell in vacuum.}
	\label{Tab2:comparisons}
	\pgfplotstableset{% global config, for example in the preamble
	% these columns/<colname>/.style={<options>} things define a style
	% which applies to <colname> only.
	columns/vacuum/.style={/pgf/number format/fixed, sci sep align, column name={Vacuum $\rho_{\mathrm{f}}=0$}},
	columns/air/.style={/pgf/number format/fixed, sci sep align, column name={Air $\rho_{\mathrm{f}}=1$}},
	columns/water/.style={/pgf/number format/fixed, sci sep align, column name={Water $\rho_{\mathrm{f}}=1000$}},
	columns/shelltheory/.style={/pgf/number format/fixed, sci sep align, column name={Shell theory $\rho_{\mathrm{f}}=1000$}},
	every head row/.style={before row=\toprule,after row=\midrule},
	every last row/.style={after row=\bottomrule}
	}
	\pgfplotstabletypeset[fixed zerofill,precision=9, 1000 sep={\,},1000 sep in fractionals]{../../data/plotData/analyticEigenValuesSphericalShell/comparison.dat}
\end{table}

Ihlenburg uses a shell theory solution as a reference solution. The only difference will then be the function $Z_n$ which in the case of shell theory is given by
\begin{equation*}
	Z_0 = \frac{E t\left[\Omega^2 - 2(1+nu)\right]}{\imag\omega R^2\left(1-\nu^2\right)}
\end{equation*}
for $n=0$ and
\begin{equation*}
	Z_n = \frac{\begin{vmatrix}
	\Omega^2-\left(1+\beta^2\right)(\nu+\lambda_n-1) & -\beta^2(\nu+\lambda_n - 1)-(1+\nu)\\
	-\lambda_n \left(\beta^2(\nu+\lambda_n-1)+(1+\nu)\right) & \Omega^2-2(1+\nu)-\beta^2\lambda_n (\nu+\lambda_n-1)
	\end{vmatrix}}{-\imag\omega\begin{vmatrix}
		\Omega^2-\left(1+\beta^2\right)(\nu+\lambda_n-1) & 0\\
		-\lambda_n\left[\beta^2(\nu+\lambda_n-1)(1+\nu)\right] & -\frac{R^2\left(1-\nu^2\right)}{Et}
	\end{vmatrix}}
\end{equation*}
for $n>0$, where
\begin{equation*}
	\Omega = \frac{R\omega}{c_s},\quad\omega = kc_{\mathrm{f}},\quad c_s = \sqrt{\frac{E}{(1+\nu^2)\rho_s}},\quad \lambda_n = n(n+1)\quad\text{and}\quad \beta = \frac{t}{\sqrt{12}R}.
\end{equation*}
\tikzsetnextfilename{shellTheory3Dcomparison}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed}, 
				{mycolor}, 
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel=$k$,
			ylabel=$|F(k)|$,
			ymax=30,
			ymin=-7			
			]
			\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_shelltheory2.dat};
			\addplot table[x=k,y=F_k] {../../data/plotData/backscatteredPressureSphericalShell/analytic_fine2.dat};
			\addlegendentry{Shell theory solution}
			\addlegendentry{Full 3D exact solution}
		\end{axis}
	\end{tikzpicture}
	\caption[Comparison between shell theory solution and full 3D exact solution]{\textbf{Scattering on elastic spherical shell}: Comparison between shell theory solution and full 3D exact solution.}
\label{Fig2:shellTheory3Dcomparison}
\end{figure}

In \Cref{Fig2:shellTheory3Dcomparison} we plot both our full 3D solution and this shell theory solution. The error is significant and is specially large at the eigenmodes. In \Cref{Fig2:shellTheory3DcomparisonError} a more informative picture regarding the error is computed. Due to the large variation of the data sets, the most reasonable norm is the absolute difference divided by the maximum absolute value. That is, for two finite data sets $\{x_i\}$ and $\{y_i\}$ the relative difference $E_i$ for each pair $(x_i,y_i)$ is given by
\begin{equation}\label{Eq2:absoluteRelDiffNew}
	E_i = \frac{| x_i - y_i|}{\mathrm{max}(|x_i|, |y_i|)}
\end{equation}
We obviously also here see large errors at every eigenmode, but also elsewhere, the error is significant. In average, the error lies above 1\%. In the applications of complex geometries, this result would be acceptable, but we want to be able to perform convergence analysis on this spherical shell where the obtained error may end up being far below 1\%. This way, we can draw conclusion of which sets of parameters increases the convergence rate the most. The exactness of the solution is therefore considered to be of importance.
\tikzsetnextfilename{shellTheory3DcomparisonError}
\begin{figure}
	\centering
	\ifplotData
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor}, 
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%ymax=30,
			%ymin=-7
			xlabel=$k$,
			ylabel=Relative absolute difference (\%)			
			]
			\addplot table[x=k,y=F_k,y expr= \thisrow{F_k}*100] {../../data/plotData/backscatteredPressureSphericalShell/error2.dat};
		\end{semilogyaxis}
	\end{tikzpicture}
	\fi
	\caption[Error between shell theory solution and full 3D exact solution]{\textbf{Scattering on elastic spherical shell}: Error between shell theory solution and full 3D exact solution.}
\label{Fig2:shellTheory3DcomparisonError}
\end{figure}

==> contents/computationalAspects.tex <==
\section{Computational aspects}
\label{Sec2:compAsp}
\tikzstyle{startstop} = [rectangle, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=yellow!30]
\tikzstyle{forloopbegin} = [rectangle, minimum width=5cm, rounded corners, minimum height=1cm, text centered, text width=5cm, draw=black, fill=green!30]
\tikzstyle{forloopend} = [circle, draw=black, fill=green!30]
\tikzstyle{processPar} = [text width=5cm, rectangle, rounded corners, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=5cm, minimum height=1cm, text centered, text width=5cm, draw=black, fill=blue!30]
\tikzsetnextfilename{flowchart} 
\begin{figure}
	\centering
	\begin{tikzpicture}[node distance=2cm]

	\node (start) [startstop] {Start};
	\node (NURBS) [process, below of=start] {Initialization};
	\node (structure) [processPar, below of=NURBS] {Build structural matrices};
	\node (fluid) [processPar, below of=structure] {Build fluid matrices};
	\node (infelems) [processPar, below of=fluid] {Add contribution from infinite elements};
	\node (ghost1a) [below of=infelems] {};
	\node (ghost1b) [right of=ghost1a, xshift=2cm] {};
	\node (ghost1c) [right of=NURBS, xshift=2cm] {};
	\node (ghost1d) [right of=ghost1c, xshift=2cm] {};
	
	\node (loopLoading) [forloopbegin, below of=ghost1d] {Loop through \\ angles $\alpha_{\mathrm{s}}$ and $\beta_{\mathrm{s}}$};
	\node (ghost2a) [right of=loopLoading, xshift=2cm] {};
	\node (loading) [processPar, below of=loopLoading] {Build loading vector and add contribution from coupling conditions};
	\node (solveSystem) [processPar, below of=loading] {Solve system};
	
	\node (loopFarField) [forloopbegin, below of=solveSystem] {Loop through \\ angles $\alpha_{\mathrm{f}}$ and $\beta_{\mathrm{f}}$};
	\node (ghost3a) [right of=loopFarField, xshift=1cm] {};	
	\node (farField) [processPar, below of=loopFarField] {Compute backscattered pressure};
	\node (forloopfinishFarField) [forloopend, below of=farField] {};
	\node (ghost3b) [right of=forloopfinishFarField, xshift=1cm] {};	
	\node (forloopfinishLoading) [forloopend, below of=forloopfinishFarField] {};
	\node (ghost2b) [right of=forloopfinishLoading, xshift=2cm] {};
	\node (stop) [startstop, below of=forloopfinishLoading] {Stop};
	
	\draw [->] (start) -- (NURBS);
	\draw [->] (NURBS) -- (structure);
	\draw [->] (structure) -- (fluid);
	\draw [->] (fluid) -- (infelems);
	\draw [->] (infelems) |- (ghost1b) -- (ghost1a) -| (ghost1c) -- (ghost1b)  |- (ghost1d) -- (ghost1c) -| (loopLoading);
	
	\draw [->] (loopLoading) -- (loading);
	\draw [->] (loading) -- (solveSystem);
	\draw [->] (solveSystem) -- (loopFarField);
	\draw [->] (loopFarField) -- (farField);
	\draw [->] (farField) -- (forloopfinishFarField);
	\draw [->] (forloopfinishFarField) -- (forloopfinishLoading);
	\draw [->] (forloopfinishFarField) -| (ghost3a) -- (ghost3b) |- (loopFarField);
	\draw [->] (forloopfinishLoading) -| (ghost2a) -- (ghost2b) |- (loopLoading);
	\draw [->] (forloopfinishLoading) -- (stop);
	
	
	\end{tikzpicture}
	\caption[The flowchart of the full FSI program]{\textbf{The FSI program}: The flowchart of the full FSI program analyzing both monostatic and bistatic cases. The boxes with rounded corners are parallelized.}
	\label{Fig2:flowchart}
\end{figure}
In \Cref{Fig2:flowchart} we give an overview of the code for the full fluid structure interaction program for both monostatic and bistatic cases. The only part which is not parallelized is the initialization part of the code. The time elapsed by this part is negligible in comparison with any other part of the program, so any effort for optimizing this part was omitted. In the following we shall briefly present the main content of each step.

\subsection{Initialization}
The initialization part consist of defining all relevant parameters and constructing the mesh for analysis. To create the IGA mesh, we first import data for the coarsest mesh of the NURBS object (i.e. data set's found in \Cref{Sec2:NURBSdata}). One typically first constructs the NURBS object for the solid domain as this domain should be the exact representation of the given object. In contrast, we have more degrees of freedom when construction the fluid mesh. The mesh for the fluid domain must be constructed by finding a suitable spheroid which may be wrapped closely around the obstacle without creating to much of a distortion in the resulting mesh (see \Cref{subse:ConstructionModel3Mesh}). Although it may certainly be possible, it has not been implemented an automated algorithm for finding such a spheroid. So in the analysis, we have found the fluid mesh by trial and failure. When the two meshes have been constructed (two NURBS patches) one has many opportunities of $k$-refinement. The two algorithms \mcode{elevateNURBSdegree} and \mcode{insertKnotsInNURBS} have been implemented for this purpose (see \Cref{subse:NURBSvolumes}). Typically we order elevate first to the desired degrees in $\xi$-, $\eta$- and $\zeta$-direction. Then we insert the desired number of knots in the desired locations (creating more elements for analysis). From this point, we are able to create the IGA mesh. We first construct an ordering of the available NURBS basis functions, then we construct a connectivity array which for each element links every basis functions having support on this element. From here, it is important to have knowledge if there is any periodicity involved for the NURBS patch. If this is the case, one must find the overlapping control points causing the periodicity. There could potentially be more than two control points at the same physical location. In any case, define the control point with lowest index to be the ``parent function'' and the rest ``children functions''. Then one constructs an array mapping all children functions to the parent function. This array is then used to modify the mentioned connectivity array. In addition to keeping track of the indices for the parent functions, one must also store the indices for the children functions as these degrees of freedom must be removed from the global system matrix.

\subsection{Structural matrices and fluid matrices}
When constructing the stiffness matrix and the mass matrix, we create four arrays for these two matrices. The first two arrays will contain the indices (columns and rows) in the global matrix. The other two arrays stores the contribution at these indices for each of the two matrices. We continue by creating an array of Gaussian quadrature points and weights. The code supports 64 Gaussian quadrature points per direction such that one is able to evaluate a 3D IGA element at $64^3=262144$ points. However, one typically determines the number of control points by the NURBS degree for each of the parameter directions. More specifically, if the degree in $\xi$ direction is $p$, then we use $p+1$ quadrature points in this direction. Thus, we have $(p+1)(q+1)(r+1)$ quadrature points per volume element. 

It is very important to note that the global stiffness matrix is very sparse. Not only is it a huge advantage in MATLAB to have the matrix in sparse format when solving the linear system, but also when assembling the matrix. If the matrix is made sparse only after assembly, then the initialization would require MATLAB to allocated place for a full stiffness matrix. This is very memory consuming and should be avoided if one wants to run the program with many degrees of freedom. A matrix in sparse format contains 3 columns; the first two represent the indices in the matrix and the third column represent the corresponding value. The problem of preallocation may be solved by first construct these three columns in three arrays. By noting that each element stiffness matrix has $\left[3(p+1)(q+1)(r+1)\right]^2$ number of components, we initialize the arrays by the following.
\begin{lstlisting}
n_en = (p+1)*(q+1)*(r+1);
sizeOfk_e = (3*n_en)^2;
indices = zeros(3*n_en,noElems); 
spIdxRow = zeros(sizeOfk_e,noElems);
spIdxCol = zeros(sizeOfk_e,noElems);
Kvalues = zeros(sizeOfk_e,noElems); 
\end{lstlisting}
Note that we initialize these ``vectors'' in matrix form as this allows us to easily parallelize using \mcode{parfor} in MATLAB.

Note that we do not here sum overlapping element matrices, but this is automatically done when the \mcode{sparse} function is called in MATLAB.
\begin{lstlisting}
K = sparse(spIdxRow,spIdxCol,values);
\end{lstlisting}
That is, there will be index combinations which will repeat and therefore this method would require a lot more memory. Using server with 256GB memory space, one is able to run this implementation with up to $10^6$ degrees of freedom, which is more than enough for this thesis. Thus, the results evaluated for this thesis is done relatively fast.

The other obvious method is simply using
\begin{lstlisting}
K(sctrB,sctrB) = K(sctrB,sctrB) + k_e;
\end{lstlisting}
which typically results in the MATLAB warning ``This sparse indexing expression is likely to be slow''. In~\cite{Karatarakis2013cot} it is described how one could optimize the assembly, and in~\cite{Hughes2010eqf} we find theory around efficiently use of quadrature for NURBS. In~\cite{Jansson2013osm} a new stack based representation of the sparse matrix is presented, which could speed up the matrix assembly part. This is however outside the scope of this thesis, and is therefore not included.

We are now ready to loop through all structure elements and calculate their contribution to the stiffness and mass matrix. For each element in this loop (which is parallelized) we must loop through all quadrature points. For each quadrature point in this inner loop, we evaluate all the NURBS basis functions which have support on the current element. The Jacobian is then computed (by \Cref{Eq2:NURBSjacobian}) in order to find the derivative of the basis functions with respect to physical coordinates (\Cref{Eq2:basisFunsDerivativeRel}) which is then used to find the strain matrix $\vec{B}$ (\Cref{Eq2:strainMatrixB}). Note that if body forces is to be applied to the solid, these will be calculated in this same loop. So one must not mistake the part of building the loading vector with the implementation of body forces. However, we never encounter body forces in the analysis of acoustic scattering, but it has been implemented anyways as some static elasticity problems involving body forces has been analyzed in this thesis (the Kneaded cylinder in \Cref{subse:KneadedCylinder} and Scordelis-Lo Roof in \Cref{subse:Scordeli}).

After looping through all elements, one creates the sparse matrices $\vec{K}$ and $\vec{M}$ using the \mcode{sparse} function in MATLAB. These matrices are then added (with a scaling factor for the mass matrix). The reason why they are not added during calculation is simply to create a more general function which handles the elastostatic case as well (no construction of the mass matrix).

The next step is to construct the matrices for the fluid part of the domain. The setup is almost identical to the case for the structure matrices. However, we are now working with scalar valued domain instead of a vector valued domain. This will affect the indexing. In addition, the bilinear form is different for the two cases. After computing the fluid matrices, the result is added to the global matrix.

\subsection{Contribution from infinite elements}
The infinite elements are implemented using the multi-pole expansion after Burnett in~\cite{Burnett1994atd}. We generalize this work, which was based on the BGU formulation, to the other three formulations BGC, PGU and PGC (see \Cref{se:infElems}).

One first needs to locate the indices for the NURBS basis functions having support on the artificial boundary $\Gamma_{\mathrm{a}}$. In addition, the radial integrals in the bilinear or sesquilinear form must be computed (depending on which infinite element formulation is chosen). Finally, one must compute the coefficients used for the radial basis functions in the infinite elements (from the relation \Cref{Eq2:infElemCoeffs}). These two last step suffers from round off errors for a high number of infinite element radial basis functions $N$. The way to solve this is to increase the precision using the mentioned MuPAD in MATLAB.

We are now ready to loop through all surface elements on $\Gamma_{\mathrm{a}}$. Once again, for each element, we have an inner loop over all quadrature points. And for each quadrature points, the NURBS basis functions are evaluated, such that the Jacobi matrix can be computed. This is in turn used to compute the derivative with respect to the prolate spheroidal coordinates. In this regards it has been implemented a function which evaluates $(r,\vartheta,\phi)$ for a given point $(x,y,z)$ (using the relations in \Cref{Eq2:XtoProl}). Moreover, the derivatives of $(r,\vartheta,\phi)$ with respect to $(x,y,z)$ must be computed (using the relations in \Cref{Eq2:dProlateSphericalCoordinatesdX}). We may then compute the derivatives of $(r,\vartheta,\phi)$ w.r.t, the surface parameters $\xi$ and $\eta$ using \Cref{Eq2:dPdNURBS}. These derivatives are finally used to evaluate the derivatives of the basis functions with respect to the angles $\vartheta$ and $\phi$ using \Cref{Eq2:dRdP}. This enables us to compute the contributions to the surface integrals $J_{AB}^{(1)}$, $J_{AB}^{(2)}$, $J_{AB}^{(3)}$, $J_{AB}^{(4)}$ and $J_{AB}^{(5)}$ (expressions in \Cref{Eq2:surfaceIntegralsInfElems}). Note that we do not compute the full bilinear or sesquilinear form in this inner loop, as the radial integrals is independent of the angular coordinates (to avoid redundant computations). After looping through the quadrature points, we continue the loop on the current element and evaluates the bilinear or the sesquilinear form. This is done by looping through all radial basis functions in the infinite elements. The result is then collected and added to the global matrix.

\subsection{Loading vector and coupling condition}
The coupling conditions connects the two spaces for the solid domain and the fluid domain. This involves a coupling of two NURBS objects. The implementations assume the surfaces to be connected have the same NURBS parametrization. It also assumes the NURBS patches to be parametrized in such a way that these surfaces are given at $\zeta=0$ for the fluid and $\zeta =1$ for the solid. This causes restriction in the refinement process; if we want to, say, insert a knot in the $\xi$ direction, or order elevate in this direction in the fluid, we must do the same refinement process in the solid.

Keeping these remarks in mind, we start again by constructing the surface mesh. This mesh is constructed on the basis of the surface at $\zeta=1$ for the solid. We then loop through these surface elements, and for each element we must loop through the quadrature points. For each such quadrature point we now evaluate 2D NURBS functions, as we know the 3D NURBS functions reduce to 2D NURBS functions when $\zeta$ is constant. This obviously saves a lot of computations. Once again, these evaluations are used to compute the (2D) Jacobian which is in this case not used to evaluate derivatives of the NURBS functions w.r.t. physical coordinates, as they do not appear in the coupling conditions. The Jacobian is only used to compute the cross product needed to compute the surface integral (see \Cref{Eq2:surfIntegral}). This cross product is also needed to determine the normal vector in the coupling term in the FSI bilinear form (\Cref{Eq2:FSIbilinearForm}). As we want this normal vector to point out from the solid domain, and we consider the NURBS parametrization of the solid domain, the normal vector is given by
\begin{equation*}
	\vec{n} = \frac{\pderiv{\vec{X}}{\xi}\times\pderiv{\vec{X}}{\eta}}{\left\| \pderiv{\vec{X}}{\xi}\times\pderiv{\vec{X}}{\eta}\right\|}
\end{equation*}
for right hand oriented NURBS parametrization. It is here assumed that the parametrization is orientable. The parametrization is right hand oriented whenever $\det(\vec{J})>0$ throughout the domain. If $\det(\vec{J})<0$ throughout the domain, we simply need to change the sign of the normal vector in the expression above.

We continue by computing the physical coordinates in order to evaluate the given incident field $p_{\mathrm{inc}}$ and its derivative. The result is then collected and added to the global matrix. Note that the other contributions to the global matrix is independent of the incident field such that they only need to be computed once (thus we store this part). Moreover, if only hard walled boundary conditions are considered (only fluid, and no coupling), then there is no update in the global matrix in this loop. If a direct solver is chosen, one may split the loop over the angles $\alpha_{\mathrm{s}}$ and $\beta_{\mathrm{s}}$ such that the factorization is only done once. 

\subsection{Solving the system}
If there are many angles to be analyzed, the loops over these angles should be parallelized. However, if one only consider few angles (for instance the bistatic case when only one pair of $\alpha_{\mathrm{s}}$ and $\beta_{\mathrm{s}}$ is considered), one should take the parallelization over the loop which runs through the surface elements.

When a direct solver is to be used, the backslash operator in MATLAB will elegantly solve the problem in a efficient way. However, if the LU factorization may be reused (which is the case when no coupling is present) one should use the build in \mcode{lu} function. If the LU factorization is reused, one should no longer parallelize over the angles as this would require the LU factorization to be copied in each thread (a wast amount of extra memory is thus acquired). More details on the subject can be found in~\cite{Davis2013anf}.

For a given incident field, consider now the full global matrix. We should then remove the degrees of freedom corresponding to all children functions. After this is done, we may now investigate the resulting structure of the global matrix $A$. 
\tikzsetnextfilename{spyA} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\def\scalingFact{41.4}
		\begin{scope}[y=-1cm,x=1cm]
			\node[anchor=north west,inner sep=0] at (-0.10,-0.12) {\includegraphics[width=0.8425\textwidth]{../../graphics/spyAcutted.pdf}};
		    \draw[myGreen] (0, 0) rectangle (389.5/\scalingFact,389.5/\scalingFact);
		    \draw[myYellow] (390.5/\scalingFact,0) rectangle (416/\scalingFact,389.5/\scalingFact);
		    \draw[myYellow] (0,390.5/\scalingFact) rectangle (389.5/\scalingFact,416/\scalingFact);
		    \draw[myRed] (390.5/\scalingFact,390.5/\scalingFact) rectangle (494/\scalingFact,494/\scalingFact);
		    \draw[myRed,dashed] (469/\scalingFact,469/\scalingFact) rectangle (546/\scalingFact,546/\scalingFact);
		    
	
		    \draw (-5/\scalingFact,-5/\scalingFact) -- (-5/\scalingFact, 551/\scalingFact) node[midway, left]{$\vec{A} = $};	   
		    \draw (-5/\scalingFact,-5/\scalingFact) -- (0,-5/\scalingFact);
		    \draw (-5/\scalingFact, 551/\scalingFact) -- (0, 551/\scalingFact);
		    
		    \draw (551/\scalingFact,-5/\scalingFact) -- (551/\scalingFact, 551/\scalingFact);	   
		    \draw (551/\scalingFact,-5/\scalingFact) -- (546/\scalingFact,-5/\scalingFact);
		    \draw (551/\scalingFact, 551/\scalingFact) -- (546/\scalingFact, 551/\scalingFact);
		    
		    
		    \draw[<->,myGreen] (0,-4/\scalingFact) -- (130/\scalingFact, -4/\scalingFact) node[midway, above,myGreen]{$x$ component};
		    \draw[<->,myGreen] (130/\scalingFact,-4/\scalingFact) -- (260/\scalingFact, -4/\scalingFact) node[midway, above,myGreen]{$y$ component};
		    \draw[<->,myGreen] (260/\scalingFact,-4/\scalingFact) -- (390/\scalingFact, -4/\scalingFact) node[midway, above,myGreen]{$z$ component};
		    
		    \draw[<-,myGreen] (370/\scalingFact, 145/\scalingFact) -- (450/\scalingFact,145/\scalingFact) node[right,myGreen]{Solid};
		    \draw[<-,myYellow] (400/\scalingFact, 170/\scalingFact) -- (450/\scalingFact,170/\scalingFact) node[right,myYellow]{Coupling};
		    
		    \draw[<-,myRed] (440/\scalingFact, 398/\scalingFact) -- (440/\scalingFact,195/\scalingFact) -- (450/\scalingFact,195/\scalingFact) node[right,myRed]{Fluid (FE)};
		    
		    \draw[<-,myRed,dashed] (515/\scalingFact, 475/\scalingFact) -- (494/\scalingFact,234/\scalingFact) node[above,myRed]{Fluid (IE)};
		    
		    \node[below right] at (0,416/\scalingFact) {
			\begin{minipage}{0.6\linewidth}
				\footnotesize{
				\begin{align*}
					\textcolor{myRed}{\int_{\Omega^+} \nabla q\cdot\nabla p - k^2 qp\idiff \Omega} &+ \textcolor{myYellow}{\rho_{\mathrm{f}}\omega^2\left(\int_\Gamma q u_i n_i \idiff \Gamma + \int_\Gamma v_i n_i p \idiff \Gamma\right)}\\
					 &+ \textcolor{myGreen}{\rho_{\mathrm{f}} \omega^2\int_\Omega v_{i,j}\sigma_{ij} - \rho_{\mathrm{s}}\omega^2 u_i v_i\idiff\Omega}\\ 
					 &= -\rho_{\mathrm{f}}\omega^2\int_\Gamma p_{\mathrm{inc}} v_i n_i\idiff \Gamma + \int_\Gamma \pderiv{p_{\mathrm{inc}}}{n}q\idiff \Gamma
				\end{align*}}
			\end{minipage}};
		\end{scope}
	\end{tikzpicture}
	\caption[Global matrix for elastic scattering on spherical shell]{\textbf{Elastic scattering on spherical shell:} Location of non zero entries in the sparse global matrix $A$. The polynomial degree is 2 in every parameter directions for both the solid and the fluid except in the radial direction for the fluid (where it is 1). The number of radial basis functions for the infinite elements is $N=3$. The only $h$-refinement has been in the radial direction; there has been inserted 2 knots in the radial direction for both the solid and the fluid.}
	\label{Fig2:spyA}
\end{figure}

In \Cref{Fig2:spyA} we show the results of typing \mcode{spy(A)} in MATLAB (with additional effects added). The function gives an overview of the location of the nonzero entries in the global matrix. This result comes from elastic scattering on a spherical shell, where the mesh is simply a union of two spherical shells; one for the solid and the other for the fluid. In particular, the polynomial degree for the solid is $p_{\mathrm{s}}=q_{\mathrm{s}}=r_{\mathrm{s}}=2$ and for the fluid $p_{\mathrm{f}}=q_{\mathrm{f}}=2$ and $r_{\mathrm{f}}=1$. No refinement is done on the coarsest mesh (cf. \Cref{Fig2:sphereInWater}), except for two knots in the radial direction for both the solid and the fluid (namely $\zeta=\frac{1}{3}$ and $\zeta=\frac{2}{3}$). That is, the number of basis functions in the solid are $n_{\mathrm{s}}=9$, $m_{\mathrm{s}}=5$ and $l_{\mathrm{s}}=5$ (originally 3) and $n_{\mathrm{f}}=9$, $m_{\mathrm{f}}=5$ and $l_{\mathrm{s}}=4$ (originally 3) for the fluid (cf, \Cref{se:sphericalShellNURBSData}). Due to periodicity, some of these basis functions should be considered as the same. For a given set of basis functions in the radial direction we get $n_{\mathrm{s}} m_{\mathrm{s}} = 45$ basis functions in the solid (and correspondingly in the fluid). Due to gluing, this number reduces to 26. The number represent the width of the ``squares'' showing up all over the matrix. Obviously we get $26l_{\mathrm{s}} = 130$ basis functions for each of the spatial components of the solid, such that there is in total 390 degrees of freedom in the solid. Moreover, we see $26l_{\mathrm{f}}=104$ basis functions for the finite element (FE) part of the fluid. As we use $N=3$ basis functions in the radial direction for the infinite elements, we can observe an additional $26(N-1)=52$ basis functions corresponding to the infinite elements (IE). The total number of degrees of freedom for this mesh is thus $390+104+52=546$. Also note that we get $d\cdot 1+1\cdot d = 6$ such ``squares'' in the coupling area (recall that $d=3$ is the number of physical dimensions we use). Without this coupling part, the system becomes decoupled, and one end up solving two separate problems in one go (this is actually a good test for developing the procedure of fluid-structure interaction problems). 

In \Cref{Fig2:spyApermuted} we show another configuration of the indexing of the NURBS basis function in the solid. Here the first three indices corresponds to the $x$, $y$ and $z$ component of the displacement field for the first NURBS basis function. This results in a smaller bandwidth. However, MATLAB uses its own permutation algorithm when a direct solver is applied, so the ordering is not so important.
\tikzsetnextfilename{spyApermuted} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\def\scalingFact{41.4}
		\begin{scope}[y=-1cm,x=1cm]
			\node[anchor=north west,inner sep=0] at (-0.10,-0.12) {\includegraphics[width=0.8425\textwidth]{../../graphics/spyAcuttedPermuted.pdf}};
		    
	
		    \draw (-5/\scalingFact,-5/\scalingFact) -- (-5/\scalingFact, 551/\scalingFact) node[midway, left]{$\vec{A} = $};	   
		    \draw (-5/\scalingFact,-5/\scalingFact) -- (0,-5/\scalingFact);
		    \draw (-5/\scalingFact, 551/\scalingFact) -- (0, 551/\scalingFact);
		    
		    \draw (551/\scalingFact,-5/\scalingFact) -- (551/\scalingFact, 551/\scalingFact);	   
		    \draw (551/\scalingFact,-5/\scalingFact) -- (546/\scalingFact,-5/\scalingFact);
		    \draw (551/\scalingFact, 551/\scalingFact) -- (546/\scalingFact, 551/\scalingFact);
		    
		\end{scope}
	\end{tikzpicture}
	\caption[Global matrix for elastic scattering on spherical shell with permutations]{\textbf{Elastic scattering on spherical shell:} The same global matrix as in \Cref{Fig2:spyA}, but with permutations in the solid part of the matrix to reduce bandwidth.}
	\label{Fig2:spyApermuted}
\end{figure}

\subsection{Computation of backscattered pressure}
Again we loop through the surface elements at $\Gamma$ and use \Cref{Eq2:farfieldFormula} to compute the backscattered pressure. The main difference from the computation of the coupling conditions, is that we here need to compute the derivative. Thus, the full 3D NURBS is needed in order to compute the Jacobian matrix.

If there are many angles to be analyzed, the two loops over these angles should be parallelized. However, if one only consider few angles (for instance the bistatic case when only one pair of $\alpha_s$ and $\beta_s$ is considered), one should take the parallelization over the loop which runs through the surface elements.

==> contents/coordinateSystems.tex <==
\section{Coordinate systems}


\subsection{General 3D coordinate system}
\label{Sec2:general3DcoordinateSystem}
We shall now consider the general 3D coordinate system, which one may reduce to the the cylindrical coordinate system and the spherical coordinate system. Let the coordinate system be defined by
\begin{equation*}
	\vec{r} = \begin{bmatrix}
	x(\xi, \eta, \zeta)\\
	y(\xi, \eta, \zeta)\\
	z(\xi, \eta, \zeta)
\end{bmatrix} :	 \R^3\to\R^3, \quad  \begin{bmatrix}
	\xi\\
	\eta\\
	\zeta
	\end{bmatrix}\mapsto \vec{r}(\xi, \eta, \zeta).
\end{equation*}
We shall frequently use the scaling lengths defined by
\begin{align}
	h_{\upxi} &= \norm{\pderiv{\vec{r}}{\xi}} = \sqrt{\left(\pderiv{x}{\xi}\right)^2+\left(\pderiv{y}{\xi}\right)^2+\left(\pderiv{z}{\xi}\right)^2}\nonumber\\
	h_{\upeta} &= \norm{\pderiv{\vec{r}}{\eta}} = \sqrt{\left(\pderiv{x}{\eta}\right)^2+\left(\pderiv{y}{\eta}\right)^2+\left(\pderiv{z}{\eta}\right)^2}\label{Eq2:ScalingLengths}\\
	h_{\upzeta} &= \norm{\pderiv{\vec{r}}{\zeta}} = \sqrt{\left(\pderiv{x}{\zeta}\right)^2+\left(\pderiv{y}{\zeta}\right)^2+\left(\pderiv{z}{\zeta}\right)^2}.\nonumber
\end{align}
The standard basis vectors in this general coordinate system are then
\begin{equation*}
	\vec{e}_{\upxi} = \frac{1}{h_{\upxi}}\pderiv{\vec{r}}{\xi},\quad\vec{e}_{\upeta} = \frac{1}{h_{\upeta}}\pderiv{\vec{r}}{\eta},\quad\vec{e}_{\upzeta} = \frac{1}{h_{\upzeta}}\pderiv{\vec{r}}{\zeta}.
\end{equation*}
We now want to develop an expression for the nabla operator in terms of these unit vectors. In our coordinate system, the nabla operator is defined by
\begin{equation*}
	\nabla f = \vec{e}_{\upxi} g_{\upxi} +\vec{e}_{\upeta} g_{\upeta} +\vec{e}_{\upzeta} g_{\upzeta}.
\end{equation*}
where $g_{\upxi}$, $g_{\upeta}$ and $g_{\upzeta}$ are functionals of $f$ which are to be determined.

Moreover, the nabla operator satisfy
\begin{equation*}
	\diff f = \nabla f\cdot\diff \vec{r},
\end{equation*}
where (by the chain rule)
\begin{align*}
	\diff \vec{r} &= \pderiv{\vec{r}}{\xi}\diff\xi + \pderiv{\vec{r}}{\eta}\diff\eta + \pderiv{\vec{r}}{\zeta}\diff\zeta\\
	  &= h_{\upxi}\vec{e}_{\upxi} \diff\xi + h_{\upeta}\vec{e}_{\upeta} \diff\eta + h_{\upzeta}\vec{e}_{\upzeta} \diff\zeta.
\end{align*}
Using the chain rule once again, we also have
\begin{equation*}
	\diff f = \pderiv{f}{\xi} \diff\xi + \pderiv{f}{\eta} \diff\eta + \pderiv{f}{\zeta} \diff\zeta.
\end{equation*}
Combining the equations for $\diff f$ we get the relation
\begin{align}
	\pderiv{f}{\xi} \diff\xi + \pderiv{f}{\eta} \diff\eta + \pderiv{f}{\zeta} \diff\zeta &= \left(\vec{e}_{\upxi} g_{\upxi} +\vec{e}_{\upeta} g_{\upeta} +\vec{e}_{\upzeta} g_{\upzeta}\right)\cdot\left(h_{\upxi}\vec{e}_{\upxi} \diff\xi + h_{\upeta}\vec{e}_{\upeta} \diff\eta + h_{\upzeta}\vec{e}_{\upzeta} \diff\zeta\right)\\
	&=h_{\upxi}(g_{\upxi} +  \vec{e}_{\upxi}\cdot \vec{e}_{\upeta} g_{\upeta} +  \vec{e}_{\upxi}\cdot\vec{e}_{\upzeta} g_{\upzeta})\diff\xi\\
	&+h_{\upeta}(\vec{e}_{\upxi}\cdot \vec{e}_{\upeta} g_{\upxi} +  g_{\upeta} +  \vec{e}_{\upeta}\cdot\vec{e}_{\upzeta} g_{\upzeta})\diff\eta\\
	&+h_{\upzeta}(\vec{e}_{\upxi}\cdot \vec{e}_{\upzeta} g_{\upxi} +  \vec{e}_{\upeta}\cdot\vec{e}_{\upzeta} g_{\upeta}+  g_{\upzeta})\diff\zeta
\end{align}
where we have used the fact that $\vec{e}_{\upxi}\cdot\vec{e}_{\upxi}= 1$, $\vec{e}_{\upeta}\cdot\vec{e}_{\upeta}= 1$ and $\vec{e}_{\upzeta}\cdot\vec{e}_{\upzeta}= 1$. As the coefficients in front of $\diff\xi$, $\diff\eta$ and $\diff\zeta$ must be the same on both side, we get a system of equations given by
\begin{equation}\label{Eq2:systemNablaOperator}
\begin{alignedat}{4}
	 g_{\upxi} & {}+{} &  \vec{e}_{\upxi}\cdot \vec{e}_{\upeta} g_{\upeta} & {}+{} &  \vec{e}_{\upxi}\cdot\vec{e}_{\upzeta} g_{\upzeta} &= \frac{1}{h_{\upxi}}\pderiv{f}{\xi}\\
	\vec{e}_{\upxi}\cdot \vec{e}_{\upeta} g_{\upxi} & {}+{} &  g_{\upeta} & {}+{} & \vec{e}_{\upeta}\cdot\vec{e}_{\upzeta} g_{\upzeta} &= \frac{1}{h_{\upeta}}\pderiv{f}{\eta}\\
	\vec{e}_{\upxi}\cdot \vec{e}_{\upzeta} g_{\upxi} & {}+{} & \vec{e}_{\upeta}\cdot\vec{e}_{\upzeta} g_{\upeta} & {}+{} & g_{\upzeta} &= \frac{1}{h_{\upzeta}}\pderiv{f}{\zeta}.
\end{alignedat}
\end{equation}
Introducing the notation
\begin{equation*}
	E_{\upxi\upeta} = \vec{e}_{\upxi}\cdot\vec{e}_{\upeta},\quad E_{\upxi\upzeta} = \vec{e}_{\upxi}\cdot\vec{e}_{\upzeta},\quad E_{\upeta\upzeta} = \vec{e}_{\upeta}\cdot\vec{e}_{\upzeta}
\end{equation*}
the system in \Cref{Eq2:systemNablaOperator} is given by can be written as
\begin{equation*}
	\begin{bmatrix}
		1 & E_{\upxi\upeta} & E_{\upxi\upzeta}\\
		E_{\upxi\upeta} & 1 & E_{\upeta\upzeta}\\
		E_{\upxi\upzeta} & E_{\upeta\upzeta} & 1\\
	\end{bmatrix}\begin{bmatrix}
		g_{\upxi}\\
		g_{\upeta}\\
		g_{\upzeta}
	\end{bmatrix} = \begin{bmatrix}
	\frac{1}{h_{\upxi}} \pderiv{f}{\xi}\\
	\frac{1}{h_{\upeta}} \pderiv{f}{\eta}\\
	\frac{1}{h_{\upzeta}} \pderiv{f}{\zeta}\end{bmatrix}.
\end{equation*}
As the determinant of this system of equation is given by
\begin{equation*}
	\nabla^2 = 1 - E_{\upxi\upeta}^2 - E_{\upxi\upzeta}^2 - E_{\upeta\upzeta}^2 + 2E_{\upxi\upeta}E_{\upxi\upzeta}E_{\upeta\upzeta}
\end{equation*}
we may write the solution as
\begin{align*}
\begin{bmatrix}
	g_{\upxi}\\
	g_{\upeta}\\
	g_{\upzeta}
\end{bmatrix} = \begin{bmatrix}
	a_{11} & a_{12} & a_{13}\\
	a_{21} & a_{22} & a_{23}\\
	a_{31} & a_{32} & a_{33}
\end{bmatrix} \begin{bmatrix}
	\frac{1}{h_{\upxi}} \pderiv{f}{\xi}\\
	\frac{1}{h_{\upeta}} \pderiv{f}{\eta}\\
	\frac{1}{h_{\upzeta}} \pderiv{f}{\zeta}
\end{bmatrix}
\end{align*}
where the coefficients $a_{ij}$ are given by the symmetric matrix
\begin{equation*}
	[a_{ij}] = \frac{1}{\nabla^2}\begin{bmatrix}
		1-E_{\upeta\upzeta}^2 & E_{\upxi\upzeta}E_{\upeta\upzeta} - E_{\upxi\upeta}  &  E_{\upxi\upeta}E_{\upeta\upzeta} - E_{\upxi\upzeta}\\
		E_{\upxi\upzeta}E_{\upeta\upzeta} - E_{\upxi\upeta} & 1-E_{\upxi\upzeta}^2 & E_{\upxi\upeta}E_{\upxi\upzeta} - E_{\upeta\upzeta}\\
		E_{\upxi\upeta}E_{\upeta\upzeta} - E_{\upxi\upzeta} & E_{\upxi\upeta}E_{\upxi\upzeta} - E_{\upeta\upzeta} & 1-E_{\upxi\upeta}^2
	\end{bmatrix}
\end{equation*}
Let's verify this calculation by finding the nabla operator in the spherical coordinate system. Letting $\xi$ correspond to the azimuthal angle $\phi$, $\eta$ the polar angle $\vartheta$ and $\zeta$ the radial direction $r$, we have the relations
\begin{align*}
	x &= \zeta\sin\eta\cos\xi\\
	y &= \zeta\sin\eta\sin\xi\\
	z &= \zeta\cos\eta.
\end{align*}
As the spherical coordinate system is an orthogonal coordinate system, we get $E_{\upxi\upeta}=0$, $E_{\upxi\upzeta}=0$ and $E_{\upeta\upzeta}=0$. Thus,
\begin{equation*}
	g_{\upxi} = \frac{1}{h_{\upxi}}\pderiv{f}{\xi},\quad g_{\upeta} =\frac{1}{h_{\upeta}}\pderiv{f}{\eta},\quad g_{\upzeta} =\frac{1}{h_{\upzeta}}\pderiv{f}{\zeta}.
\end{equation*}
By computation, we find
\begin{equation*}
	h_{\upxi} = \zeta\sin\eta,\quad h_{\upeta} = \zeta,\quad h_{\upzeta} = 1.
\end{equation*}
Thus,
\begin{align*}
	\nabla f &= \frac{1}{\zeta\sin\eta}\pderiv{f}{\xi}\vec{e}_{\upxi} + \frac{1}{\zeta}\pderiv{f}{\eta}\vec{e}_{\upeta} + \pderiv{f}{\zeta}\vec{e}_{\upzeta}\\
	&= \pderiv{f}{r}\vec{e}_{\mathrm{r}} + \frac{1}{r}\pderiv{f}{\vartheta}\vec{e}_{\upvartheta} + \frac{1}{r\sin\vartheta}\pderiv{f}{\phi}\vec{e}_{\upphi},
\end{align*}
which is the familiar expression for the nabla operator in spherical coordinates.

\subsubsection{Extended NURBS coordinate system}
\label{subsubsubsec:infElementsOnGeneralizedCoordSyst}
In this section we shall explore the possibility to have a more general coordinate system for the infinite elements. All though the prolate spheroidal coordinate system helps reduce the number of elements needed to circumference a long obstacle compared to the spherical coordinate system, it is still not ideal with respect to this problem. It is possible to define a coordinate system such that we get
\begin{equation*}
	\inf_{\vec{x}\in\Gamma} \| \vec{x} - \vec{y}_0 \| = \inf_{\vec{y}\in\Gamma_{\mathrm{a}}} \| \vec{x}_0-\vec{y}\|\quad \forall\vec{x}_0\in\Gamma,\quad\text{and}\quad\forall\vec{y}_0\in\Gamma_{\mathrm{a}}.
\end{equation*}
That is, we can have the surface $\Gamma_{\mathrm{a}}$ at a constant distance from the surface $\Gamma$ (if $\Gamma$ is convex\footnote{If this is not the case, an intermediate convex surface must be inserted between $\Gamma$ and $\Gamma_{\mathrm{a}}$ in the NURBS patch.}). However, is it possible to define a infinite element formulation on such a coordinate system? The most intuitive coordinate system would satisfy the property that for all points on $\Gamma_{\mathrm{a}}$ the normal vector is parallel to the ``radial'' unit vector for this coordinate system. This would however make the integration in the weak formulation hard as the nabla operator would not be separable, and we may no longer integrate analytically in the ``radial'' direction. In the following we shall consider another option which results in a separable nabla operator.

Let's build upon the theory developed in \Cref{Sec2:general3DcoordinateSystem} where we shall assume that the NURBS parametrization at hand has a ``radial'' parameter $\zeta$, such that $\xi$ and $\eta$ corresponds to ``angular'' parameters. This will typically be the case when considering shell objects, where $\zeta$ will run through the thickness of the elastic material. We know that at any given value $\bar{\zeta}$ the NURBS solid in 3D reduces to a NURBS surface in 3D. This is in particular true for $\bar{\zeta} = 1$, which will be our artificial boundary $\Gamma_{\mathrm{a}}$. We shall assume, without loss of generality, that the NURBS surface $\Gamma_{\mathrm{a}}$ fully encloses the origin. Finally, we assume the surface $\Gamma_{\mathrm{a}}$ to be a convex surface. We now want to extend the NURBS parametrization also for $\zeta > 1$. In particular we define (for $\zeta>1$)
\begin{equation*}
	\vec{r} = \begin{bmatrix}
	x(\xi, \eta, \zeta)\\
	y(\xi, \eta, \zeta)\\
	z(\xi, \eta, \zeta)
\end{bmatrix} :	 \R^3\to\R^3, \quad  \begin{bmatrix}
	\xi\\
	\eta\\
	\zeta
	\end{bmatrix}\mapsto s(\zeta)\bar{\vec{r}}(\xi, \eta).
\end{equation*}
where $\bar{\vec{r}}$ is the NURBS 3D surface at $\zeta = 1$ and the \textit{scaling function} $s$ is strictly increasing and satisfies $s(1) = 1$. Thus, for any $\zeta > 1$ we simply get a scaled version of $\Gamma_{\mathrm{a}}$ from the origin with the scaling factor $s(\zeta)$.

Continuing on the notation from \Cref{Sec2:general3DcoordinateSystem}, our new coordinate system has the following nice property
\begin{equation*}
	h_{\upxi} = s(\zeta)\norm{\pderiv{\bar{\vec{r}}}{\xi}},\quad h_{\upeta} = s(\zeta)\norm{\pderiv{\bar{\vec{r}}}{\eta}},\quad h_{\upzeta} = s'(\zeta)\norm{\bar{\vec{r}}}.
\end{equation*}
From this we observe that the unit vectors $\vec{e}_{\upxi}$, $\vec{e}_{\upeta}$ and $\vec{e}_{\upzeta}$ are all independent of $\zeta$. Moreover, $E_{\upxi\upeta}$, $E_{\upxi\upzeta}$ and $E_{\upeta\upzeta}$ (and thus also the determinant $\nabla^2$) will also be independent of $\zeta$. The resulting nabla operator will then be separable, which we will take advantage of. In this context we define 
\begin{equation*}
	\bar{h}_{\upxi} = \norm{\pderiv{\bar{\vec{r}}}{\xi}}, \quad \bar{h}_{\upeta} = \norm{\pderiv{\bar{\vec{r}}}{\eta}},\quad \bar{h}_{\upzeta} = \norm{\bar{\vec{r}}}
\end{equation*}
such that $h_{\upxi} = s(\zeta)\bar{h}_{\upxi}$, $h_{\upeta} = s(\zeta)\bar{h}_{\upeta}$, $h_{\upzeta} = s'(\zeta)\bar{h}_{\upzeta}$. We may now easy see that the nabla operator is separable as it is now given by (for $\zeta>1$)
\begin{align*}
	\nabla &= \left(\frac{a_{11}}{s(\zeta)\bar{h}_{\upxi}}\pderiv{}{\xi} + \frac{a_{12}}{s(\zeta)\bar{h}_{\upeta}}\pderiv{}{\eta} + \frac{a_{13}}{s'(\zeta)\bar{h}_{\upzeta}}\pderiv{}{\zeta}\right)\vec{e}_{\upxi}\\
	 &+\left(\frac{a_{21}}{s(\zeta)\bar{h}_{\upxi}}\pderiv{}{\xi} + \frac{a_{22}}{s(\zeta)\bar{h}_{\upeta}}\pderiv{}{\eta} + \frac{a_{23}}{s'(\zeta)\bar{h}_{\upzeta}}\pderiv{}{\zeta}\right)\vec{e}_{\upeta}\\
	 &+ \left(\frac{a_{31}}{s(\zeta)\bar{h}_{\upxi}}\pderiv{}{\xi} + \frac{a_{32}}{s(\zeta)\bar{h}_{\upeta}}\pderiv{}{\eta} + \frac{a_{33}}{s'(\zeta)\bar{h}_{\upzeta}}\pderiv{}{\zeta}\right)\vec{e}_{\upzeta}\\
	 &= \frac{1}{s(\zeta) \bar{h}_{\upxi}}\left(a_{11}\vec{e}_{\upxi} + a_{21} \vec{e}_{\upeta} + a_{31}\vec{e}_{\upzeta}\right)\pderiv{}{\xi}\\
	 &+\frac{1}{s(\zeta)\bar{h}_{\upeta}}\left(a_{12}\vec{e}_{\upxi} + a_{22} \vec{e}_{\upeta} + a_{32}\vec{e}_{\upzeta}\right)\pderiv{}{\eta}\\
	 &+\frac{1}{s'(\zeta)\bar{h}_{\upzeta}}\left(a_{13}\vec{e}_{\upxi} + a_{23} \vec{e}_{\upeta} + a_{33}\vec{e}_{\upzeta}\right)\pderiv{}{\zeta}\\
	 &= \frac{1}{s(\zeta)}\nabla_S + \frac{1}{s'(\zeta)}\vec{a}\pderiv{}{\zeta}
\end{align*}
where
\begin{equation*}
	\nabla_S = \frac{1}{\bar{h}_{\upxi}}\left(a_{11}\vec{e}_{\upxi} + a_{21} \vec{e}_{\upeta} + a_{31}\vec{e}_{\upzeta}\right)\pderiv{}{\xi}+\frac{1}{\bar{h}_{\upeta}}\left(a_{12}\vec{e}_{\upxi} + a_{22} \vec{e}_{\upeta} + a_{32}\vec{e}_{\upzeta}\right)\pderiv{}{\eta}
\end{equation*}
and
\begin{equation*}
	\vec{a} = \frac{1}{\bar{h}_{\upzeta}}\left(a_{13}\vec{e}_{\upxi} + a_{23} \vec{e}_{\upeta} + a_{33}\vec{e}_{\upzeta}\right).
\end{equation*}
We note that (for any normal vector $\vec{n}$ on the surface $\Gamma_{\mathrm{a}}$) we have
\begin{equation}\label{Eq2:anRel}
	\vec{a}\cdot\vec{n} = \frac{a_{33}}{\bar{h}_{\upzeta}}\vec{e}_{\upzeta}\cdot\vec{n}.
\end{equation}
and
\begin{equation*}
	\| \vec{a} \| = \frac{1}{\bar{h}_{\upzeta}}\sqrt{a_{33}}.
\end{equation*}
Moreover, we note that in the case $\vec{e}_{\upxi} \perp \vec{e}_{\upzeta}$ and $\vec{e}_{\upeta} \perp \vec{e}_{\upzeta}$ (for example when $\Gamma_{\mathrm{a}}$ is a sphere), this vector reduces to $\vec{a}=a_{33}\vec{e}_{\upzeta}/\bar{h}_{\upzeta}$.

Using the expression for the Jacobian matrix in \Cref{Eq2:NURBSjacobian} we get
\begin{equation*}
	|\mathrm{det}(\vec{J})| = [s(\zeta)]^2s'(\zeta)\left\|\pderiv{\bar{\vec{r}}}{\xi}\times\pderiv{\bar{\vec{r}}}{\eta} \right\|\bar{h}_{\upzeta} \vec{n}\cdot \vec{e}_{\upzeta}.
\end{equation*}
We may therefore write
\begin{equation*}
	\diff\Omega = [s(\zeta)]^2s'(\zeta)\bar{h}_{\upzeta}\diff S\diff\zeta
\end{equation*}
where
\begin{equation*}
	\diff S = \left\|\pderiv{\bar{\vec{r}}}{\xi}\times\pderiv{\bar{\vec{r}}}{\eta} \right\|\vec{n}\cdot \vec{e}_{\upzeta}\diff\xi\diff\eta.
\end{equation*}
We also note that a surface where $\zeta=\textrm{const}$, the surface element is 
\begin{equation*}
	 \diff\Gamma = [s(\zeta)]^2 \left\|\pderiv{\bar{\vec{r}}}{\xi}\times\pderiv{\bar{\vec{r}}}{\eta} \right\| \diff\xi\diff\eta = \frac{[s(\zeta)]^2}{\vec{n}\cdot\vec{e}_{\upzeta}}\diff S.
\end{equation*}
Hence, both $\nabla_S$ and $\diff S$ are independent of $\zeta$ which enables us to separate the integral in the weak form. 

\subsubsection{Weak formulation for infinite elements}
We shall use the most natural choice of the scaling function, namely $s(\zeta) = \zeta$. This simplifications result in the following
\begin{equation*}
	\nabla = \frac{1}{\zeta}\nabla_S + \frac{\vec{e}_{\upzeta}}{r_{\mathrm{a}}}\pderiv{}{\zeta}	,\quad\text{where}\quad\nabla_S = \frac{\vec{e}_{\upxi}}{\bar{h}_{\upxi}}\pderiv{}{\xi} + \frac{\vec{e}_{\upeta}}{\bar{h}_{\upeta}}\pderiv{}{\eta}
\end{equation*}
and
\begin{equation*}
	\diff\Omega = \zeta^2r_{\mathrm{a}}\diff S,\qquad \diff\Gamma = \zeta^2\diff S,\quad\text{where}\quad  \diff S = \left\|\pderiv{\bar{\vec{r}}}{\xi}\times\pderiv{\bar{\vec{r}}}{\eta} \right\|\diff\xi\diff\eta.	
\end{equation*}
In order to use the extended NURBS coordinate system, we have to modify the ``radial shape functions'' which Ihlenburg presents on the form
\begin{equation*}
	\phi_n(r) = \frac{\euler^{\imag k r}}{r^n},\quad n = 1,\dots,N.
\end{equation*}
We can not simply replace $r$ with $\zeta$ here, as the latter is dimensionless and invariant of the size of the object. Note that the wave number $k$ has dimension $\unit{m}^{-1}$, so we must scale $\zeta$ by a parameter with dimension $\unit{m}$. To get correspondence with these functions in spherical coordinate system, we have to scale with the ``radius'' of the artificial boundary, $r_{\mathrm{a}}$. This quantity must be independent of the angular parameters in order to make separable functions (the average distance from the origin to the surface $\Gamma_{\mathrm{a}}$ may be the most natural choice). That is,
\begin{equation}\label{Eq2:radialShapeFunctions}
	\tilde{\phi}(\zeta) = \frac{\euler^{\imag r_{\mathrm{a}} k \zeta}}{(r_{\mathrm{a}}\zeta )^n},\quad n = 1,\dots,N.	
\end{equation}

The weak formulating takes the form: For all $v\in V_1$, find $u_h^N\in V_1$ such that
\begin{equation*}
	b_{uc}(u_h^N, v) = \langle g,v\rangle_\Gamma,
\end{equation*}
where
\begin{align}\label{Eq2:infElemntBilinearForm3}
	b_{uc}(v,u) &= \lim_{\gamma\to\infty}\left(\int_{\Omega_\gamma} (\nabla v \nabla u - k^2 vu)\idiff\Omega - \int_{S_\gamma} v\partial_n u\idiff\Gamma\right),\\
	\langle g,v\rangle_\Gamma &= \int_\Gamma gv\idiff\Gamma.\nonumber
\end{align}
Here, $S_\gamma$ is the surface where $\zeta = \gamma$ and we can then recover the full domain by letting $\gamma\to\infty$. For the domain outside the artificial boundary ($\zeta = 1$) we consider trial and test functions of the form
\begin{equation*}
	u = \frac{\euler^{\imag r_{\mathrm{a}}k\zeta}}{\zeta^m}f_m(\xi,\eta),\quad v = \frac{\euler^{\imag r_{\mathrm{a}} k\zeta}}{\zeta^n}f_n(\xi,\eta),
\end{equation*}
where we have baked the constants $r_{\mathrm{a}}^n$ and $r_{\mathrm{a}}^m$ from the radial shape functions in \Cref{Eq2:radialShapeFunctions}, into $f_n$ and $f_m$ respectively. As these functions are separable, we get
\begin{align*}
	\nabla v\cdot\nabla u &= \left(\frac{1}{\zeta}\nabla_S v + \frac{\vec{e}_{\upzeta}}{r_{\mathrm{a}}}\pderiv{v}{\zeta}\right)\cdot\left(\frac{1}{\zeta}\nabla_S u + \frac{\vec{e}_{\upzeta}}{r_{\mathrm{a}}}\pderiv{u}{\zeta}\right)\\
	&= \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n+2}}\nabla_S f_m\cdot\nabla_S f_n + \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{r_{\mathrm{a}}^2\zeta^{m+n}}\left(\imag r_{\mathrm{a}} k - \frac{n}{\zeta}\right)\left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right)f_m f_n.
\end{align*}
and
\begin{align*}
	v\partial_n u &= v\nabla u\cdot\vec{n} = v\left(\frac{1}{\zeta}\nabla_S u + \frac{\vec{e}_{\upzeta}}{r_{\mathrm{a}}}\pderiv{u}{\zeta}\right)\cdot\vec{e}_{\upzeta} = \frac{v}{r_{\mathrm{a}}}\pderiv{u}{\zeta}\\
	&= \left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right) \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{r_{\mathrm{a}}\zeta^{m+n}}f_n f_m.
\end{align*}
Consider first the boundary integral at $S_\gamma$
\begin{align*}
	\int_{S_\gamma} v\partial_n u\idiff\Gamma &= \int_{S_\gamma}\left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right) \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{r_{\mathrm{a}}\zeta^{m+n}}f_n f_m\zeta^2\idiff S\\
	&= \left(\imag r_{\mathrm{a}} k - \frac{m}{\gamma}\right) \frac{\euler^{2\imag r_{\mathrm{a}} k\gamma}}{r_{\mathrm{a}} \gamma^{m+n-2}}\int_{\Gamma_{\mathrm{a}}}f_n f_m\idiff S
\end{align*}
As $m+n>1$ all terms of order $\mathcal{O}(\gamma^{-(m+n-1)})$ vanish in the limit $\gamma\to\infty$, such that the integral reduces to
\begin{equation*}
	\int_{S_\gamma} v\partial_n u\idiff\Gamma =  \frac{\imag k\euler^{2\imag r_{\mathrm{a}} k\gamma}}{\gamma^{m+n-2}}\int_{\Gamma_{\mathrm{a}}}f_n f_m\idiff S
\end{equation*}
Combining all of this into \Cref{Eq2:infElemntBilinearForm3} yields
\begin{align*}
	b_{uc}(v,u) = \lim_{\gamma\to\infty}&\left\{J_{mn}\int_1^\gamma \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\idiff\zeta\right.\\
	&\left. + I_{mn}\int_1^\gamma\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\left[-2(r_{\mathrm{a}} k\zeta)^2 - \imag r_{\mathrm{a}} k\zeta(n + m) + nm\right]\idiff\zeta \right.\\
	&\left. - I_{mn}\frac{\imag r_{\mathrm{a}} k\euler^{2\imag r_{\mathrm{a}} k\gamma}}{\gamma^{m+n-2}}\right\}
\end{align*}
where
\begin{equation}\label{Eq2:infiniteElementsSurfaceIntegrals3}
	I_{mn} = \int_{\Gamma_{\mathrm{a}}} \frac{1}{r_{\mathrm{a}}} f_m f_n\idiff S,\qquad J_{mn} = \int_{\Gamma_{\mathrm{a}}} r_{\mathrm{a}} \nabla_S f_m \cdot\nabla_S f_n\idiff S
\end{equation}
Thus, we get the same radial integrals as before. It remains to consider the case $n=m=1$. As
\begin{align*}
	L &= \lim_{\gamma\to\infty}\left[-2(r_{\mathrm{a}} k)^2 I_{11}\int_1^\gamma \euler^{2\imag r_{\mathrm{a}} k \zeta}\idiff\zeta - \imag r_{\mathrm{a}} k I_{11}\euler^{2\imag r_{\mathrm{a}} k \gamma} \right]\\
	 &= \lim_{\gamma\to\infty}\left[\imag r_{\mathrm{a}} k  I_{11} \right(\euler^{2\imag r_{\mathrm{a}} k \gamma} - \euler^{2\imag r_{\mathrm{a}} k}\left) - \imag r_{\mathrm{a}} k I_{11} \euler^{2\imag r_{\mathrm{a}} k \gamma}\right]\\
	 &= - \imag r_{\mathrm{a}} k I_{11} \euler^{2\imag r_{\mathrm{a}} k}.
\end{align*}
we get the bilinear form
\begin{align*}
	b_{uc}(v,u) &= J_{mn}E_{m+n}+ I_{mn}[-2(r_{\mathrm{a}} k)^2E_{m+n-2} - \imag r_{\mathrm{a}} k(n+m)E_{m+n-1} + nm E_{m+n}]
\end{align*}
where $E_{n} = E_{n}(-2\imag r_{\mathrm{a}} k)$. And for the special case $n=m=1$ we get
\begin{align*}
	b_{uc}(v,u) &= J_{11}E_{2} + I_{11}[- 2\imag r_{\mathrm{a}} kE_{1} + E_{2}- \imag r_{\mathrm{a}} k \euler^{2\imag r_{\mathrm{a}} k}] 
\end{align*}
Let
\begin{equation*}
	f_n = \sum_{A\in\vec{\eta}_{\mathrm{a}}} R_A c_{nA},\quad f_m = \sum_{B\in\vec{\eta}_{\mathrm{a}}} R_B d_{mB}
\end{equation*}
where $\vec{\eta}_{\mathrm{a}}$ is the set containing the indices of all the basis functions that are non-zero on $\Gamma_{\mathrm{a}}$. Using the bilinearity of $b_{uc}$ we obtain (for $\zeta > 1$)
\begin{equation*}
	\sum_{A\in\vec{\eta}_{\mathrm{a}}}\sum_{n=1}^N c_{nA}\left(\sum_{B\in\vec{\eta}_{\mathrm{a}}}\sum_{m=1}^N d_{nA} b_{uc}(R_A, R_B)\right) = 0.
\end{equation*}
As the surface integrals in \Cref{Eq2:infiniteElementsSurfaceIntegrals3} will now be independent of the indices $m$ and $n$ we now get (for $n+m>1$)
\begin{align*}
	b_{uc}(R_A,R_B) &= J_{AB}E_{m+n}+ I_{AB}[-2(r_{\mathrm{a}} k)^2E_{m+n-2} - \imag r_{\mathrm{a}} k(n+m)E_{m+n-1} + nm E_{m+n}]
\end{align*}
and in the case $n=m=1$
\begin{align*}
	b_{uc}(R_A,R_B) &= J_{AB}E_{2} + I_{AB}[- 2\imag r_{\mathrm{a}} kE_{1} + E_{2}- \imag r_{\mathrm{a}} k \euler^{2\imag r_{\mathrm{a}} k}] 
\end{align*}
where we have redefined the surface integral notations to be
\begin{equation*}
	I_{AB} = \int_{\Gamma_{\mathrm{a}}} \frac{1}{r_{\mathrm{a}}} R_A R_B\idiff S,\qquad J_{AB} = \int_{\Gamma_{\mathrm{a}}} r_{\mathrm{a}} \nabla_S R_A \cdot\nabla_S R_B\idiff S
\end{equation*}
This formulation has proven to work for a sphere when the ``radius'' $r_{\mathrm{a}}$ for the artificial boundary is constant. In~\cite{Burnett1994atd} Burnett writes that the scattered pressure field exterior to a spherical $\Gamma_{\mathrm{a}}$ may be written as
\begin{equation*}
	p = \frac{\euler^{\imag kr}}{r}\sum_{n=0}^\infty \frac{F_n(\vartheta,\phi; k)}{r^n}
\end{equation*}
where we have adjusted the sign in the exponential function to match the convention in~\cite{Ihlenburg1998fea} and this thesis. It has been proven that this series has nice convergence properties and the functions $F_n(\vartheta,\phi;k)$ for $n>0$ may be determined by the recursive relation
\begin{equation*}
	2\imag knF_n = \left[n(n-1) + \frac{1}{\sin\vartheta}\pderiv{}{\vartheta}\left(\sin\vartheta\pderiv{}{\vartheta}\right) + \frac{1}{\sin^2\vartheta}\pderiv[2]{}{\phi}\right]F_{n-1}.
\end{equation*}
Here $F_0$ is simply the radiation pattern which in this thesis has the name $F_k$.

Correspondingly, in the prolate spheroidal coordinate system the series
\begin{equation*}
	p = \frac{\euler^{\imag kr}}{r}\sum_{n=0}^\infty \frac{G_n(\vartheta,\phi; k)}{r^n}
\end{equation*}
also converges absolutely and uniformly for any point outside $\Gamma_{\mathrm{a}}$ with a six-term recursion formula for the functions $G_n(\vartheta,\phi; k)$.

To prove the convergence of such series for the coordinate system discussed in this section is outside the scope of this thesis. Due to the lacking mathematical foundation of this infinite element formulation and the time constraint of the thesis, this formulation was not analyzed further in this thesis.

The motivation of introducing the extended NURBS coordinate system is to be able to control the artificial boundary $\Gamma_{\mathrm{a}}$. This allows us to control the size of the fluid domain which would in turn enable us to reduce redundant fluid elements. Ihlenburg uses a prolate spheroid as the artificial boundary around his ``Mock shell'' (depicted in \Cref{Fig2:mockShell}) in~\cite{Ihlenburg1998fea}. As the ``Mock shell'' is a convex surface, one could have a uniform thickness of the fluid around the shell by the extended NURBS coordinate system, and thus reducing the fluid computational domain to an ideal size. 
\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{../../graphics/mockShell}
	\caption[The mock shell]{The mock shell.}
	\label{Fig2:mockShell}
\end{figure}
%
%We shall derive the weak formulation with the most natural choice of the scaling function, namely $s(\zeta) = \zeta$. The weak formulating takes the form: For all $v\in V_1$, find $u_h^N\in V_1$ such that
%\begin{equation*}
%	b_{uc}(u_h^N, v) = \langle g,v\rangle_\Gamma,
%\end{equation*}
%where
%\begin{align}\label{Eq2:infElemntBilinearForm5}
%	b_{uc}(v,u) &= \lim_{\gamma\to\infty}\left(\int_{\Omega_\gamma} (\nabla v \nabla u - k^2 vu)\idiff\Omega - \int_{S_\gamma} v\partial_n u\idiff\Gamma\right),\\
%	\langle g,v\rangle_\Gamma &= \int_\Gamma gv\idiff\Gamma.
%\end{align}
%Here, $S_\gamma$ is the surface where $\zeta = \gamma$ and we can then recover the full domain by letting $\gamma\to\infty$ (which is again dependent on the origin to be placed inside of $\Gamma_{\mathrm{a}}$). For the domain outside the artificial boundary ($\zeta = 1$) we consider trial and test functions of the form
%\begin{equation*}
%	u = \frac{\euler^{\imag r_{\mathrm{a}}k\zeta}}{\zeta^m}\frac{f_m}{r_{\mathrm{a}}^m},\quad v = \frac{\euler^{\imag r_{\mathrm{a}} k\zeta}}{\zeta^n}\frac{f_n}{r_{\mathrm{a}}^n}.
%\end{equation*}
%It is important that these functions are separable. This is obviously the case if $r_{\mathrm{a}}$ is constant, which is the case if $\Gamma_{\mathrm{a}}$ is a sphere. However, for more complex geometries, $r_{\mathrm{a}}$ will depend on the parameters $\xi$ and $\eta$. In order to have separable functions one must then create a series expansion of the exponential function
%\begin{equation*}
%	\euler^{\imag k r_{\mathrm{a}}\zeta} = \sum_{j=1}^\infty \frac{(\imag k r_{\mathrm{a}}\zeta)^j}{j!}
%\end{equation*}
%and take the analytic integration term wise. In the following we will only consider the simple case of $\Gamma_{\mathrm{a}}$ being a sphere (with arbitrary radius). In the general case we have,
%\begin{align*}
%	\nabla v\cdot\nabla u &= \left(\frac{1}{\zeta}\nabla_S v + \vec{a}\pderiv{v}{\zeta}\right)\cdot\left(\frac{1}{\zeta}\nabla_S u + \vec{a}\pderiv{u}{\zeta}\right)\\
%	&= \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n+2}}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\nabla_S \left(\frac{f_n}{r_{\mathrm{a}}^n}\right) +\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n+1}}\left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right)\frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\nabla_S \left(\frac{f_n}{r_{\mathrm{a}}^n}\right)\\
%	&+ \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n+1}}\left(\imag k - \frac{n}{\zeta}\right)\frac{f_n}{r_{\mathrm{a}}^n}\vec{a}\cdot\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) + \norm{\vec{a}}^2\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\left(\imag r_{\mathrm{a}} k - \frac{n}{\zeta}\right)\left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right)\frac{f_m}{r_{\mathrm{a}}^m} \frac{f_n}{r_{\mathrm{a}}^n}.
%\end{align*}
%and
%\begin{align*}
%	v\partial_n u &= v\nabla u\cdot\vec{n} = v\left(\frac{1}{\zeta}\nabla_S u + \vec{a}\pderiv{u}{\zeta}\right)\cdot\vec{n} = \frac{1}{\zeta}v\nabla_S u\cdot\vec{n} + v\pderiv{u}{\zeta}\vec{a}\cdot\vec{n}\\
%	&= \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n+1}}\frac{f_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n} + \left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right) \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\frac{f_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\vec{n}.
%\end{align*}
%Consider first the boundary integral at $S_\gamma$
%\begin{align*}
%	\int_{S_\gamma} v\partial_n u\idiff\Gamma &= \int_{\Gamma_{\mathrm{a}}}\frac{\euler^{2\imag k R}}{R^{m+n+1}}\frac{f_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n} R^2 \kappa\idiff S + \int_{\Gamma_{\mathrm{a}}} \left(\imag r_{\mathrm{a}} k - \frac{m}{R}\right) \frac{\euler^{2\imag k R}}{R^{m+n}}\frac{f_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m} \vec{a}\cdot\vec{n}R^2\kappa\idiff S\\
%	&= \frac{\euler^{2\imag k R}}{R^{m+n-1}}\int_{\Gamma_{\mathrm{a}}}\frac{f_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n}\kappa\idiff S + \frac{\euler^{2\imag k R}}{R^{m+n-2}}\left(\imag r_{\mathrm{a}} k - \frac{m}{R}\right)\int_{\Gamma_{\mathrm{a}}}  \frac{f_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\vec{n}\kappa\idiff S
%\end{align*}
%As $m+n>1$ all terms of order $\mathcal{O}(\gamma^{-(m+n-1)})$ vanish in the limit $\gamma\to\infty$, such that the integral reduces to
%\begin{equation*}
%	\int_{S_\gamma} v\partial_n u\idiff\Gamma = \imag k\frac{\euler^{2\imag k R}}{R^{m+n-2}}\int_{\Gamma_{\mathrm{a}}} \frac{a_{33}}{\bar{h}_{\upzeta}^2} \frac{f_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\idiff S
%\end{equation*}
%where we have used \Cref{Eq2:anRel} and \Cref{Eq2:kapparel}.
%
%Combining all of this into \Cref{Eq2:infElemntBilinearForm5} yields
%\begin{align*}
%	b_{uc}(v,u) = \lim_{\gamma\to\infty}&\left\{J_{mn}\int_1^\gamma \frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\idiff\zeta + P_{mn}\int_1^\gamma\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n-1}}\left(\imag r_{\mathrm{a}} k - \frac{m}{\zeta}\right)\idiff\zeta\right.\\
%	 &\left.+ Q_{mn}\int_1^\gamma\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n-1}}\left(\imag r_{\mathrm{a}} k - \frac{n}{\zeta}\right)\idiff\zeta \right.\\
%	&\left. + I_{mn}'\int_1^\gamma\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}\left[-(r_{\mathrm{a}} k\zeta)^2 - \imag r_{\mathrm{a}} k\zeta(n + m) + nm\right]\idiff\zeta \right.\\
%	&\left.- I_{mn}\int_1^\gamma\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^{m+n}}(k\zeta)^2\idiff\zeta - \imag r_{\mathrm{a}} kI_{mn}'\frac{\euler^{2\imag r_{\mathrm{a}} kR}}{R^{m+n-2}}\right\}
%\end{align*}
%where
%\begin{equation}\label{Eq2:infiniteElementsSurfaceIntegrals5}
%\begin{alignedat}{2}
%	& I_{mn} = \int_{\Gamma_{\mathrm{a}}} \frac{f_m}{r_{\mathrm{a}}^m} \frac{f_n}{r_{\mathrm{a}}^n}\idiff S,\qquad\qquad && I_{mn}' = \int_{\Gamma_{\mathrm{a}}} \frac{a_{33}}{\bar{h}_{\upzeta}^2} \frac{f_m}{r_{\mathrm{a}}^m} \frac{f_n}{r_{\mathrm{a}}^n}\idiff S\\
%	& P_{mn} = \int_{\Gamma_{\mathrm{a}}} \frac{f_m}{r_{\mathrm{a}}^m} \vec{a}\cdot\nabla_S \left(\frac{f_n}{r_{\mathrm{a}}^n}\right)\idiff S, \quad && Q_{mn} = \int_{\Gamma_{\mathrm{a}}}\frac{f_n}{r_{\mathrm{a}}^n}\vec{a}\cdot\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) \idiff S\\
%	& J_{mn} = \int_{\Gamma_{\mathrm{a}}} \nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) \cdot\nabla_S \left(\frac{f_n}{r_{\mathrm{a}}^n}\right)\idiff S.
%\end{alignedat}	
%\end{equation}
%In the case of spherical coordinates (where $\Gamma_{\mathrm{a}}$ is the unit sphere) we get $P_{mn}=0$, $Q_{mn} = 0$ and $I_{mn} = I_{mn}'$ such that the bilinear form reduces to the expression in~\cite[p. 93]{Ihlenburg1998fea}. Ihlenburg then notes that the integrals of the form
%\begin{equation*}
%	\int_1^\infty\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^n}\idiff\zeta,\quad n\geq 1
%\end{equation*}
%exist and may be computed. Indeed, the \textit{exponential integral} function defined by
%\begin{equation*}
%	E_n(x) = \int_1^\infty \frac{\euler^{-x\zeta}}{\zeta^n}\idiff\zeta
%\end{equation*}
%is implemented in MATLAB for $n=1$, and using the recursive relation
%\begin{equation*}
%	E_n(x) = \frac{1}{n-1}\left(\euler^{-x} - xE_{n-1}(x)\right),\quad n=2,3,4,\dots
%\end{equation*}
%found in~\cite[p. 229]{Abramovitz1964ham}, we can compute the integrals by
%\begin{equation*}
%	\int_1^\infty\frac{\euler^{2\imag r_{\mathrm{a}} k\zeta}}{\zeta^n}\idiff\zeta = E_n(-2\imag r_{\mathrm{a}} k).
%\end{equation*}
%Also for our case, it thus remains to consider the case $n=m=1$. Consider the limit
%\begin{align*}
%	L &= \lim_{\gamma\to\infty}\left[-\left(r_{\mathrm{a}}^2I_{11}' + I_{11}\right)k^2\int_1^\gamma\euler^{2\imag r_{\mathrm{a}} k\zeta}\idiff\zeta - I_{11}'\imag r_{\mathrm{a}} k\euler^{2\imag r_{\mathrm{a}} kR}\right]\\
%	 &= \lim_{\gamma\to\infty}\left[\frac{\imag k}{2}\left(I_{11} - r_{\mathrm{a}}^2I_{11}'\right)\euler^{2\imag k R} - \frac{\imag k}{2}\left(r_{\mathrm{a}}^2I_{11}' + I_{11}\right)\euler^{2\imag k r_{\mathrm{a}}}\right]
%\end{align*}
%which exists since $I_{11} = r_{\mathrm{a}}^2I_{11}'$. The limit reduces therefore to
%\begin{equation*}
%	L = - \frac{\imag k}{2}\left(r_{\mathrm{a}}^2I_{11}' + I_{11}\right)\euler^{2\imag r_{\mathrm{a}} k}
%\end{equation*}
%The bilinear form is then
%\begin{align*}
%	b_{uc}(v,u) &= J_{mn}E_{m+n} +P_{mn}[\imag r_{\mathrm{a}} k E_{m+n-1} - mE_{m+n}]+Q_{mn}[\imag r_{\mathrm{a}} kE_{m+n-1} - nE_{m+n}]\\
%	 &+ I_{mn}'[-(r_{\mathrm{a}} k)^2E_{m+n-2} - \imag r_{\mathrm{a}} k(n+m)E_{m+n-1} + nm E_{m+n}] - I_{mn}k^2E_{m+n-2}
%\end{align*}
%where $E_{n} = E_{n}(-2\imag r_{\mathrm{a}} k)$. And for the special case $n=m=1$ we get
%\begin{align*}
%	b_{uc}(v,u) &= J_{11}E_{2} +P_{11}[\imag r_{\mathrm{a}} k E_{1} - E_{2}]+Q_{11}[\imag r_{\mathrm{a}} kE_{1} - E_{2}]\\
%	 &+ I_{11}'[- 2\imag r_{\mathrm{a}} kE_{1} + E_{2}] - \frac{\imag k}{2}\left(r_{\mathrm{a}}^2 I_{11}' + I_{11}\right)\euler^{2\imag r_{\mathrm{a}} k}
%\end{align*}
%This will also be the result of PG method if the test functions are not conjugated. This is because all integrals exist as $n+m>3$ in this case.
%
%Let
%\begin{equation*}
%	f_n = \sum_{A\in\vec{\eta}_{\mathrm{a}}} R_A c_{nA},\quad f_m = \sum_{B\in\vec{\eta}_{\mathrm{a}}} R_B d_{mB}
%\end{equation*}
%where we bake $r_{\mathrm{a}}^n$ a,d $r_{\mathrm{a}}^m$ into the coefficients of $c_{nA}$ and $d_{mB}$, respectively.
%
%where $\vec{\eta}_{\mathrm{a}}$ is the set containing the indices of all the basis functions that are non-zero on $\Gamma_{\mathrm{a}}$. As the $b_{uc}$ are linear we then obtain (for $\zeta > 1$)
%\begin{equation*}
%	\sum_{A\in\vec{\eta}_{\mathrm{a}}}\sum_{n=1}^N c_{nA}\left(\sum_{B\in\vec{\eta}_{\mathrm{a}}}\sum_{m=1}^N d_{nA} b_{uc}(R_A, R_B)\right) = 0.
%\end{equation*}
%As the surface integrals in \Cref{Eq2:infiniteElementsSurfaceIntegrals5} will now be independent of the indices $m$ and $n$ we could now define the bilinear form by (for $n+m>1$)
%\begin{align*}
%	b_{uc}(R_A,R_B) &= J_{AB} E_{m+n} +P_{AB} [\imag k E_{m+n-1} - mE_{m+n}]+Q_{AB} [\imag kE_{m+n-1} - nE_{m+n}]\\
%	 &+ I_{AB}'[-k^2E_{m+n-2} - \imag k(n+m)E_{m+n-1} + nm E_{m+n}] - I_{AB} k^2E_{m+n-2}
%\end{align*}
%and for the case $n=m=1$ by
%\begin{align*}
%	b_{uc}(v,u) &= J_{AB}E_{2} +P_{AB}[\imag r_{\mathrm{a}} k E_{1} - E_{2}]+Q_{AB}[\imag r_{\mathrm{a}} kE_{1} - E_{2}]\\
%	 &+ I_{AB}'[- 2\imag r_{\mathrm{a}}kE_{1} + E_{2}] - \frac{\imag k}{2}\left(r_{\mathrm{a}}^2I_{AB}' + I_{AB}\right)\euler^{2\imag k}
%\end{align*}
%where we have redefined the surface integral notations to be
%\begin{alignat*}{2}
%	& I_{AB} = \int_{\Gamma_{\mathrm{a}}} R_A R_B \idiff S,\qquad\qquad && P_{AB} = \int_{\Gamma_{\mathrm{a}}} R_B \vec{a}\cdot\nabla_S R_A\idiff S\\
%	& I_{AB}' = \int_{\Gamma_{\mathrm{a}}} \norm{\vec{a}}^2 R_A R_B\idiff S, \quad && Q_{AB} = \int_{\Gamma_{\mathrm{a}}}R_A\vec{a}\cdot\nabla_S R_B \idiff S\\
%	& J_{AB} = \int_{\Gamma_{\mathrm{a}}} \nabla_S R_B \cdot\nabla_S R_A\idiff S.
%\end{alignat*}
%The infinite elements are thus only contributing whenever we have an element adjacent to the boundary $\Gamma_{\mathrm{a}}$. It is important to note that we now have increased the number of degrees of freedom at the surface $\Gamma_{\mathrm{a}}$ from $|\vec{\eta}_{\mathrm{a}}|$ to $N|\vec{\eta}_{\mathrm{a}}|$. Hence, the method of infinite elements adds a total of $(N-1)|\vec{\eta}_{\mathrm{a}}|$ degrees of freedom. Also note that the surface integrals for $P_{AB}$ and $Q_{AB}$ results in the same set of values. In fact $Q_{AB} = P_{BA}$.  Due to redundancy, we should not evaluate the full 3D NURBS function set at $\zeta=1$ as the 3D NURBS basis functions reduce to a 2D NURBS surface in 3D. Rather, we loop over the surface elements which is then done separate from the main matrix assembly. Thus, the procedure of adding contribution from infinite elements follows the procedure of applying Neumann conditions except that we do not update the load vector $\vec{F}$, rather, we now update the global matrix.
%
%
%
%
%
%
%
%
%
%
%It is also possible to use the complex conjugate of the test functions. In stead of a bilinear form, we then get a sesquilinear form.  The weak formulating then takes the form: For all $v\in V_1$, find $u_h^N\in V_1$ such that
%\begin{equation*}
%	b_c(u_h^N, v) = \langle g,v\rangle_\Gamma,
%\end{equation*}
%where
%\begin{align}\label{Eq2:infElemntBilinearForm6}
%	b_c(v,u) &= \lim_{\gamma\to\infty}\left(\int_{\Omega_\gamma} (\nabla \bar{v} \nabla u - k^2 \bar{v}u)\idiff\Omega - \int_{S_\gamma} \bar{v}\partial_n u\idiff\Gamma\right),\\
%	\langle g,\bar{v}\rangle_\Gamma &= \int_\Gamma g\bar{v}\idiff\Gamma.
%\end{align}
%Again we consider trial and test functions of the form
%\begin{equation*}
%	u = \frac{\euler^{\imag r_{\mathrm{a}} k\zeta}}{\zeta^m}\frac{f_m}{r_{\mathrm{a}}^m},\quad v = \frac{\euler^{\imag r_{\mathrm{a}} k\zeta}}{\zeta^n}\frac{f_n}{r_{\mathrm{a}}^n},\quad
%\end{equation*}
%such that
%\begin{align*}
%	\nabla \bar{v}\cdot\nabla u &= \left(\frac{1}{\zeta}\nabla_S \bar{v} + \vec{a}\pderiv{\bar{v}}{\zeta}\right)\cdot\left(\frac{1}{\zeta}\nabla_S u + \vec{a}\pderiv{u}{\zeta}\right)\\
%	&= \frac{1}{\zeta^{m+n+2}}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\nabla_S \frac{\bar{f}_n}{r_{\mathrm{a}}^n} +\frac{1}{\zeta^{m+n+1}}\left(\imag k - \frac{m}{\zeta}\right)\frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\nabla_S \frac{\bar{f}_n}{r_{\mathrm{a}}^n}\\
%	&+ \frac{1}{\zeta^{m+n+1}}\left(-\imag k - \frac{n}{\zeta}\right)\frac{\bar{f}_n}{r_{\mathrm{a}}^n}\vec{a}\cdot\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) + \norm{\vec{a}}^2\frac{1}{\zeta^{m+n}}\left(-\imag k - \frac{n}{\zeta}\right)\left(\imag k - \frac{m}{\zeta}\right)\frac{f_m}{r_{\mathrm{a}}^m} \frac{\bar{f}_n}{r_{\mathrm{a}}^n}.
%\end{align*}
%and
%\begin{align*}
%	\bar{v}\partial_n u &= \bar{v}\nabla u\cdot\vec{n} = \bar{v}\left(\frac{1}{\zeta}\nabla_S u + \vec{a}\pderiv{u}{\zeta}\right)\cdot\vec{n} = \frac{1}{\zeta}\bar{v}\nabla_S u\cdot\vec{n} + \bar{v}\pderiv{u}{\zeta}\vec{a}\cdot\vec{n}\\
%	&= \frac{1}{\zeta^{m+n+1}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n} + \left(\imag k - \frac{m}{\zeta}\right) \frac{1}{\zeta^{m+n}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\vec{n}.
%\end{align*}
%Again we first consider the boundary integral at $S_\gamma$
%\begin{align*}
%	\int_{S_\gamma} \bar{v}\partial_n u\idiff\Gamma &= \int_{\Gamma_{\mathrm{a}}}\frac{1}{R^{m+n+1}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n} R^2 \kappa\idiff S + \int_{\Gamma_{\mathrm{a}}} \left(\imag k - \frac{m}{R}\right) \frac{1}{R^{m+n}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m} \vec{a}\cdot\vec{n}R^2\kappa\idiff S\\
%	&= \frac{1}{R^{m+n-1}}\int_{\Gamma_{\mathrm{a}}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n}\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right)\cdot\vec{n}\kappa\idiff S + \frac{1}{R^{m+n-2}}\left(\imag k - \frac{m}{R}\right)\int_{\Gamma_{\mathrm{a}}}  \frac{\bar{f}_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\vec{a}\cdot\vec{n}\kappa\idiff S
%\end{align*}
%As $m+n>1$ all terms of order $\mathcal{O}(\gamma^{-(m+n-1)})$ vanish in the limit $\gamma\to\infty$, such that the integral reduces to
%\begin{equation*}
%	\int_{S_\gamma} v\partial_n u\idiff\Gamma = \imag k\frac{1}{R^{m+n-2}}\int_{\Gamma_{\mathrm{a}}} \frac{a_{33}}{\bar{h}_{\upzeta}^2} \frac{\bar{f}_n}{r_{\mathrm{a}}^n} \frac{f_m}{r_{\mathrm{a}}^m}\idiff S
%\end{equation*}
%Combining all of this into \Cref{Eq2:infElemntBilinearForm6} yields
%\begin{align*}
%	b_c(v,u) = \lim_{\gamma\to\infty}&\left\{J_{mn}\int_1^\gamma \frac{1}{\zeta^{m+n}}\idiff\zeta + P_{mn}\int_1^\gamma\frac{1}{\zeta^{m+n-1}}\left(\imag k - \frac{m}{\zeta}\right)\idiff\zeta\right.\\
%	 &\left.+ Q_{mn}\int_1^\gamma\frac{1}{\zeta^{m+n-1}}\left(-\imag k - \frac{n}{\zeta}\right)\idiff\zeta \right.\\
%	&\left. + I_{mn}'\int_1^\gamma\frac{1}{\zeta^{m+n}}\left[(k\zeta)^2 - \imag k\zeta(n - m) + nm\right]\idiff\zeta \right.\\
%	&\left.- I_{mn}\int_1^\gamma\frac{1}{\zeta^{m+n}}(k\zeta)^2\idiff\zeta - \imag kI_{mn}'\frac{1}{R^{m+n-2}}\right\}
%\end{align*}
%where
%\begin{equation}\label{Eq2:infiniteElementsSurfaceIntegrals6}
%\begin{alignedat}{2}
%	& I_{mn} = \int_{\Gamma_{\mathrm{a}}} \frac{f_m}{r_{\mathrm{a}}^m} \frac{\bar{f}_n}{r_{\mathrm{a}}^n}\idiff S,\qquad\qquad && I_{mn}' = \int_{\Gamma_{\mathrm{a}}} \frac{a_{33}}{\bar{h}_{\upzeta}^2} \frac{f_m}{r_{\mathrm{a}}^m} \frac{\bar{f}_n}{r_{\mathrm{a}}^n}\idiff S\\
%	& P_{mn} = \int_{\Gamma_{\mathrm{a}}} \frac{f_m}{r_{\mathrm{a}}^m} \vec{a}\cdot\nabla_S \frac{\bar{f}_n}{r_{\mathrm{a}}^n}\idiff S, \quad && Q_{mn} = \int_{\Gamma_{\mathrm{a}}}\frac{\bar{f}_n}{r_{\mathrm{a}}^n}\vec{a}\cdot\nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) \idiff S\\
%	& J_{mn} = \int_{\Gamma_{\mathrm{a}}} \nabla_S \left(\frac{f_m}{r_{\mathrm{a}}^m}\right) \cdot\nabla_S \frac{\bar{f}_n}{r_{\mathrm{a}}^n}\kappa\idiff S.
%\end{alignedat}	
%\end{equation}
%This time we not only need to consider the case $n=m=1$, but also the cases $n+m=3$. For the case $n+m=3$ we observe that we are depending on the cancellation of the terms involving $\frac{1}{\zeta^{m+n-2}}$. This occurs only if $I_{mn} = I_{mn}'$. Assume this to be the case. We must then consider the the limit (when $n=m=1$)
%\begin{align*}
%	L &= \lim_{\gamma\to\infty}\left[P_{11}\int_1^\gamma \frac{\imag k}{\zeta}\idiff\zeta - Q_{11}\int_1^\gamma \frac{\imag k}{\zeta}\idiff\zeta\right]\\
%	 &= \lim_{\gamma\to\infty}\left[\imag k(P_{11} - Q_{11})\int_1^\gamma \frac{\diff \zeta}{\zeta}\right]
%\end{align*}
%which exists if $P_{11} = Q_{11}$. Again, this only holds for special surfaces $\Gamma_{\mathrm{a}}$, like the unit sphere.  If this is the case, the limit is simply zero.
%
%For $m+n>2$ we simply evaluate the integrals
%\begin{equation*}
%	\int_1^\infty \frac{\diff\zeta}{\zeta^n} = \frac{1}{n-1},\quad n>1.
%\end{equation*}
%The sesquilinear form is then
%\begin{align*}
%	b_c(v,u) &= \frac{J_{mn}}{m+n-1} +P_{mn}\left(\frac{\imag k}{m+n-2} - \frac{m}{m+n-1}\right)+Q_{mn}\left(\frac{-\imag k}{m+n-2} - \frac{n}{m+n-1}\right)\\
%	 &+ I_{mn}'\left(\frac{k^2}{m+n-3} - \frac{\imag k(n-m)}{m+n-2} + \frac{nm}{n+m-1}\right) - I_{mn}\frac{k^2}{m+n-3}
%\end{align*}
%
%Let
%\begin{equation*}
%	\frac{f_n}{r_{\mathrm{a}}^n} = \sum_{A\in\vec{\eta}_{\mathrm{a}}} R_A c_{nA},\quad \frac{f_m}{r_{\mathrm{a}}^m} = \sum_{B\in\vec{\eta}_{\mathrm{a}}} R_B d_{mB}
%\end{equation*}
%where $\vec{\eta}_{\mathrm{a}}$ is the set containing the indices of all the basis functions that are non-zero on $\Gamma_{\mathrm{a}}$. As the $b_{uc}$ are linear we then obtain (for $\zeta > 1$)
%\begin{equation*}
%	\sum_{A\in\vec{\eta}_{\mathrm{a}}}\sum_{n=1}^N \bar{c}_{nA}\left(\sum_{B\in\vec{\eta}_{\mathrm{a}}}\sum_{m=1}^N d_{nA} b_{uc}(R_A, R_B)\right) = 0.
%\end{equation*}
%As the surface integrals in \Cref{Eq2:infiniteElementsSurfaceIntegrals6} will now be independent of the indices $m$ and $n$ we could now define the sesquilinear form by (for $n+m>1$)
%\begin{align*}
%	b_c(R_A,R_B) &= \frac{J_{AB}}{m+n-1} +P_{AB}\left(\frac{\imag k}{m+n-2} - \frac{m}{m+n-1}\right)\\
%	&+Q_{AB}\left(\frac{-\imag k}{m+n-2} - \frac{n}{m+n-1}\right)\\
%	 &+ I_{AB}'\left(\frac{k^2}{m+n-3} - \frac{\imag k(n-m)}{m+n-2} + \frac{nm}{n+m-1}\right) - I_{AB}\frac{k^2}{m+n-3}
%\end{align*}
%We must thus conclude that the extended NURBS coordinate system works best for Petrov--Galerkin methods as there will be no further restriction on the surface $\Gamma_{\mathrm{a}}$. For Bubnov--Galerkin methods the surface $\Gamma_{\mathrm{a}}$ is restricted to surfaces like the unit sphere, which then eliminates the point of introducing the extended NURBS coordinate system in the first place.
%
%The motivation of introducing the extended NURBS coordinate system is to be able to controle the artificial boundary $\Gamma_{\mathrm{a}}$. This allows us to control the size of the fluid domain which would in turn able us to reduce redundant fluid elements. Ihlenburg uses a prolate spheroid as the artificial boundary around his ``Mock shell'' in~\cite{Ihlenburg1998fea}. As the ``Mock shell'' is a convex surface, one could have a uniform thickness of the fluid around the shell by the extended NURBS coordinate system, and thus reducing the fluid computational domain to an ideal size. 

%
\subsection{The cylindrical coordinate system}
\label{Sec2:cylindricalCoordinates}
\tikzsetnextfilename{polarDecomposition_11}
\begin{figure}
	\centering
	\begin{tikzpicture}
	\def\x{1.414213562373095}
	 
	\draw [->](0,1) -- (7,1) node[right] {$x$};
	\draw [->](1,0) -- (1,7) node[above] {$y$};
	
	\draw [-](1,1) -- (4,4);
	
	\draw [dashed] (4,4) node (v1) {} ellipse (2 and 2);
	
	\draw (2,1) arc (0:45:1);
	
	  
	\draw[->] (4,4) -- (4-\x, 4+\x) node (v2) {};
	\draw[->]  (4,4) -- (4,6);
	\draw[->] (4,4) -- (4+\x, 4+\x) node (v3) {};
	\draw[->] (4,4) -- (6,4);
	\draw[->] (4,4) -- (2,4);
	
	\draw[dotted] (v2) -- (4-\x,4);
	\draw[dotted] (v3) -- (4+\x,4);
	
	\node at (2.1,1.5) {$\vartheta$};
	\node at (6.3,4) {$\vec{e}_{\mathrm{x}}$};
	\node at (2-0.5,4) {$-\vec{e}_{\mathrm{x}}$};
	\node at (4,6.3) {$\vec{e}_{\mathrm{y}}$};
	\node at (2.4,5.6) {$\vec{e}_{\upvartheta}$};
	\node at (5.6,5.6) {$\vec{e}_{\mathrm{r}}$};
	
	\node at (2*1.59,2*1.91) {\scriptsize $\sin\vartheta$};
	\node at (4.7,2*1.9) {\scriptsize $\cos\vartheta$};
	
	\node at (2.4,4.6)[rotate=90] {\scriptsize $\cos\vartheta$};
	\node at (6-0.4,4.6)[rotate=90] {\scriptsize $\sin\vartheta$};
	
	\node at (4-\x+0.2,5-0.2) {\scriptsize $\vartheta$};
	\node at (4+0.6,4+0.3) {\scriptsize $\vartheta$};
	
	\draw (4-\x,5) arc (-90:-45:\x-1);
	\draw (4+\x-1,4) arc (0:45:\x-1);
	
	\end{tikzpicture}
	\caption[Unit vectors in polar coordinate system]{Decomposition of the standard unit vectors in the polar coordinate system to the standard unit vectors in the Cartesian coordinate system.}
	\label{Fig2:polarDecomposition}
\end{figure}
The cylindrical coordinate system is simply an extension of the polar coordinate system, which from standard Cartesian coordinates is given by the transformation
\begin{align*}
	x &= r\cos\vartheta\\
	y &= r\sin\vartheta\\
\end{align*}
such that
\begin{align*}
	r &= \sqrt{x^2+y^2}\\
	\vartheta &= \operatorname{atan2}(y,x)
\end{align*}
where
\begin{equation*}
	\operatorname{atan2}(y,x) = \begin{cases}
	\arctan(\frac{y}{x}) & \mbox{if } x > 0\\
	\arctan(\frac{y}{x}) + \PI & \mbox{if } x < 0 \mbox{ and } y \ge 0\\
	\arctan(\frac{y}{x}) - \PI & \mbox{if } x < 0 \mbox{ and } y < 0\\
	\frac{\PI}{2} & \mbox{if } x = 0 \mbox{ and } y > 0\\
	-\frac{\PI}{2} & \mbox{if } x = 0 \mbox{ and } y < 0\\
	\text{undefined} & \mbox{if } x = 0 \mbox{ and } y = 0
	\end{cases}.
\end{equation*}
By this we find
\begin{alignat*}{3}
	\pderiv{r}{x} &= \cos\vartheta,\qquad	&&\pderiv{r}{y} = \sin\vartheta\\
	\pderiv{\vartheta}{x} &= -\frac{1}{r}\sin\vartheta,\qquad	&&\pderiv{\vartheta}{y} = \frac{1}{r}\cos\vartheta.
\end{alignat*}
So for a scalar valued function $\psi$ we get (using the chain rule)
\begin{align}
\label{Eq2:derivativesInPolar}
\begin{split}
	\pderiv{\psi}{x} = \pderiv{\psi}{r}\pderiv{r}{x} + \pderiv{\psi}{\vartheta}\pderiv{\vartheta}{x} = \cos\vartheta\pderiv{\psi}{r} -\frac{1}{r}\sin\vartheta \pderiv{\psi}{\vartheta}\\
	\pderiv{\psi}{y} = \pderiv{\psi}{r}\pderiv{r}{y} + \pderiv{\psi}{\vartheta}\pderiv{\vartheta}{y} = \sin\vartheta\pderiv{\psi}{r} + \frac{1}{r}\cos\vartheta\pderiv{\psi}{\vartheta}
\end{split}
\end{align}
Moreover, by decomposing the standard unit vectors in the polar coordinate system to the standard unit vectors in the Cartesian coordinate system (cf. \Cref{Fig2:polarDecomposition}) we get
\begin{align*}
	\vec{e}_{\mathrm{r}} &= \cos\vartheta\vec{e}_{\mathrm{x}} + \sin\vartheta\vec{e}_{\mathrm{y}}\\
	\vec{e}_{\upvartheta} &= -\sin\vartheta\vec{e}_{\mathrm{x}}+\cos\vartheta\vec{e}_{\mathrm{y}}.
\end{align*}
Hence, for any vector valued function in two dimensions
\begin{equation*}
	\vec{\Psi} = \Psi_{\mathrm{x}}\vec{e}_{\mathrm{x}} + \Psi_{\mathrm{y}}\vec{e}_{\mathrm{y}} = \Psi_{\mathrm{r}}\vec{e}_{\mathrm{r}} + \Psi_{\upvartheta}\vec{e}_{\upvartheta}
\end{equation*}
we get the relations (by comparing each component)
\begin{align}
\label{Eq2:PolarToXfun}
\begin{split}
	\Psi_{\mathrm{x}} &= \Psi_{\mathrm{r}}\cos\vartheta - \Psi_{\upvartheta}\sin\vartheta\\
	\Psi_{\mathrm{y}} &= \Psi_{\mathrm{r}}\sin\vartheta + \Psi_{\upvartheta}\cos\vartheta.
\end{split}
\end{align}
By a corresponding argument, we have
\begin{align}
\label{Eq2:XtoPolar}
\begin{split}
	\vec{e}_{\mathrm{x}} &= \cos\vartheta\vec{e}_{\mathrm{r}} - \sin\vartheta\vec{e}_{\upvartheta}\\
	\vec{e}_{\mathrm{y}} &= \sin\vartheta\vec{e}_{\mathrm{r}}+\cos\vartheta\vec{e}_{\upvartheta}
\end{split}
\end{align}
such that
\begin{align*}
	\Psi_{\mathrm{r}} &= \Psi_{\mathrm{x}}\cos\vartheta + \Psi_{\mathrm{y}}\sin\vartheta\\
	\Psi_{\upvartheta} &= -\Psi_{\mathrm{x}}\sin\vartheta + \Psi_{\mathrm{y}}\cos\vartheta.
\end{align*}
All of these relation also holds for cylindrical coordinates as the $z$ variable is the same for both coordinate systems.

Using \Cref{Eq2:derivativesInPolar}, \Cref{Eq2:PolarToXfun} and \Cref{Eq2:XtoPolar} we get
\begin{align}
	\nabla\psi &= \pderiv{\psi}{x}\vec{e}_{\mathrm{x}} + \pderiv{\psi}{y}\vec{e}_{\mathrm{y}} + \pderiv{\psi}{z}\vec{e}_{\mathrm{z}} = \pderiv{\psi}{r}\vec{e}_{\mathrm{r}}+\frac{1}{r}\pderiv{\psi}{\vartheta}\vec{e}_{\upvartheta}+\pderiv{\psi}{z}\vec{e}_{\mathrm{z}} \label{Eq2:delScalarCyl} \\	
	\nabla^2\psi &= \pderiv[2]{\psi}{x} + \pderiv[2]{\psi}{y} + \pderiv[2]{\psi}{z} = \frac{1}{r}\pderiv{}{r}\left(r\pderiv{\psi}{r}\right) + \frac{1}{r^2}\pderiv[2]{\psi}{\vartheta} +\pderiv[2]{\psi}{z}\\
	\nabla\cdot\vec{\Psi} &= \pderiv{\Psi_{\mathrm{x}}}{x}\ + \pderiv{\Psi_{\mathrm{y}}}{y} + \pderiv{\Psi_{\mathrm{z}}}{z} = \frac{1}{r}\pderiv{(r\Psi_{\mathrm{r}})}{r} + \frac{1}{r}\pderiv{\Psi_{\upvartheta}}{\vartheta}+\pderiv{\Psi_{\mathrm{z}}}{z} \label{Eq2:DelDotVecCyl}\\ 
	\nabla^2\vec{\Psi} &= \left(\nabla^2\Psi_{\mathrm{r}} - \frac{1}{r^2}\Psi_{\mathrm{r}}-\frac{2}{r^2}\pderiv{\Psi_{\upvartheta}}{\vartheta}\right)\vec{e}_{\mathrm{r}} + \left(\nabla^2\Psi_{\upvartheta}-\frac{1}{r^2}\Psi_{\upvartheta} + \frac{2}{r^2}\pderiv{\Psi_{\mathrm{r}}}{\vartheta}\right)\vec{e}_{\upvartheta} + \nabla^2\Psi_{\mathrm{z}}\vec{e}_{\mathrm{z}} \label{Eq2:LapVecPotCyl}
\end{align}
For axisymmetric problems, it is also convenient to write the stress field and the strain field in terms of polar coordinates. Recall that
\begin{equation*}
	\begin{bmatrix}
		\sigma_{11}\\
		\sigma_{22}\\
		\sigma_{33}\\
		\sigma_{23}\\
		\sigma_{13}\\
		\sigma_{12}\\
	\end{bmatrix} = \vec{C}
	\begin{bmatrix}
		\varepsilon_{11}\\
		\varepsilon_{22}\\
		\varepsilon_{33}\\
		2\varepsilon_{23}\\
		2\varepsilon_{13}\\
		2\varepsilon_{12}\\
	\end{bmatrix} = \begin{bmatrix}
		2\mu+\lambda & \lambda & \lambda & 0 & 0 & 0\\
		\lambda & 2\mu+\lambda & \lambda & 0 & 0 & 0\\
		\lambda & \lambda & 2\mu+\lambda & 0 & 0 & 0\\
		0 & 0 & 0 & \mu & 0 & 0\\
		0 & 0 & 0 & 0 & \mu & 0\\
		0 & 0 & 0 & 0 & 0 & \mu
	\end{bmatrix}
	\begin{bmatrix}
		\varepsilon_{11}\\
		\varepsilon_{22}\\
		\varepsilon_{33}\\
		2\varepsilon_{23}\\
		2\varepsilon_{13}\\
		2\varepsilon_{12}\\
	\end{bmatrix}.
\end{equation*}
such that if the stress field is given, we may invert the elasticity matrix to find the strain field. We note that
\begin{equation*}
	\vec{C}^{-1} = \frac{1}{E}\begin{bmatrix}
		1 & -\nu & -\nu & 0 & 0 & 0\\
		-\nu & 1 & -\nu & 0 & 0 & 0\\
		-\nu & -\nu & 1 & 0 & 0 & 0\\
		0 & 0 & 0 & \frac{1}{\mu} & 0 & 0\\
		0 & 0 & 0 & 0 & \frac{1}{\mu} & 0\\
		0 & 0 & 0 & 0 & 0 & \frac{1}{\mu}
	\end{bmatrix}.
\end{equation*}
In~\cite[p. 19]{Gould1994itl} we find the transformation formula for the stress tensor from an arbitrary coordinate system to another. If $\vec{e}_i$ and $\vec{e}_i'$ represents the basis vectors of these two coordinate systems and the stress field is known in the first coordinate system, then the stress field in terms of the second coordinate system is found by
\begin{equation*}
	\sigma_{ij}' = \alpha_{ik}\alpha_{jl}\sigma_{kl}
\end{equation*}
where
\begin{equation*}
	\alpha_{ij} = \cos(\vec{e}_i', \vec{e}_j) = \vec{e}_i'\cdot\vec{e}_j
\end{equation*}
represents the cosine of the angle between the axis corresponding to the vectors $\vec{e}_i$ and $\vec{e}_i'$, respectively. Letting $\vec{e}_1' = \vec{e}_{\mathrm{r}}$, $\vec{e}_2' = \vec{e}_{\mathrm{r}}$ and $\vec{e}_3' = \vec{e}_{\mathrm{z}}$ (the basis vectors in cylindrical coordinates), and $\{\vec{e}_1, \vec{e}_2, \vec{e}_3\}$ the standard basis vectors in Cartesian coordinates, we find (using \Cref{Eq2:XtoPolar})
\begin{equation*}
	[\alpha_{ij}] = \begin{bmatrix}
	\cos\vartheta & \sin\vartheta & 0\\
	-\sin\vartheta & \cos\vartheta & 0\\
	0 & 0 & 1
	\end{bmatrix}.
\end{equation*}
This yields the following relations
\begin{align*}
	\sigma_{\mathrm{rr}} &= \sigma_{11}\cos^2\vartheta + \sigma_{22}\sin^2\vartheta + \sigma_{12}\sin(2\vartheta)\\
	\sigma_{\upvartheta\upvartheta} &= \sigma_{11}\sin^2\vartheta + \sigma_{22}\cos^2\vartheta - \sigma_{12}\sin(2\vartheta)\\
	\sigma_{\mathrm{zz}} &= \sigma_{33}\\
	\sigma_{\upvartheta\mathrm{z}} &= \sigma_{23}\cos\vartheta - \sigma_{13}\sin\vartheta\\
	\sigma_{\mathrm{rz}} &= \sigma_{23}\sin\vartheta + \sigma_{13}\cos\vartheta\\
	\sigma_{\mathrm{r}\upvartheta} &= -\frac{1}{2}\sigma_{11}\sin(2\vartheta) + \frac{1}{2}\sigma_{22}\sin(2\vartheta) + \sigma_{12}\cos(2\vartheta)
\end{align*}
The inverse relations are found to be
\begin{align*}
	\sigma_{11} &= \sigma_{\mathrm{rr}}\cos^2\vartheta + \sigma_{\upvartheta\upvartheta}\sin^2\vartheta - \sigma_{\mathrm{r}\upvartheta}\sin(2\vartheta)\\
	\sigma_{22} &= \sigma_{\mathrm{rr}}\sin^2\vartheta + \sigma_{\upvartheta\upvartheta}\cos^2\vartheta + \sigma_{\mathrm{r}\upvartheta}\sin(2\vartheta)\\
	\sigma_{33} &= \sigma_{\mathrm{zz}}\\
	\sigma_{23} &= \sigma_{\upvartheta\mathrm{z}}\cos\vartheta + \sigma_{\mathrm{rz}}\sin\vartheta\\
	\sigma_{13} &= -\sigma_{\upvartheta\mathrm{z}}\sin\vartheta + \sigma_{\mathrm{rz}}\cos\vartheta\\
	\sigma_{12} &= \frac{1}{2}\sin(2\vartheta)\sigma_{\mathrm{rr}} - \frac{1}{2}\sin(2\vartheta)\sigma_{\upvartheta\upvartheta} - \cos(2\vartheta)\sigma_{\mathrm{r}\upvartheta}.
\end{align*}
Moreover, we have
\begin{equation}\label{Eq2:constitutiveRelationPolar}
	\begin{bmatrix}
		\sigma_{\mathrm{rr}}\\
		\sigma_{\upvartheta\upvartheta}\\
		\sigma_{\mathrm{zz}}\\
		\sigma_{\upvartheta\mathrm{z}}\\
		\sigma_{\mathrm{rz}}\\
		\sigma_{\mathrm{r}\upvartheta}\\
	\end{bmatrix} = \vec{C}
	\begin{bmatrix}
		\varepsilon_{\mathrm{rr}}\\
		\varepsilon_{\upvartheta\upvartheta}\\
		\varepsilon_{\mathrm{zz}}\\
		2\varepsilon_{\upvartheta\mathrm{z}}\\
		2\varepsilon_{\mathrm{rz}}\\
		2\varepsilon_{\mathrm{r}\upvartheta}\\
	\end{bmatrix},
\end{equation}
where (see~\cite{Slaughter2002tlt} for details)
\begin{equation}
\label{Eq2:strainsInPolar}
\begin{split}
	\varepsilon_{\mathrm{rr}} &= \pderiv{u_{\mathrm{r}}}{r}\\
	\varepsilon_{\upvartheta\upvartheta} &= \frac{1}{r}\left(\pderiv{u_{\upvartheta}}{\vartheta} + u_{\mathrm{r}}\right)\\
	\varepsilon_{\mathrm{zz}} &= \pderiv{u_z}{z}\\
	\varepsilon_{\upvartheta\mathrm{z}} &= \frac{1}{2}\left(\pderiv{u_{\upvartheta}}{z} + \frac{1}{r}\pderiv{u_z}{\vartheta}\right)\\
	\varepsilon_{\mathrm{rz}} &= \frac{1}{2}\left(\pderiv{u_{\mathrm{r}}}{z} + \pderiv{u_z}{r}\right)\\
	\varepsilon_{\mathrm{r}\upvartheta} &= \frac{1}{2}\left(\frac{1}{r}\pderiv{u_{\mathrm{r}}}{\vartheta} + \pderiv{u_{\upvartheta}}{r} - \frac{u_{\upvartheta}}{r}\right).
\end{split}
\end{equation}


\subsection{The spherical coordinate system}
\label{Sec2:sphericalCoordinates}
There are several conventions for defining the spherical coordinate system, but we shall here follow the ISO standard (International Organization for Standardization), which is the convention often used in physics. The reason why the mathematical convention of the spherical coordinate system is not used (where the angle $\vartheta$ is preserved in the $xy$-plane as in polar coordinates) is because of the existing literature on the subject of this thesis (in particular~\cite{Ihlenburg1998fea}). The spherical coordinate system is defined by the transformation (from the standard Cartesian coordinates)
\begin{align*}
	x &= r\sin\vartheta\cos\phi\\
	y &= r\sin\vartheta\sin\phi\\
	z &= r\cos\vartheta
\end{align*}
such that
\begin{align*}
	r &= \sqrt{x^2+y^2+z^2}\\
	\vartheta &= \arccos\left(\frac{z}{\sqrt{x^2+y^2+z^2}}\right)\\
	\phi &= \operatorname{atan2}(y,x).
\end{align*}
By this we find
\begin{alignat*}{4}
	\pderiv{r}{x} &= \sin\vartheta\cos\phi,\qquad	&&\pderiv{r}{y} = \sin\vartheta\sin\phi,\qquad	&&\pderiv{r}{z} = \cos\vartheta\\
	\pderiv{\vartheta}{x} &= \frac{1}{r}\cos\vartheta\cos\phi,\qquad	&&\pderiv{\vartheta}{y} = \frac{1}{r}\cos\vartheta\sin\phi,\qquad	&&\pderiv{\vartheta}{z} = -\frac{1}{r}\sin\vartheta\\
	\pderiv{\phi}{x} &= -\frac{1}{r}\frac{\sin\phi}{\sin\vartheta},\qquad	&&\pderiv{\phi}{y} = \frac{1}{r}\frac{\cos\phi}{\sin\vartheta},\qquad	&&\pderiv{\phi}{z} = 0.
\end{alignat*}
So for a scalar valued function $\psi$ we get (using the chain rule)
\begin{align}
\label{Eq2:derivativesInSphericalCoordinates}
\begin{split}
	\pderiv{\psi}{x} &= \pderiv{\psi}{r}\pderiv{r}{x} + \pderiv{\psi}{\phi}\pderiv{\phi}{x} + \pderiv{\psi}{\vartheta}\pderiv{\vartheta}{x} =  \sin\vartheta\cos\phi\pderiv{\psi}{r} - \frac{1}{r}\frac{\sin\phi}{\sin\vartheta}\pderiv{\psi}{\phi} + \frac{1}{r}\cos\vartheta\cos\phi\pderiv{\psi}{\vartheta}\\
	\pderiv{\psi}{y} &= \pderiv{\psi}{r}\pderiv{r}{y} + \frac{1}{r}\frac{\cos\phi}{\sin\vartheta}\pderiv{\psi}{\phi} + \pderiv{\psi}{\vartheta}\pderiv{\vartheta}{y} = \sin\vartheta\cos\phi\pderiv{\psi}{r} + \pderiv{\psi}{\phi}\pderiv{\phi}{y} + \frac{1}{r}\cos\vartheta\sin\phi\pderiv{\psi}{\vartheta}\\
	\pderiv{\psi}{z} &= \pderiv{\psi}{r}\pderiv{r}{z} + \pderiv{\psi}{\phi}\pderiv{\phi}{z} + \pderiv{\psi}{\vartheta}\pderiv{\vartheta}{z} = \cos\vartheta\pderiv{\psi}{r} -\frac{1}{r}\sin\vartheta\pderiv{\psi}{\vartheta}\pderiv{\vartheta}{z}
\end{split}
\end{align}
Moreover, by decomposing the standard unit vectors in the polar coordinate system to the standard unit vectors in the Cartesian coordinate system we get
\begin{align*}
	\vec{e}_{\mathrm{r}} &= \sin\vartheta\cos\phi\vec{e}_{\mathrm{x}} + \sin\vartheta\sin\phi\vec{e}_{\mathrm{y}} + \cos\vartheta\vec{e}_{\mathrm{z}}\\
	\vec{e}_{\upvartheta} &= \cos\vartheta\cos\phi\vec{e}_{\mathrm{x}} + \cos\vartheta\sin\phi\vec{e}_{\mathrm{y}} - \sin\vartheta\vec{e}_{\mathrm{z}}\\
	\vec{e}_{\upphi} &= -\sin\phi\vec{e}_{\mathrm{x}} + \cos\phi\vec{e}_{\mathrm{y}}.
\end{align*}
Hence, for any vector valued function in two dimensions
\begin{equation*}
	\vec{\Psi} = \Psi_{\mathrm{x}}\vec{e}_{\mathrm{x}} + \Psi_{\mathrm{y}}\vec{e}_{\mathrm{y}}  + \Psi_{\mathrm{z}}\vec{e}_{\mathrm{z}} = \Psi_{\mathrm{r}}\vec{e}_{\mathrm{r}} + \Psi_{\upphi}\vec{e}_{\upphi} + \Psi_{\upvartheta}\vec{e}_{\upvartheta}
\end{equation*}
we get the relations (by comparing each component)
\begin{align}
\label{Eq2:SphericalToXfun}
\begin{split}
	\Psi_{\mathrm{x}} &= \Psi_{\mathrm{r}}\sin\vartheta\cos\phi + \Psi_{\upvartheta}\cos\vartheta\cos\phi - \Psi_{\upphi}\sin\phi\\
	\Psi_{\mathrm{y}} &= \Psi_{\mathrm{r}}\sin\vartheta\sin\phi + \Psi_{\upvartheta}\cos\vartheta\sin\phi - \Psi_{\upphi}\cos\phi\\
	\Psi_{\mathrm{z}} &= \Psi_{\mathrm{r}}\cos\vartheta - \Psi_{\upvartheta}\sin\vartheta.
\end{split}
\end{align}
By a corresponding argument, we have
\begin{align}
\label{Eq2:XtoSpherical}
\begin{split}
	\vec{e}_{\mathrm{x}} &= \sin\vartheta\cos\phi\vec{e}_{\mathrm{r}} + \cos\vartheta\cos\phi\vec{e}_{\upvartheta} - \sin\phi\vec{e}_{\upphi}\\
	\vec{e}_{\mathrm{y}} &= \sin\vartheta\sin\phi\vec{e}_{\mathrm{r}} + \cos\vartheta\sin\phi\vec{e}_{\upvartheta} + \cos\phi\vec{e}_{\upphi}\\
	\vec{e}_{\mathrm{z}} &= \cos\vartheta\vec{e}_{\mathrm{r}} - \sin\vartheta\vec{e}_{\upvartheta}.
\end{split}
\end{align}
such that
\begin{align*}
\begin{split}
	\Psi_{\mathrm{r}} &= \Psi_{\mathrm{x}}\sin\vartheta\cos\phi + \Psi_{\mathrm{y}}\sin\vartheta\sin\phi + \Psi_{\mathrm{z}}\cos\vartheta\\
	\Psi_{\upvartheta} &= \Psi_{\mathrm{x}}\cos\vartheta\cos\phi + \Psi_{\mathrm{y}}\cos\vartheta\sin\phi - \Psi_{\mathrm{z}}\sin\vartheta\\
	\Psi_{\upphi} &= - \Psi_{\mathrm{x}}\sin\phi + \Psi_{\mathrm{y}}\cos\phi.
\end{split}
\end{align*}
Using \Cref{Eq2:derivativesInSphericalCoordinates}, \Cref{Eq2:SphericalToXfun} and \Cref{Eq2:XtoSpherical} we get
\begin{align}
	\nabla\psi &= \pderiv{\psi}{x}\vec{e}_{\mathrm{x}} + \pderiv{\psi}{y}\vec{e}_{\mathrm{y}} + \pderiv{\psi}{z}\vec{e}_{\mathrm{z}} = \pderiv{\psi}{r}\vec{e}_{\mathrm{r}}+\frac{1}{r}\pderiv{\psi}{\vartheta}\vec{e}_{\upvartheta}+\frac{1}{r\sin\vartheta}\pderiv{\psi}{\phi}\vec{e}_{\upphi} \label{Eq2:delScalarSpherical} \\	
	\nabla^2\psi &= \pderiv[2]{\psi}{x} + \pderiv[2]{\psi}{y} + \pderiv[2]{\psi}{z}\\ 
	&= \frac{1}{r^2}\pderiv{}{r}\left(r^2\pderiv{\psi}{r}\right) + \frac{1}{r^2\sin\vartheta}\pderiv{}{\vartheta}\left(\sin\vartheta\pderiv{\psi}{\vartheta}\right) +\frac{1}{r^2\sin^2\vartheta}\pderiv[2]{\psi}{\phi}\\
	\nabla\cdot\vec{\Psi} &= \pderiv{\Psi_{\mathrm{x}}}{x}\ + \pderiv{\Psi_{\mathrm{y}}}{y} + \pderiv{\Psi_{\mathrm{z}}}{z} = \frac{1}{r^2}\pderiv{(r^2\Psi_{\mathrm{r}})}{r} + \frac{1}{r\sin\vartheta}\pderiv{(\Psi_{\upvartheta}\sin\vartheta)}{\vartheta}+\frac{1}{r\sin\vartheta}\pderiv{\Psi_{\upphi}}{\phi} \label{Eq2:DelDotVecSpherical} \\ 
	\nabla^2\vec{\Psi} &= \left(\nabla^2\Psi_{\mathrm{r}} - \frac{2}{r^2}\Psi_{\mathrm{r}}-\frac{2}{r^2\sin\vartheta}\pderiv{(\Psi_{\upvartheta}\sin\vartheta)}{\vartheta} -\frac{2}{r^2\sin\vartheta}\pderiv{\Psi_{\upphi}}{\phi}\right)\vec{e}_{\mathrm{r}} \\
	&+ \left(\nabla^2\Psi_{\upvartheta}-\frac{1}{r^2\sin^2\vartheta}\Psi_{\upvartheta} + \frac{2}{r^2}\pderiv{\Psi_{\mathrm{r}}}{\vartheta} -\frac{2\cos\vartheta}{r^2\sin^2\vartheta}\pderiv{\Psi_{\upphi}}{\phi}\right)\vec{e}_{\upvartheta} \\
	&+ \left(\nabla^2\Psi_{\upphi} - \frac{1}{r^2\sin^2\vartheta}\Psi_{\upphi} + \frac{2}{r^2\sin\vartheta}\pderiv{\Psi_{\mathrm{r}}}{\phi}+\frac{2\cos\vartheta}{r^2\sin^2\vartheta}\pderiv{\Psi_{\upvartheta}}{\phi}\right)\vec{e}_{\upphi} \label{Eq2:LapVecPotSpherical}
\end{align}
We may also for the spherical coordinates find the relation between the stress fields as we did for the cylindrical coordinates in \Cref{Sec2:cylindricalCoordinates}. In spherical coordinates we get
\begin{equation*}
	[\alpha_{ij}] = \begin{bmatrix}
	\sin\vartheta\cos\phi & \sin\vartheta\sin\phi & \cos\vartheta\\
	\cos\vartheta\cos\phi & \cos\vartheta\sin\phi & -\sin\vartheta\\
	-\sin\phi & \cos\phi & 0
	\end{bmatrix}.
\end{equation*}
Which yields the relation
\begin{equation*}
	\begin{bmatrix}
		\sigma_{\mathrm{rr}}\\
		\sigma_{\upvartheta\upvartheta}\\
		\sigma_{\upphi\upphi}\\
		\sigma_{\upvartheta\upphi}\\
		\sigma_{\mathrm{r}\upphi}\\
		\sigma_{\mathrm{r}\upvartheta}
	\end{bmatrix} = \vec{D}
	\begin{bmatrix}
		\sigma_{11}\\
		\sigma_{22}\\
		\sigma_{33}\\
		\sigma_{23}\\
		\sigma_{13}\\
		\sigma_{12}
	\end{bmatrix}
\end{equation*}
where

\begin{equation*}\resizebox{\linewidth}{!}{$
	\vec{D} =\begin{bmatrix}
	 \sin^2\vartheta\cos^2\phi&\sin^2\vartheta\sin^2\phi&\cos^2\vartheta&\sin2\vartheta\sin\phi&\sin2\vartheta\cos\phi&\sin^2\vartheta\sin2\phi\\ 
	 \cos^2\vartheta\cos^2\phi&\cos^2\vartheta\sin^2\phi&\sin^2\vartheta&-\sin2\vartheta\sin\phi&-\sin2\vartheta\cos\phi&\cos^2\vartheta\sin2\phi\\ 
	 \sin^2\phi&\cos^2\phi&0&0&0&-\sin2\phi\\ 
	 -\frac12\cos\vartheta\sin2\phi&\frac12\cos\vartheta\sin2\phi&0&-\sin\vartheta\cos\phi&\sin\vartheta\sin\phi&\cos\vartheta\cos2\phi\\ 
	 -\frac12\sin\vartheta\sin2\phi&\frac12\sin\vartheta\sin2\phi&0&\cos\vartheta\cos\phi&-\cos\vartheta\sin\phi&\sin\vartheta\cos2\phi\\ 
	 \frac12\sin2\vartheta\cos^2\phi&\frac12\sin2\vartheta\sin^2\phi&-\frac12\sin2\vartheta&\cos2\vartheta\sin\phi&\cos2\vartheta\cos\phi&\frac12\sin2\vartheta\sin2\phi
	\end{bmatrix}$}
\end{equation*}

The inverse relation is found by inverting the matrix $\vec{D}$.

\begin{equation*}\resizebox{\linewidth}{!}{$
	\vec{D}^{-1} =\begin{bmatrix}
	 \sin^2\vartheta\cos^2\phi & \cos^2\vartheta\cos^2\phi & \sin^2\phi & -\cos\vartheta\sin2\phi & -\sin\vartheta\sin2\phi & \sin2\vartheta\cos^2\phi \\
	 \sin^2\vartheta\sin^2\phi & \cos^2\vartheta\sin^2\phi & \cos^2\phi & \cos\vartheta\sin2\phi & \sin\vartheta\sin2\phi & \sin2\vartheta\sin^2\phi\\
	 \cos^2\vartheta & \sin^2\vartheta & 0 & 0 & 0 & -\sin2\vartheta\\
	 \frac12\sin2\vartheta\sin\phi & -\frac12\sin2\vartheta\sin\phi & 0 & -\sin\vartheta\cos\phi & \cos\vartheta\cos\phi & \sin\phi\cos2\vartheta\\
	 -\sin\vartheta\sin2\phi & -\frac12\sin2\vartheta\cos\phi & 0 & \sin\vartheta\sin\phi & -\cos\vartheta\sin\phi & \cos2\vartheta\cos\phi\\
	 \frac12\sin^2\vartheta\sin2\phi & \frac12\cos^2\vartheta\sin2\phi &-\frac12\sin2\phi & \cos\vartheta\cos2\phi & \cos2\phi\sin\vartheta &\frac12\sin2\vartheta\sin2\phi
	\end{bmatrix}$}
\end{equation*}


Moreover, we have
\begin{equation}
\label{Eq2:constitutiveRelationSpherical}
	\begin{bmatrix}
		\sigma_{\mathrm{rr}}\\
		\sigma_{\upvartheta\upvartheta}\\
		\sigma_{\upphi\upphi}\\
		\sigma_{\upvartheta \upphi}\\
		\sigma_{\mathrm{r} \upphi}\\
		\sigma_{\mathrm{r}\upvartheta}\\
	\end{bmatrix} = \vec{C}
	\begin{bmatrix}
		\varepsilon_{\mathrm{rr}}\\
		\varepsilon_{\upvartheta\upvartheta}\\
		\varepsilon_{\upphi\upphi}\\
		2\varepsilon_{\vartheta \phi}\\
		2\varepsilon_{r \phi}\\
		2\varepsilon_{\mathrm{r}\upvartheta}\\
	\end{bmatrix},
\end{equation}
where (see~\cite{Slaughter2002tlt} for details)
\begin{equation}
\label{Eq2:strainsInSpherical}
\begin{split}
	\varepsilon_{\mathrm{rr}} &= \pderiv{u_{\mathrm{r}}}{r}\\
	\varepsilon_{\upvartheta\upvartheta} &= \frac{1}{r}\left(\pderiv{u_{\upvartheta}}{\vartheta} + u_{\mathrm{r}}\right)\\
	\varepsilon_{\upphi\upphi} &= \frac{1}{r\sin\vartheta}\left(\pderiv{u_{\phi}}{\phi} + u_{\mathrm{r}}\sin\vartheta + u_{\upvartheta}\cos\vartheta\right)\\
	\varepsilon_{\upvartheta\upphi} &= \frac{1}{2r}\left(\frac{1}{\sin\vartheta}\pderiv{u_{\upvartheta}}{\phi} + \pderiv{u_{\upphi}}{\vartheta} - u_{\upphi}\cot\vartheta\right)\\
	\varepsilon_{\mathrm{r}\upphi} &= \frac{1}{2}\left(\frac{1}{r\sin\vartheta}\pderiv{u_{\mathrm{r}}}{\phi} + \pderiv{u_{\upphi}}{r} - \frac{u_{\upphi}}{r}\right)\\
	\varepsilon_{\mathrm{r}\upvartheta} &= \frac{1}{2}\left(\frac{1}{r}\pderiv{u_{\mathrm{r}}}{\vartheta} + \pderiv{u_{\upvartheta}}{r} - \frac{u_{\upvartheta}}{r}\right).
\end{split}
\end{equation}

\subsection{The prolate spheroidal coordinate system}
\label{Sec2:prolateSphericalCoordinateSystem}
The prolate spheroidal coordinate system is an extension of the spherical coordinate system. It is defined by the relations
\begin{align*}
	x &= \sqrt{r^2 - f^2}\sin\vartheta\cos\phi\\
	y &= \sqrt{r^2 - f^2}\sin\vartheta\sin\phi\\
	z &= r\cos\vartheta
\end{align*}
with foci located at $z = \pm f$. Note that we define $r\geq f$ such that the coordinate system reduces to the spherical coordinate system when $f=0$. Using this condition, we may establish the following inverse formulas
\begin{align}\label{Eq2:XtoProl}
\begin{split}
	r &= \frac{1}{\sqrt{2}}\sqrt{T_f + \sqrt{T_f^2-4f^2z^2}}\\
	\vartheta &= \arccos\left(\frac{\sqrt{2}z}{\sqrt{T_f + \sqrt{T_f^2-4f^2z^2}}}\right)\\
	\phi &= \operatorname{atan2}(y,x).
\end{split}
\end{align}
where $T_f = T_f(x,y,z) = x^2+y^2+z^2+f^2$.

The derivatives are found to be
\begin{equation}\label{Eq2:dXdProlateSphericalCoordinates}
\begin{alignedat}{4}
	\pderiv{x}{r} &= \frac{r\sin\vartheta\cos\phi}{\sqrt{r^2-f^2}},\qquad	&&\pderiv{y}{r} = \frac{r\sin\vartheta\sin\phi}{\sqrt{r^2-f^2}},\qquad	&&\pderiv{z}{r} = \cos\vartheta\\
	\pderiv{x}{\vartheta} &=\sqrt{r^2-f^2}\cos\vartheta\cos\phi,\qquad	&&\pderiv{y}{\vartheta} = \sqrt{r^2-f^2}\cos\vartheta\sin\phi,\qquad	&&\pderiv{z}{\vartheta} = -r\sin\vartheta\\
	\pderiv{x}{\phi} &= -\sqrt{r^2-f^2}\sin\vartheta\sin\phi,\qquad	&&\pderiv{y}{\phi} = \sqrt{r^2-f^2}\sin\vartheta\cos\phi,\qquad	&&\pderiv{z}{\phi} =0.
\end{alignedat}
\end{equation}
and
\begin{equation}\label{Eq2:dProlateSphericalCoordinatesdX}
\begin{alignedat}{4}
	\pderiv{r}{x} &= \frac{xr}{2r^2-T_f},\qquad	&&\pderiv{r}{y} = \frac{yr}{2r^2-T_f},\qquad	&&\pderiv{r}{z} = \frac{z}{r}\frac{r^2-f^2}{2r^2-T_f}\\
	\pderiv{\vartheta}{x} &= \frac{xz}{r\sin\vartheta (2r^2-T_f)},\qquad	&&\pderiv{\vartheta}{y} = \frac{yz}{r\sin\vartheta (2r^2-T_f)},\qquad	&&\pderiv{\vartheta}{z} = \frac{1}{r\sin\vartheta}\left(\frac{z^2}{r^2}\frac{r^2-f^2}{2r^2-T_f}-1\right)\\
	\pderiv{\phi}{x} &= -\frac{y}{x^2+y^2},\qquad	&&\pderiv{\phi}{y} = \frac{x}{x^2+y^2},\qquad	&&\pderiv{\phi}{z} = 0.
\end{alignedat}
\end{equation}

Using \Cref{Eq2:ScalingLengths} we have
\begin{align*}
	h_{\mathrm{r}} &= \sqrt{\frac{r^2-f^2\cos^2\vartheta}{r^2-f^2}}\\
	h_{\upvartheta} &= \sqrt{r^2-f^2\cos^2\vartheta}\\
	h_{\upphi} &= \sqrt{r^2-f^2}\sin\vartheta	
\end{align*}
As the prolate spheroidal coordinate system is an orthogonal coordinate system, the general nabla operator developed in \Cref{Sec2:general3DcoordinateSystem} reduces to
\begin{equation*}
	\nabla = \frac{\vec{e}_{\mathrm{r}}}{h_{\mathrm{r}}} \pderiv{}{r} + \frac{\vec{e}_{\upvartheta}}{h_{\upvartheta}} \pderiv{}{\vartheta} + \frac{\vec{e}_{\upphi}}{h_{\upphi}} \pderiv{}{\phi}
\end{equation*}
The determinant of the jacobian in \Cref{Eq2:NURBSjacobian} may now be written as
\begin{equation*}
	J_1 = h_{\mathrm{r}} h_{\upvartheta} h_{\upphi} = \left(r^2-f^2\cos^2\vartheta\right)\sin\vartheta
\end{equation*}
The surface Jacobian at a given (constant) $r=\hat{r}$ is
\begin{equation*}
	J_S = h_{\upvartheta} h_{\upphi} = \sqrt{r^2-f^2\cos^2\vartheta}\sqrt{r^2-f^2}\sin\vartheta	.
\end{equation*}
Note that 
\begin{equation*}
	\lim_{\hat{r}\to\infty}J_S = \hat{r}^2\sin\vartheta.
\end{equation*}
That is, in the limit $\hat{r}\to\infty$ the surface Jacobian of the prolate spheroidal coordinate system is the same as the surface Jacobian of the spherical coordinate system.



==> contents/discoveredErrors.tex <==

\section{List of discovered errors}


\begin{itemize}
	\item In~\cite[pp. 191-192]{Ihlenburg1998fea} Ihlenburg writes that ``... We observe that no resonance peaks are formed at higher eigenmodes for the shells S05 and S15, ...''.
	
	Ihlenburg uses too few samples in the FRF plot to find the resonance peaks at higher eigenmodes.
	
	\item The original article~\cite[p. 4156]{Hughes2005iac} has a misprint in the analytic solution (equation 20). The correct solution is
\begin{equation*}
	u_{\mathrm{r}}(r) = \frac{1}{E}\frac{P R_1^2}{R_0^2 - R_1^2}\left((1-2\nu)(1+\nu)r+\frac{R_0^2(1+\nu)}{r}\right)
\end{equation*}
which can be written as \Cref{Eq2:analyticSolutionSolidCircularCylinder}.

This solution is derived in \Cref{Sec2:solidCircularCylinderSolution}. Where it is also showed that if the solution varies only with $r$ and $\vartheta$, the internal pressure loading $\cos 2\vartheta$ imposes restrictions on the parameter $\nu$. In fact, if we demand that $0\leq \nu\leq 0.5$ then $\nu = 0$ or $\nu = \frac12$.

\item In~\cite[p. 188]{Meirovitch1967ami} there is a misprint in the first eigenfrequency: $C_{01} = 1.015$ where the true value is $C_{01} = 1.0173886$. Hughes copies this misprint in~\cite{Hughes2005iac} such that he compares his result with $\omega_{01} = 53.863$ when the true value is $\omega_{01} = 54.117$. Hence, in~\cite{Cottrell2009iat} there seems to be convergence to the wrong result when this is not the case.

Moreover, the three first eigenmodes in~\cite{Hughes2005iac} does not represent the eigenmodes corresponding to the lowest eigenvalues as the book suggests in Figure 5.20.

\item There is an inconsistency in the length ($L$) of Scordelis-Lo roof in Figure 4.12 and Figure 4.13 in~\cite[pp. 125-126]{Cottrell2009iat}. Moreover, the scaling factor should rather be 20 than 200 in 4.13 in~\cite[p. 126]{Cottrell2009iat}.

\item Mulig også en feil i convergensplottet til Hughes~\cite[p. 129]{Cottrell2009iat} for $p=4$, da jeg oppnår bedre resultater her. Har opplevd tilsvarende fenomener når et sett med gausspunkt har en marginal feil.

\end{itemize}

==> contents/gaussImplications.tex <==
\section{Gauss theorem and its implications}
Gauss theorem is given by
\begin{equation}\label{Eq2:GaussTheorem}
	\oint_{\partial\V} \vec{\Psi}\cdot\vec{n}\idiff S = \int_\V\nabla\cdot \vec{\Psi}\idiff\V.
\end{equation}

\subsection{Gauss theorem for scalar functions}
Let $\{\vec{e}_i\}_{i=1,2,3}$ be the standard basis for the euclidean space and let $\vec{\Psi}=\psi\vec{e}_i$ for some $i\in\{1,2,3\}$. Then
\begin{align*}
	\oint_{\partial\V} \psi\vec{e}_i\cdot\vec{n}\idiff S &= \int_\V\nabla\cdot \psi\vec{e}_i\idiff\V\\
	&\Updownarrow\\
	\oint_{\partial\V} \psi n_i\idiff S &= \int_\V\partial_{x_i} \psi\idiff\V.
\end{align*}
Since this holds for all $i\in\{1,2,3\}$, we have three equations which we may combine as follows
\begin{align}\notag
	\left\{\oint_{\partial\V} \psi n_1\idiff S,\oint_{\partial\V} \psi n_2\idiff S,\oint_{\partial\V} \psi n_3\idiff S\right\} &=
	\left\{\int_\V\partial_{x_1} \psi\idiff\V,\int_\V\partial_{x_2} \psi\idiff\V,\int_\V\partial_{x_3} \psi\idiff\V\right\}\\ \notag
	&\Updownarrow\\ \notag
	\oint_{\partial\V}\psi\left\{n_1,n_2,n_3\right\}\idiff S &=
	\int_\V\left\{\partial_{x_1} \psi,\partial_{x_2} \psi,\partial_{x_3} \psi\right\}\idiff\V\\ \notag
	&\Updownarrow\\ \label{Eq2:GaussImplication}
	\oint_{\partial\V}\psi\vec{n}\idiff S &=
	\int_\V\nabla \psi\idiff\V.
\end{align}

\subsection{Green's first identity}
Green's first identity is simply Gauss theorem applied to $\vec{\Psi}=\psi\vec{\Phi}$ where $\vec{\Phi}=\nabla\phi$. Insertion of the identity
\begin{equation*}
	\nabla\cdot(\psi\vec{\Phi}) = \nabla\psi\cdot\vec{\Phi} + \psi\nabla\cdot\vec{\Phi}
\end{equation*}
into Gauss theorem yields
\begin{equation}
	\label{Eq2:GaussImplication2}
	\int_\Omega\psi\nabla\cdot\vec{\Phi}\idiff\V = -\int_\Omega\nabla\psi\cdot\vec{\Phi}\idiff\V + \int_{\partial\Omega} \psi\vec{\Phi}\cdot \vec{n}\idiff S.
\end{equation}
As $\nabla\cdot\vec{\Phi}=\nabla\cdot\nabla\phi=\nabla^2\phi$, we arrive at Green's first identity
\begin{equation}\label{Eq2:GreensFirstIdentity}
	\int_\Omega\psi\nabla^2\phi\idiff\V = -\int_\Omega\nabla\psi\cdot\nabla\phi\idiff\V + \int_{\partial\Omega}\psi\nabla\phi\cdot \vec{n}\idiff S.
\end{equation}


==> contents/infiniteElementsBilinearForm_old.tex <==
\section{Derivation of bilinear form in infinite elements}
In this appendix we will separate the integrals in the bilinear forms for the infinite elements\footnote{As we mainly use the PGU formulation in this work, we restrict ourselves to the derivation of this formulation. The other three formulations has been derived in~\cite{Venas2015iao}. For the more general ellipsoidal coordinate system, we refer to~\cite{Burnett1998aea}.}. For generality, we do this derivation in the prolate spheroidal coordinate system.
\subsection{The prolate spheroidal coordinate system}
\label{Sec2:prolateSphericalCoordinateSystem}
The prolate spheroidal coordinate system is an extension of the spherical coordinate system. It is defined by the relations
\begin{align*}
	x &= \sqrt{r^2 - \Upsilon^2}\sin\vartheta\cos\varphi\\
	y &= \sqrt{r^2 - \Upsilon^2}\sin\vartheta\sin\varphi\\
	z &= r\cos\vartheta
\end{align*}
with foci located at $z = \pm \Upsilon$. Note that we define $r\geq \Upsilon$ such that the coordinate system reduces to the spherical coordinate system when $\Upsilon=0$. Using this condition, we may establish the following inverse formulas
\begin{align}\label{Eq2:XtoProl}
\begin{split}
	r &= \frac{1}{2}\left(\sqrt{T_\Upsilon-2z\Upsilon}+\sqrt{T_\Upsilon+2z\Upsilon}\right)\\
	\vartheta &= \arccos\left(\frac{z}{r}\right)\\
	\varphi &= \operatorname{atan2}(y,x)
\end{split}
\end{align}
where $T_\Upsilon = T_\Upsilon(x,y,z) = x^2+y^2+z^2+\Upsilon^2$ and 
\begin{equation*}
	\operatorname{atan2}(y,x) = \begin{cases}
	\arctan(\frac{y}{x}) & \mbox{if } x > 0\\
	\arctan(\frac{y}{x}) + \PI & \mbox{if } x < 0 \mbox{ and } y \ge 0\\
	\arctan(\frac{y}{x}) - \PI & \mbox{if } x < 0 \mbox{ and } y < 0\\
	\frac{\PI}{2} & \mbox{if } x = 0 \mbox{ and } y > 0\\
	-\frac{\PI}{2} & \mbox{if } x = 0 \mbox{ and } y < 0\\
	\text{undefined} & \mbox{if } x = 0 \mbox{ and } y = 0.
	\end{cases}
\end{equation*}
The derivatives are found to be
\begin{equation}\label{Eq2:dXdProlateSphericalCoordinates}
\begin{alignedat}{4}
	\pderiv{x}{r} &= \frac{r\sin\vartheta\cos\varphi}{\sqrt{r^2-\Upsilon^2}},\qquad	&&\pderiv{y}{r} = \frac{r\sin\vartheta\sin\varphi}{\sqrt{r^2-\Upsilon^2}},\qquad	&&\pderiv{z}{r} = \cos\vartheta\\
	\pderiv{x}{\vartheta} &=\sqrt{r^2-\Upsilon^2}\cos\vartheta\cos\varphi,\qquad	&&\pderiv{y}{\vartheta} = \sqrt{r^2-\Upsilon^2}\cos\vartheta\sin\varphi,\qquad	&&\pderiv{z}{\vartheta} = -r\sin\vartheta\\
	\pderiv{x}{\varphi} &= -\sqrt{r^2-\Upsilon^2}\sin\vartheta\sin\varphi,\qquad	&&\pderiv{y}{\varphi} = \sqrt{r^2-\Upsilon^2}\sin\vartheta\cos\varphi,\qquad	&&\pderiv{z}{\varphi} =0
\end{alignedat}
\end{equation}
and
\begin{equation}\label{Eq2:dProlateSphericalCoordinatesdX}
\begin{alignedat}{4}
	\pderiv{r}{x} &= \frac{xr}{2r^2-T_\Upsilon},\qquad	&&\pderiv{r}{y} = \frac{yr}{2r^2-T_\Upsilon},\qquad	&&\pderiv{r}{z} = \frac{z}{r}\frac{r^2-\Upsilon^2}{2r^2-T_\Upsilon}\\
	\pderiv{\vartheta}{x} &= \frac{xz}{r\sin\vartheta (2r^2-T_\Upsilon)},\qquad	&&\pderiv{\vartheta}{y} = \frac{yz}{r\sin\vartheta (2r^2-T_\Upsilon)},\qquad	&&\pderiv{\vartheta}{z} = \frac{1}{r\sin\vartheta}\left(\frac{z^2}{r^2}\frac{r^2-\Upsilon^2}{2r^2-T_\Upsilon}-1\right)\\
	\pderiv{\varphi}{x} &= -\frac{y}{x^2+y^2},\qquad	&&\pderiv{\varphi}{y} = \frac{x}{x^2+y^2},\qquad	&&\pderiv{\varphi}{z} = 0.
\end{alignedat}
\end{equation}
With the notation
\begin{align*}
	h_{\mathrm{r}} &= \sqrt{\frac{r^2-\Upsilon^2\cos^2\vartheta}{r^2-\Upsilon^2}}\\
	h_{\upvartheta} &= \sqrt{r^2-\Upsilon^2\cos^2\vartheta}\\
	h_{\upvarphi} &= \sqrt{r^2-\Upsilon^2}\sin\vartheta	
\end{align*}
the general nabla operator can be written as
\begin{equation*}
	\nabla = \frac{\vec{e}_{\mathrm{r}}}{h_{\mathrm{r}}} \pderiv{}{r} + \frac{\vec{e}_{\upvartheta}}{h_{\upvartheta}} \pderiv{}{\vartheta} + \frac{\vec{e}_{\upvarphi}}{h_{\upvarphi}} \pderiv{}{\varphi}
\end{equation*}
where
\begin{equation*}
	\vec{e}_{\mathrm{r}} = \frac{1}{h_{\mathrm{r}}}\left[\pderiv{x}{r}, \pderiv{y}{r}, \pderiv{z}{r}\right]^\transpose,\qquad
	\vec{e}_{\upvartheta} = \frac{1}{h_{\upvartheta}}\left[\pderiv{x}{\vartheta}, \pderiv{y}{\vartheta}, \pderiv{z}{\vartheta}\right]^\transpose,\qquad
	\vec{e}_{\upvarphi} = \frac{1}{h_{\upvarphi}}\left[\pderiv{x}{\varphi}, \pderiv{y}{\varphi}, \pderiv{z}{\varphi}\right]^\transpose.
\end{equation*}
The Jacobian determinant (for the mapping from Cartesian coordinates to prolate spheroidal coordinates) may now be written as
\begin{equation*}
	J_1 = h_{\mathrm{r}} h_{\upvartheta} h_{\upvarphi} = \left(r^2-\Upsilon^2\cos^2\vartheta\right)\sin\vartheta.
\end{equation*}
By noting that any normal vector at a surface with constant radius $r=\gamma$ can be written as $\vec{n} = \vec{e}_{\upvartheta}\times\vec{e}_{\upphi}=\vec{e}_{\mathrm{r}}$ we get
\begin{equation*}
	\partial_n p = \vec{n}\cdot\nabla p = \vec{e}_{\mathrm{r}}\cdot\nabla p = \frac{1}{h_{\mathrm{r}}} \pderiv{p}{r}.
\end{equation*}
The surface Jacobian determinant at a given (constant) $r=\gamma$ is
\begin{equation*}
	J_S = h_{\upvartheta} h_{\upvarphi} = \sqrt{r^2-\Upsilon^2\cos^2\vartheta}\sqrt{r^2-\Upsilon^2}\sin\vartheta	.
\end{equation*}
and we may therefore note that
\begin{equation*}
	q\partial_n p J_S = \bigoh\left(r^{-3}\right)\quad\text{whenever}\quad q=\bigoh\left(r^{-3}\right)\quad\text{and}\quad p = \bigoh\left(r^{-1}\right).
\end{equation*}
That is, for the Petrov--Galerkin formulations we have
\begin{equation*}
	\lim_{\gamma\to\infty}\int_{S^\gamma} q\partial_n p\idiff\Gamma = \lim_{\gamma\to\infty}\int_0^{2\PI}\int_0^\PI q\partial_n p J_S\idiff\vartheta\idiff\varphi = 0.
\end{equation*}

\subsection{Bilinear form}
The bilinear form (in the domain outside the artificial boundary) in~\Cref{Eq2:B_uc_a} (in the unconjugated case) can in the Petrov--Galerkin formulations be simplified to
\begin{align}\label{Eq2:BilinearFormInserted}
	\begin{split}
	B_{\mathrm{uc},\mathrm{a}}(R_I\psi_n,R_J\phi_m) &= \lim_{\gamma\to\infty}\int_{\Omega_{\mathrm{a}}^\gamma} \left[\nabla(R_I\psi_n)\cdot \nabla (R_J\phi_m)- k^2 R_I\psi_n R_J\phi_m\right]\idiff\Omega\\
		&=\int_{\Omega_{\mathrm{a}}^+} \left[\nabla(R_I\psi_n)\cdot \nabla (R_J\phi_m)- k^2 R_I\psi_n R_J\phi_m\right]\idiff\Omega
	\end{split}
\end{align}
as the mentioned surface integral in the far-field vanishes (this is however not the case for the Bubnov--Galerkin formulations). With the summation convention (over the indices $\tilde{n}$ and $\tilde{m}$) we can write
\begin{equation*}
	\psi_n = \euler^{\imag k(r-r_n)}\frac{\tilde{D}_{n\tilde{n}}}{r^{\tilde{n}+2}}\quad\text{and}\quad\phi_m = \euler^{\imag k(r-r_m)}\frac{D_{m\tilde{m}}}{r^{\tilde{m}}}.
\end{equation*}
Using the expression for the nabla operator found in \Cref{Sec2:prolateSphericalCoordinateSystem} we get
\begin{align*}
	\nabla(R_I\psi_n)\cdot \nabla (R_J\phi_m) &= \frac{1}{h_{\mathrm{r}}^2}\pderiv{(R_I\psi_n)}{r}\pderiv{(R_J\phi_m)}{r} + \frac{1}{h_{\upvartheta}^2}\pderiv{(R_I\psi_n)}{\vartheta}\pderiv{(R_J\phi_m)}{\vartheta} + \frac{1}{h_{\upvarphi}^2}\pderiv{(R_I\psi_n)}{\varphi}\pderiv{(R_J\phi_m)}{\varphi}\\
	 &= \frac{1}{h_{\mathrm{r}}^2}\pderiv{\psi_n}{r}\pderiv{\phi_m}{r}R_IR_J + \frac{1}{h_{\upvartheta}^2}\pderiv{R_I}{\vartheta}\pderiv{R_J}{\vartheta}\phi_m\psi_n + \frac{1}{h_{\upvarphi}^2}\pderiv{R_I}{\varphi}\pderiv{R_J}{\varphi}\psi_n\phi_m\\
	 &=  \left(\imag k - \frac{\tilde{n}+2}{r}\right)\left(\imag k - \frac{\tilde{m}}{r}\right)\frac{\euler^{2\imag k r}\euler^{-\imag k (r_n+r_m)}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}}{r^{\tilde{n}+\tilde{m}+2}h_{\mathrm{r}}^2}R_I R_J \\
	 &\quad+ \frac{\euler^{2\imag k r}\euler^{-\imag k (r_n+r_m)}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}}{h_{\upvartheta}^2 r^{\tilde{n}+\tilde{m}+2}}\pderiv{R_I}{\vartheta}\pderiv{R_J}{\vartheta} + \frac{\euler^{2\imag k r}\euler^{-\imag k (r_n+r_m)}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}}{h_{\upvarphi}^2 r^{\tilde{n}+\tilde{m}+2}}\pderiv{R_I}{\varphi}\pderiv{R_J}{\varphi}\\
	 &= \left[\frac{(r^2-\Upsilon^2)\left[-(kr)^2 - \imag kr(\tilde{n}+\tilde{m}+2) + (\tilde{n}+2)\tilde{m}\right]}{r^2(r^2-\Upsilon^2\cos^2\vartheta)}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}R_I R_J\right.\\ 
	 &\qquad\left.+ \frac{1}{r^2-\Upsilon^2\cos^2\vartheta}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\pderiv{R_I}{\vartheta}\pderiv{R_J}{\vartheta} \right.\\
	 &\qquad\left.+ \frac{1}{(r^2-\Upsilon^2)\sin^2\vartheta}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\pderiv{R_I}{\varphi}\pderiv{R_J}{\varphi}\right]\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}
\end{align*}
which multiplied with the Jacobian $J_1$ yields
\begin{align*}
	\nabla(R_I\psi_n)\cdot \nabla (R_J\phi_m) J_1&= \left[\frac{(r^2-\Upsilon^2)\left[-(kr)^2 - \imag kr(\tilde{n}+\tilde{m}+2) + (\tilde{n}+2)\tilde{m}\right]}{r^2}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\sin\vartheta R_I R_J\right.\\ 
	&\qquad+ \left.\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\sin\vartheta \pderiv{R_I}{\vartheta}\pderiv{R_J}{\vartheta} \right.\\
	&\qquad+\left. \frac{(r^2-\Upsilon^2\cos^2\vartheta)}{(r^2-\Upsilon^2)\sin\vartheta}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\pderiv{R_I}{\varphi}\pderiv{R_J}{\varphi}\right]\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}
\end{align*}
Also note that the term contributing to the mass matrix multiplied with the same Jacobian is given by
\begin{equation*}
	k^2R_I\psi_n R_J\phi_m J_1 = \frac{k^2\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}} (r^2-\Upsilon^2\cos^2\vartheta)\sin\vartheta R_I R_J\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}.
\end{equation*}
Combining all of this into \Cref{Eq2:BilinearFormInserted} yields
\begin{align*}
	B_{\mathrm{uc},\mathrm{a}}(R_I\psi_n,R_J\phi_m) =&\left\{\int_{r_{\mathrm{a}}}^{\infty}\left[-\frac{k^2}{r^{\tilde{n}+\tilde{m}}} - \frac{\imag k(\tilde{n}+\tilde{m}+2)}{r^{\tilde{n}+\tilde{m}+1}} +\frac{(\tilde{n}+2)\tilde{m}+\Upsilon^2k^2}{r^{\tilde{n}+\tilde{m}+2}}\right.\right.\\
	&\left.\left.\quad\qquad + \frac{\imag k \Upsilon^2 (\tilde{n}+\tilde{m}+2)}{r^{\tilde{n}+\tilde{m}+3}} - \frac{(\tilde{n}+2)\tilde{m}\Upsilon^2}{r^{\tilde{n}+\tilde{m}+4}}\right]\euler^{2\imag k r}\idiff r \int_0^{2\PI}\int_0^\PI R_I R_J\sin\vartheta\idiff\vartheta\idiff\varphi\right.\\
	&\left.\quad +\int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\idiff r\int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\vartheta} \pderiv{R_J}{\vartheta}\sin\vartheta\idiff\vartheta\idiff\varphi\right.\\
	&\left.\quad +\int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}}{(r^2-\Upsilon^2)r^{\tilde{n}+\tilde{m}}}\idiff r\int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\varphi} \pderiv{R_J}{\varphi}\frac{1}{\sin\vartheta}\idiff\vartheta\idiff\varphi \right.\\
	&\left.\quad- \int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}\Upsilon^2}{(r^2-\Upsilon^2)r^{\tilde{n}+\tilde{m}+2}}\idiff r\int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\varphi} \pderiv{R_J}{\varphi}\frac{\cos^2\vartheta}{\sin\vartheta}\idiff\vartheta\idiff\varphi \right.\\
	&\left.\quad- \int_{r_{\mathrm{a}}}^{\infty}\frac{k^2\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}}}\idiff r\int_0^{2\PI}\int_0^\PI R_I R_J\sin\vartheta\idiff\vartheta\idiff\varphi\right.\\
	&\left.\quad+ \int_{r_{\mathrm{a}}}^{\infty}\frac{k^2\Upsilon^2\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\idiff r\int_0^{2\PI}\int_0^\PI R_I R_J\cos^2\vartheta\sin\vartheta\idiff\vartheta\idiff\varphi\right\}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}.
\end{align*}
Defining the angular integrals
\begin{equation}\label{Eq2:infiniteElementsSurfaceIntegrals}
\begin{alignedat}{2}
	& A_{IJ}^{(1)} = \int_0^{2\PI}\int_0^\PI R_I R_J\sin\vartheta\idiff\vartheta\idiff\varphi,\qquad\qquad && A_{IJ}^{(2)} = \int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\vartheta} \pderiv{R_J}{\vartheta}\sin\vartheta\idiff\vartheta\idiff\varphi\\
	& A_{IJ}^{(3)} = \int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\varphi} \pderiv{R_J}{\varphi}\frac{1}{\sin\vartheta}\idiff\vartheta\idiff\varphi, \quad && A_{IJ}^{(4)} = \int_0^{2\PI}\int_0^\PI \pderiv{R_I}{\varphi} \pderiv{R_J}{\varphi}\frac{\cos^2\vartheta}{\sin\vartheta}\idiff\vartheta\idiff\varphi\\
	& A_{IJ}^{(5)} = \int_0^{2\PI}\int_0^\PI R_I R_J\cos^2\vartheta\sin\vartheta\idiff\vartheta\idiff\varphi
\end{alignedat}	
\end{equation}
we can write
\begin{align*}
	B_{\mathrm{uc},\mathrm{a}}(R_I\psi_n,R_J\phi_m) =&\left\{A_{IJ}^{(1)}\int_{r_{\mathrm{a}}}^{\infty}\left[-\frac{k^2}{r^{\tilde{n}+\tilde{m}}} - \frac{\imag k(\tilde{n}+\tilde{m}+2)}{r^{\tilde{n}+\tilde{m}+1}} +\frac{(\tilde{n}+2)\tilde{m}+\Upsilon^2k^2}{r^{\tilde{n}+\tilde{m}+2}}\right.\right.\\
	&\left.\left.\quad\qquad\qquad + \frac{\imag k \Upsilon^2 (\tilde{n}+\tilde{m}+2))}{r^{\tilde{n}+\tilde{m}+3}} - \frac{(\tilde{n}+2)\tilde{m}\Upsilon^2}{r^{\tilde{n}+\tilde{m}+4}}\right]\euler^{2\imag k r}\idiff r\right.\\
	&\left.\quad + A_{IJ}^{(2)}\int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\idiff r +A_{IJ}^{(3)}\int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}}{(r^2-\Upsilon^2)r^{\tilde{n}+\tilde{m}}}\idiff r\right.\\
	&\left.\quad - A_{IJ}^{(4)}\int_{r_{\mathrm{a}}}^{\infty}\frac{\euler^{2\imag k r}\Upsilon^2}{(r^2-\Upsilon^2)r^{\tilde{n}+\tilde{m}+2}}\idiff r\right.\\
	&\left.\quad- A_{IJ}^{(1)}\int_{r_{\mathrm{a}}}^{\infty}\frac{k^2\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}}}\idiff r + A_{IJ}^{(5)}\int_{r_{\mathrm{a}}}^{\infty}\frac{k^2\Upsilon^2\euler^{2\imag k r}}{r^{\tilde{n}+\tilde{m}+2}}\idiff r\right\}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}.
\end{align*}
Integrals of the form
\begin{equation*}
	\int_{r_{\mathrm{a}}}^\infty\frac{\euler^{2\imag k r}}{r^n}\idiff r,\quad n\geq 1
\end{equation*}
and
\begin{equation}\label{Eq2:2ndIntegralType}
	\int_{r_{\mathrm{a}}}^\infty\frac{\euler^{2\imag k r}}{(r^2-\Upsilon^2)r^n}\idiff r, \quad n\geq 0
\end{equation}
can be evaluated using the algorithms presented in \Cref{Sec2:radIntegrals}. Using the following notation for the radial integrals
\begin{equation*}
	B_{n}^{(1)} = \int_{r_{\mathrm{a}}}^\infty \frac{\euler^{2\imag k r}}{r^n}\idiff r \qquad B_{n}^{(2)} = \int_{r_{\mathrm{a}}}^\infty \frac{\euler^{2\imag k r}}{(r^2-\Upsilon^2)r^{n-1}}\idiff r,\qquad n\geq 1
\end{equation*}
we may now finally write the bilinear form as
\begin{align}\label{Eq2:finalBilinearFormB_uc_a}
\begin{split}
	B_{\mathrm{uc},\mathrm{a}}(R_I\psi_n,R_J\phi_m) = &\sum_{\tilde{n}=1}^N\sum_{\tilde{m}=1}^N\left\{A_{IJ}^{(1)}\left[-2k^2B_{\tilde{n}+\tilde{m}}^{(1)}-\imag k(\tilde{n}+\tilde{m}+2)B_{\tilde{n}+\tilde{m}+1}^{(1)} \right.\right.\\
	&\left.\left.\qquad\qquad\qquad + \left((\tilde{n}+2)\tilde{m}+\Upsilon^2k^2\right)B_{\tilde{n}+\tilde{m}+2}^{(1)} \right.\right.\\
	&\left.\left.\qquad\qquad\qquad + \imag k \Upsilon^2(\tilde{n}+\tilde{m}+2)B_{\tilde{n}+\tilde{m}+3}^{(1)}-(\tilde{n}+2)\tilde{m} \Upsilon^2 B_{\tilde{n}+\tilde{m}+4}^{(1)}\right]\right.\\
	&\left.\qquad\qquad + A_{IJ}^{(2)} B_{\tilde{n}+\tilde{m}+2}^{(1)} +A_{IJ}^{(3)}B_{\tilde{n}+\tilde{m}+1}^{(2)} - A_{IJ}^{(4)} \Upsilon^2B_{\tilde{n}+\tilde{m}+3}^{(2)} \right.\\
	&\left.\qquad\qquad + A_{IJ}^{(5)} k^2 \Upsilon^2 B_{\tilde{n}+\tilde{m}+2}^{(1)}\right\}\tilde{D}_{n\tilde{n}}D_{m\tilde{m}}\euler^{-\imag k (r_n+r_m)}.
\end{split}
\end{align}
We typically parameterize the domain such that the artificial boundary $\Gamma_{\mathrm{a}}$ is parameterized by $\xi$ and $\eta$ at $\zeta=1$ (which is at $r_{\mathrm{a}}$ in the prolate spheroidal coordinates). As $\Gamma_{\mathrm{a}}$ is a surface with constant radius, $r=r_{\mathrm{a}}$, in the prolate spheroidal coordinate system, it may also be parametrized by $\vartheta$ and $\varphi$. We therefore have
\begin{equation}
	\diff \vartheta\diff\varphi = \begin{vmatrix}
		\pderiv{\vartheta}{\xi} & \pderiv{\varphi}{\xi}\\
		\pderiv{\vartheta}{\eta} & \pderiv{\varphi}{\eta}		
	\end{vmatrix}\diff\xi\diff\eta
\end{equation}
where
\begin{align*}
	\pderiv{\vartheta}{\xi} &= \pderiv{\vartheta}{x}\pderiv{x}{\xi} + \pderiv{\vartheta}{y}\pderiv{y}{\xi} + \pderiv{\vartheta}{z}\pderiv{z}{\xi},\qquad
	\pderiv{\vartheta}{\eta} = \pderiv{\vartheta}{x}\pderiv{x}{\eta} + \pderiv{\vartheta}{y}\pderiv{y}{\eta} + \pderiv{\vartheta}{z}\pderiv{z}{\eta}\\
	\pderiv{\varphi}{\xi} &= \pderiv{\varphi}{x}\pderiv{x}{\xi} + \pderiv{\varphi}{y}\pderiv{y}{\xi} + \pderiv{\varphi}{z}\pderiv{z}{\xi},\qquad
	\pderiv{\varphi}{\eta} = \pderiv{\varphi}{x}\pderiv{x}{\eta} + \pderiv{\varphi}{y}\pderiv{y}{\eta} + \pderiv{\varphi}{z}\pderiv{z}{\eta}
\end{align*}
where the inverse partial derivatives with respect to the coordinate transformation\footnote{From the prolate spheroidal coordinate system to the Cartesian coordinate system.\label{Fn:CartToProl}} is found in \Cref{Eq2:dProlateSphericalCoordinatesdX}. This Jacobian matrix may be evaluated by
\begin{equation*}
	J_3 = \begin{bmatrix}
		\pderiv{\vartheta}{\xi} & \pderiv{\vartheta}{\eta}\\
		\pderiv{\varphi}{\xi}	 & \pderiv{\varphi}{\eta}
	\end{bmatrix} = \begin{bmatrix}
		\pderiv{\vartheta}{x} & \pderiv{\vartheta}{y} & \pderiv{\vartheta}{z}\\
		\pderiv{\varphi}{x} & \pderiv{\varphi}{y} & \pderiv{\varphi}{z}
	\end{bmatrix}\begin{bmatrix}
		\pderiv{x}{\xi} & \pderiv{x}{\eta}\\
		\pderiv{y}{\xi} & \pderiv{y}{\eta}\\
		\pderiv{z}{\xi} & \pderiv{z}{\eta}
	\end{bmatrix}
\end{equation*}
and the derivatives of the basis functions may be computed by
\begin{equation*}
	\begin{bmatrix}
		\pderiv{R_A}{\vartheta}\\
		\pderiv{R_A}{\varphi}
	\end{bmatrix} = J_3^{-\transpose}\begin{bmatrix}
		\pderiv{R_A}{\xi}\\
		\pderiv{R_A}{\eta}	
	\end{bmatrix}.
\end{equation*}

==> contents/physicalProblem.tex <==
\section{Governing physical equations}
\label{Sec2:physicalProblem}
The problem at hand is obviously time dependent. But we shall assume harmonic time dependency, such that all scalar function $\hat{F}=\hat{F}(\vec{x},t)$ may be written
\begin{equation}\label{Eq2:periodicityAssumption}
	\hat{F}(\vec{x}, t) = F(\vec{x})\euler^{-\imag\omega t}
\end{equation}
and corresponding for vector fields $\hat{\vec{F}} = \hat{\vec{F}}(\vec{x},t)$
\begin{equation*}
	\hat{\vec{F}}(\vec{x},t) = \vec{F}(\vec{x})\euler^{-\imag\omega t}
\end{equation*}
where $\omega$ is the angular frequency. We refer to this assumption as the \textit{harmonic time dependency assumption}. The sign in the exponential factor is just a matter of convention. Burnett uses $\euler^{\imag\omega t}$ in~\cite{Burnett1994atd}, while Ihlenburg uses $\euler^{-\imag\omega t}$ in~\cite{Ihlenburg1998fea}. In this thesis, we shall use the convention after Ihlenburg.

We start by following~\cite[pp. 1-4]{Ihlenburg1998fea} in presenting the physical equation for the problem at hand.

\subsection{Acoustic waves}
The fluid domain to be considered is homogeneous throughout the domain, and we shall use simplifying assumption including linearization to end up with the wave equation. From here, we move from the time domain to the frequency domain when using the harmonic time dependency assumption.

\subsubsection{The continuity equation}
Let $\V$ be a volume element in the fluid domain with boundary $\partial \V$ and outward normal vector $\vec{n}(\vec{x})$ where $\vec{x}\in\partial\V$. Denote by $\rho(\vec{x},t)$ and $\vec{V}(\vec{x},t)$, the mass density of the fluid in $\V$ and the velocity field of the fluid, respectively. Then, $\vec{V}\cdot\vec{n}$ denotes the velocity of the normal flux out of $\V$ through the boundary $\partial \V$. Conservation of mass in $\V$ then yields
\begin{equation}\label{Eq2:conservationOfMass}
	\pderiv{}{t}\int_\V \rho\idiff\V = -\oint \rho\left(\vec{V}\cdot \vec{n}\right)\idiff S.
\end{equation}
Gauss theorem in \Cref{Eq2:GaussTheorem} let us rewrite the right hand side as
\begin{equation*}
	\oint \rho\left(\vec{V}\cdot \vec{n}\right)\idiff S = \oint \left(\rho\vec{V}\right)\cdot\vec{n}\idiff S = \int_\V\nabla\cdot \left(\rho\vec{V}\right)\idiff\V
\end{equation*}
such that \Cref{Eq2:conservationOfMass} may be written as
\begin{equation*}
	\int_\V \pderiv{\rho}{t}+\nabla\cdot\left(\rho\vec{V}\right)\idiff\V = 0.
\end{equation*}
As conservation of mass is supposed to hold for any (smooth enough) domain $\V$ it means it has to be valid pointwise and we thus end up with the \textit{continuity equation}
\begin{equation}\label{Eq2:continuityEquation}
	 \pderiv{\rho}{t}+\nabla\cdot\left(\rho\vec{V}\right) = 0.
\end{equation}

\subsubsection{Equation of motion}
Newton's second law of motion implies that we have conservation of momentum. Thus, any change of momentum in the control volume $\V$ must either be due to the momentum leaving or entering the control volume, or the acts of external surface/volume forces acting on the control volume. Mathematically, this may be written as
\begin{equation}\label{Eq2:ConservationOfMoment}
	\pderiv{}{t}\int_\V\rho\vec{V}\idiff\V = -\oint_{\partial \V} (\rho \vec{V})(\vec{V}\cdot \vec{n})\idiff S -\oint_{\partial \V}P(\vec{x},t)\vec{n}\idiff S + \int_\V \rho \vec{g}\idiff\V
\end{equation}
were we have neglected viscous forces (note that this is a vector equation). The $i^{\textnormal{th}}$ component of the first term on the right hand side may (using Gauss theorem in \Cref{Eq2:GaussTheorem}) be written as
\begin{equation*}
	\oint_{\partial \V} (\rho  V_i)\vec{V}\cdot \vec{n}\idiff\V = \oint_{\partial \V} (\rho  V_i\vec{V})\cdot \vec{n}\idiff\V = \int_\V\nabla\cdot (\rho  V_i\vec{V})\idiff\V
\end{equation*}
where $V_i$ denotes the $i^{\textnormal{th}}$ component of $\vec{V}$. Using \Cref{Eq2:GaussImplication}, we have
\begin{equation*}
	\oint_{\partial \V}P(\vec{x},t)\vec{n}\idiff S = \int_\V\nabla P(\vec{x},t)\idiff\V.
\end{equation*}
Combining these surface integral transformations we may write the $i^{\textnormal{th}}$ component of \Cref{Eq2:ConservationOfMoment} as
\begin{equation*}
	\int_\V\pderiv{(\rho V_i)}{t}-\nabla\cdot (\rho  V_i\vec{V}) + \nabla_i P(\vec{x},t)-\rho \vec{g}_i\idiff\V = 0.
\end{equation*}
Using the same argument as before we get
\begin{equation*}
	\pderiv{(\rho V_i)}{t}-\nabla\cdot (\rho  V_i\vec{V}) = -\nabla_i P(\vec{x},t) + \rho \vec{g}_i.
\end{equation*}
Expanding left hand side yields
\begin{equation*}
	\rho\pderiv{ V_i}{t}+\pderiv{\rho}{t} V_i+\nabla\cdot (\rho\vec{V}) V_i+  (\rho \vec{V}) \cdot\nabla V_i= -\nabla_i P + \rho \vec{g}_i.
\end{equation*}
such that we may use \Cref{Eq2:conservationOfMass} to eliminate the second and third term of left hand side
\begin{equation*}
	\rho\pderiv{ V_i}{t}+ (\rho \vec{V}) \cdot\nabla V_i= -\nabla_i P + \rho \vec{g}_i.
\end{equation*}
Combining all components we arrive at \textit{Euler's equation}
\begin{equation}\label{Eq2:EulerEquation}
	\rho\pderiv{\vec{V}}{t}+ \rho (\vec{V}\cdot\nabla)\vec{V}= -\nabla P + \rho \vec{g}.
\end{equation}
\subsubsection{Helmholtz equation}
We first need to linearize the continuity equation in \Cref{Eq2:continuityEquation} and Euler's equation in \Cref{Eq2:EulerEquation}. This is done by setting
\begin{equation}\label{Eq2:linearizedExpressions}
	P=P_0+P_1,\quad\rho=\rho_0+\rho_1,\quad\text{and}\quad\vec{V}=\vec{V}_0+\vec{V}_1
\end{equation}
where parameters with subscript 0 is equilibrium parameters and parameters with subscript 1 refer to small perturbed parameters. That is, we assume there is only a small perturbation of a background field for the pressure, density and the velocity field. Assuming there is no background velocity, we have $\vec{V}_0=\zerovec$. We shall also assume the background density to be constant, such that
\begin{equation*}
	\pderiv{\rho_0}{t} = 0\quad\text{and}\quad\nabla\rho_0 = \zerovec.
\end{equation*}
The background pressure field can only be due to the hydrostatic pressure from the gravity force density ($\rho\vec{g} = -\rho g \vec{e}_3$)  such that we have
\begin{equation*}
	P_0 = P_{\mathrm{a}} - \rho z g.
\end{equation*}
where $P_{\mathrm{a}}$ is the (constant) background pressure at $z=0$. This implies that
\begin{equation*}
	\pderiv{P_0}{t} = 0\quad\text{and}\quad \nabla P_0 = \rho\vec{g}.
\end{equation*}
Euler's equation thus simplifies to
\begin{equation}\label{Eq2:simplifiedEulerEquation}
	\rho\pderiv{\vec{V}}{t}+ \rho (\vec{V}\cdot\nabla)\vec{V}= -\nabla P_1.
\end{equation}
The linearization procedure is then completed by inserting the expression in \Cref{Eq2:linearizedExpressions}, and neglect the terms of second order or higher. For the continuity equation in \Cref{Eq2:continuityEquation}, we have
\begin{equation*}
	 \pderiv{\rho_1}{t}+\nabla\cdot\left((\rho_0+\rho_1)\vec{V}_1\right) = 0 
\end{equation*}
which after linearization yields the \textit{linearized version} of the continuity equation
\begin{equation}\label{Eq2:linearizedContinuityEquation}
	 \pderiv{\rho_1}{t}+\rho_0\nabla\cdot\vec{V}_1 = 0.
\end{equation}
For the simplified Euler equation in \Cref{Eq2:simplifiedEulerEquation} we get
\begin{equation*}
	(\rho_0+\rho_1)\pderiv{\vec{V}_1}{t}+ \rho (\vec{V}_1\cdot\nabla)\vec{V}_1 = -\nabla P_1
\end{equation*}
which after linearization yields the \textit{linearized version} of the Euler equation
\begin{equation}\label{Eq2:linearizedEulerEquation}
	\rho_0\pderiv{\vec{V}_1}{t} = -\nabla P_1.
\end{equation}
We shall assume a linear material law, 
\begin{equation*}
	P = c^2\rho\qquad \Rightarrow\qquad \pderiv{P_1}{t} = c^2\pderiv{\rho_1}{t},
\end{equation*}
where $c$ is the speed of sound (material parameter which we assume to be constant). Using \Cref{Eq2:linearizedContinuityEquation} and \Cref{Eq2:linearizedEulerEquation}, we get
\begin{align*}
	\pderiv[2]{P_1}{t} &= c^2\pderiv[2]{\rho_1}{t} = c^2\pderiv{}{t}\left(\pderiv{\rho_1}{t}\right)= c^2\pderiv{}{t}\left(-\rho_0\nabla\cdot\vec{V}_1\right) = -c^2\nabla\cdot\left(\rho_0\pderiv{\vec{V}_1}{t}\right)\\
	&= -c^2\nabla\cdot\left(-\nabla P_1\right) = c^2\nabla^2 P_1
\end{align*}
which is simply the classical wave equation for the pressure 
\begin{equation}\label{Eq2:waveEquation}
	\frac{1}{c^2}\pderiv[2]{P_1}{t} = \nabla^2 P_1.
\end{equation}
Inserting $P_1(\vec{x},t) = \bar{P}_1(\vec{x},k)\euler^{-\imag \omega t}$ then yields the \textit{Helmholtz equation}
\begin{equation*}
	\nabla^2\bar{P}_1+k^2\bar{P}_1 = 0
\end{equation*}
where $k=\frac{\omega}{c}$ is called the \textit{wave number}. The pressure $\bar{P}_1$ will later be denoted by $p$.
%
%Let now the \textit{Fourier transformation} of the $P_1$ be given by
%\begin{equation*}
%	\hat{P}_1(\vec{x},\omega) = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty P_1(\vec{x},t)\euler^{-\imag\omega t}\idiff t.
%\end{equation*}
%such that
%\begin{equation*}
%	P_1(\vec{x},t) = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \hat{P}_1(\vec{x},\omega)\euler^{\imag\omega t}\idiff\omega.
%\end{equation*}
%Observe that
%\begin{equation}\label{Eq2:FourierFormula1}
%	\frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \pderiv[2]{P_1}{t}\euler^{-\imag\omega t}\idiff t = -\omega^2 \hat{P}_1.
%\end{equation}
%and
%\begin{equation}\label{Eq2:FourierFormula2}
%	\frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \nabla^2 P_1\euler^{-\imag\omega t}\idiff t = \nabla^2 \hat{P}_1.
%\end{equation}
%Taking the Fourier transform of \Cref{Eq2:waveEquation} we get
%\begin{equation*}
%	\frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \frac{1}{c^2} \pderiv[2]{P_1}{t}\euler^{-\imag\omega t}\idiff t = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \nabla^2 P_1\euler^{-\imag\omega t}\idiff t
%\end{equation*}
%which, using \Cref{Eq2:FourierFormula1} and \Cref{Eq2:FourierFormula2}, is equivalent to
%\begin{equation*}
%	-\frac{\omega^2}{c^2}\hat{P}_1 = \nabla^2\hat{P}_1.
%\end{equation*}
%Hence, we have arrived at the \textit{Helmholtz equation}
%\begin{equation*}
%	\nabla^2\hat{P}_1+k^2\hat{P}_1 = 0
%\end{equation*}
%where $k=\frac{\omega}{c}$ is called the \textit{wave number}. \textcolor{red}{denne utledningen gir ikke mening hvis vi antar periodisitet, siden fourierintegralet ikke da vil eksistere.} Sett $P_1(\vec{x},t) = \bar{P}_1(\vec{x},k)\euler^{-\imag \omega t}$ da blir
%\begin{equation*}
%	\hat{P}_1(\vec{x},\omega) = \frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty P_1(\vec{x},t)\euler^{-\imag\omega t}\idiff t = \bar{P}_1(\vec{x},k)\frac{1}{\sqrt{2\pi}}\int_{-\infty}^\infty \euler^{-2\imag \omega t}\idiff t.
%\end{equation*}
%som er et integral som ikke eksisterer. \textcolor{red}{(Trond Jenserud skal se på dette)}.

\subsection{Linear elasticity}
One important assumption for using linear elasticity is that only small deformations of the material occurs. We will here not show in detail the derivation of the governing equation for linearized elasticity, but we present the notation used in the formulation of the isogeometric analysis. 

The notations used, takes inspirations from~\cite{Cottrell2009iat}. In this section, the indices $i$, $j$, $k$ and $l$ will denote a specific spatial direction. All calculations will be in three dimensions, such that $i,j,k,l=1,2,3$. Moreover, $u_i$ shall denote the $i^{\textnormal{th}}$ component of the vector $\vec{u}$ and differentiation is denoted with a comma such that
\begin{equation*}
	u_{i,j} = u_{i,x_j} = \frac{\partial u_i}{\partial x_j}.
\end{equation*}
Finally, we use the convention that if an index is repeated, it imply summation. That is,
\begin{equation*}
	\sigma_{ij} n_j = \sigma_{i,1} n_1 + \sigma_{i,2} n_2 + \sigma_{i,3} n_3
\end{equation*}
and
\begin{equation*}
	\sigma_{ij,j} + f_i = \frac{\partial\sigma_{i1}}{\partial x_1} + \frac{\partial\sigma_{i2}}{\partial x_2} + \frac{\partial\sigma_{i3}}{\partial x_3} + f_i.
\end{equation*}
Note that we do not sum over $i$ in the latter example since the quantities are separated by a plus sign. Define now the \textit{symmetric part} of a general tensor $\vec{A}=[A_{ij}]$ to be
\begin{equation*}
	A_{(ij)} = A_{(ji)} := \frac{A_{ij}+A_{ji}}{2}
\end{equation*}
and note that if $\vec{B}=[B_{ij}] = [B_{(ij)}]$ is a symmetric tensor, then
\begin{equation}\label{Eq2:tensorSymmetry}
	A_{ij} B_{ij} = A_{(ij)} B_{ij}.
\end{equation}
That is, we can combine the components of $\vec{B}$ which are equal to reduce redundant computations.

Let now $\sigma_{ij}$ denote the Cartesian components of the Cauchy \textit{stress tensor} and let $\varepsilon_{ij}$ denote the \textit{infinitesimal strain tensor} which is defined by
\begin{equation*}
	\varepsilon_{ij} = u_{(i,j)} = \frac{u_{i,j}+u_{j,i}}{2}.
\end{equation*}
We can now state the relation between $\varepsilon_{ij}$ as $\sigma_{ij}$ using the generalized Hooke's law as
\begin{equation*}
	\sigma_{ij} = c_{ijkl}\varepsilon_{kl}
\end{equation*}
where $c_{ijkl}$ are \textit{elastic coefficients}. In the case of isotropic material, these coefficients are given by
\begin{equation*}
	c_{ijkl} = \lambda\delta_{ij}\delta_{kl} +\mu\left(\delta_{ik}\delta_{jl}+\delta_{il}\delta_{jk}\right)
\end{equation*}
where the Kronecker delta function is given by
\begin{equation*}
	\delta_{ij}=\begin{cases}
	1 &i=j\\
	0&\text{otherwise}
	\end{cases}
\end{equation*}
and the parameters $\lambda$ and $\mu$ are the \textit{Lamé parameters} which are expressed in terms of $E$ and $\nu$ (\textit{Young's modulus} and \textit{Poisson's ratio} respectively) by
\begin{equation*}
	\lambda=\frac{\nu E}{(1+\nu)(1-2\nu)}\quad\text{and}\quad\mu = \frac{E}{2(1+\nu)}.
\end{equation*}
We are now ready to state the \textit{strong form} of the linear elasticity problem in three dimensions. 

Let $\Omega\subset\R^3$ be the domain with a boundary $\partial \Omega$ which is composed of two parts; $\Gamma_{D_i}$ and $\Gamma_{N_i}$. These are called \textit{Dirichlet} and \textit{Neumann} boundary conditions, respectively, and satisfies $\bigcup_{i=1}^3\Gamma_{D_i}\cup\Gamma_{N_i}=\partial\Omega$ and $\Gamma_{D_i}\cap\Gamma_{N_i}=\emptyset$. Moreover, let the functions $f_i:\Omega\to\R$, $g_i:\Gamma_{D_i}\to\R$ and $h_i:\Gamma_{N_i}\to\R$ be given. Then, find $u_i:\overline{\Omega}\to\R$ such that
\begin{alignat}{3}
	\sigma_{ij,j} + f_i &= \rho_{\mathrm{s}} u_{i,tt}\qquad 	&&\text{in}\quad \Omega,\label{Eq2:mainDiffEqn}\\
	u_i &= g_i						&&\text{on}\quad \Gamma_{D_i},\label{Eq2:mainDiffEqnBC1}\\
	\sigma_{ij} n_j &= h_i 			&&\text{on}\quad \Gamma_{N_i},\label{Eq2:mainDiffEqnBC2}
\end{alignat}
for $i=1,2,3$.

Using the assumption of periodicity, we may insert $u_i \rightarrow u_i \euler^{-\imag\omega t}$  (and $f_i \rightarrow f_i \euler^{-\imag\omega t}$) into \Cref{Eq2:mainDiffEqn}. As $\sigma$ is a linear function of $u_i$, we get a common factor $\euler^{-\imag\omega t}$ which simplifies the equation to
\begin{equation}
	\sigma_{ij,j} + \omega^2 \rho_{\mathrm{s}} u_i = -f_i \qquad \text{in}\quad \Omega\label{Eq2:mainDiffEqn2}.
\end{equation}


==> contents/preface.tex <==
\section{Preface}
This thesis concludes my master's degree in Mathematics at the Norwegian University of Technology and Science (NTNU). The work spans both the fall 2014 and the spring 2015. The thesis represents the second half of the 2 year master program, which is a continuation of my bachelor's in degree at NTNU.

The thesis was proposed by my supervisor Trond Jenserud\footnote{Researcher at Norwegian Defence Research Establishment (FFI).}. At that time, I had experience both with FEM and IGA as I had been following three courses involving these methods. These courses would set the foundation of the knowledge needed to complete a thesis on the subject. All of these courses was supervised by Trond Kvamsdal\footnote{Professor in Computational Mathematics at Department of Mathematical Sciences, NTNU.}, and it was thus natural to choose Kvamsdal as an adviser at NTNU. Although two complete programs had been made for FEM and IGA (both involving solution of elasticity problems) in these courses, I decided to start from scratch by building each part of the code in a structural way. This way, I was able to create generic functions which could solve a larger set of problems. To test the validity of the implementations, many test examples was executed, mostly from the article and book of Hughes et al. (\cite{Hughes2005iac} and~\cite{Cottrell2009iat}). Some additional test examples were invented to validate special aspects of the implementations. These include linear elasticity problem on a Solid circular cylinder and rectangular prisms. This groundwork then enabled more complicated simulations of the vibration analysis, exterior Helmholtz problems and finally fully structure interaction problems. 

The work of this thesis has been to consider the application of IGA. After all, the chosen specialization in the master's degree is applied mathematics. One typically presents the foundation of the theory from functional analysis where the relevant spaces are a topic of discussion. However, I shall in these cases simply refer to other literature.

This thesis forms a basis for a huge study that could be made on the subject. Not only are there topics to be investigated in regards to IGA on acoustic scattering, but also the coupling of IGA and absorbing boundary conditions. In this thesis I choose the infinite element method, but there are many other candidates which could work very well with IGA. Much of this study will be a topic of my PhD which will start this fall.

I would like to express my appreciation to the BeTSSi community for providing a good description for the models to be analyzed, alongside a well arranged setup for the results obtained. I would also like express my appreciation for the two books in~\cite{Cottrell2009iat} and~\cite{Ihlenburg1998fea} by Cotterell et al. and Frank Ihlenburg, respectively. The first has been my main reference to IGA, while the second has been my main reference for acoustic scattering using FEA.

I would like to thank NTNU for a perfect course of study, and in particular I want to thank the Department of Mathematical Sciences for providing an environment with hardware capable of computationally expensive simulations, which have been essential for this thesis. I would also thank Ilkka Karasalo and Martin Østberg\footnote{Researchers at Swedish Defence Research Agency (FOI).}  for providing validating data sets for the final simulations and enthusiastic support. Moreover, I would like to express my gratitude to my two supervisors Trond Jenserud and Trond Kvamsdal for their encouragement and guidance. Finally, I would like to thank Kjetil Andre Johannessen\footnote{Postdoctoral at NTNU.} for his inspirational encouragement which has not only been essential for my master thesis, but also ignited my interest in FEM/IGA in the early stages.
\vspace{2cm}
\begin{flushright}
Jon Vegard Venås\\
NTNU, Trondheim\\
\today
\end{flushright}


==> contents/resultsAndDiscussion_backup.tex <==
\section{Numerical examples} 
\label{Sec2:resultsDisc}
We start by investigating the pollution effect for the scattering problem on a rigid sphere, and then continue with the acoustic structure interaction (ASI) problem on the spherical shell. Rigid scattering on a sphere and elastic scattering on a spherical shell are often used to verify the methods because both cases admits analytic solutions. The latter case is the only known problem which admits such an analytic solution for the ASI scattering problem in 3D, and is thus especially valuable. Moreover, these cases has been used as a benchmark example for many methods and one is then able to compare the performance of each method on this problem.

The multipole layers for the infinite elements will be placed at $r_n=nr_{\mathrm{a}}$ for $n=1,\dots,N$ (this is suggested by Burnett in~\cite{Burnett1994atd}). Moreover, unless otherwise stated, we shall use the PGU formulation by default for the infinite elements.

\subsection{Plane wave scattered by a rigid sphere}
Let the plane wave\footnote{We here use the spherical coordinate system where $r\in[0,\infty)$ is the radius, $\vartheta\in[0,\pi]$ is the polar angle and $\varphi\in[0,2\pi)$ is the asimuth angle satisfying the relations
\begin{equation*}
	x = r\sin\vartheta\cos\varphi,\quad y = r\sin\vartheta\sin\varphi,\quad z = r\cos\vartheta.
\end{equation*}
} (with $\vec{k}=[0, 0, k]^\transpose$)
\begin{equation*}
	p_{\textrm{inc}}(r,\vartheta) = P_{\mathrm{inc}}\euler^{\imag kz} = P_{\mathrm{inc}}\euler^{\imag kr\cos\vartheta}
\end{equation*}
be scattered on a sphere with radius $R=0.5$. That is, we send the wave along the $z$-axis. The resulting scattered wave is then\footnote{Here, $P_n(x)$ denotes the $n^{\mathrm{th}}$ Legendre polynomial and $j_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Bessel function of first kind, and $h_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Hankel function of the first kind.} (rigid scattering)
\begin{equation}\label{Eq2:rigidScattering_p}
	p_{\mathrm{rs}} (r,\vartheta) = -P_{\mathrm{inc}}\sum_{n=0}^\infty \imag^n (2n+1) P_n(\cos\vartheta)\frac{j_n'(kR)}{h_n'(kR)} h_n(kr).
\end{equation}
When computing the $H^1$-norm of the error we will also need the corresponding gradient, which in spherical coordinates is given by
\begin{align*}
	\nabla p_{\mathrm{rs}} (r,\vartheta) &= \pderiv{p_{\mathrm{rs}}}{r}\vec{e}_{\mathrm{r}} + \frac{1}{r}\pderiv{p_{\mathrm{rs}}}{\vartheta}\vec{e}_{\upvartheta} + \frac{1}{r\sin\vartheta}\pderiv{p_{\mathrm{rs}}}{\varphi}\vec{e}_{\upvarphi}\\
	&= -P_{\mathrm{inc}}\sum_{n=0}^\infty \imag^n (2n+1) \frac{j_n'(kR)}{h_n'(kR)} \left(P_n(\cos\vartheta)kh_n'(kr)\vec{e}_{\mathrm{r}} - \frac{\sin\vartheta}{r}P_n'(\cos\vartheta)h_n(kr)\vec{e}_{\upvartheta}\right)
\end{align*}
where the involved unit vectors in spherical coordinates are related to the Cartesian coordinates by
\begin{align*}
	\vec{e}_{\mathrm{r}} &= \sin\vartheta\cos\varphi\vec{e}_{\mathrm{x}} + \sin\vartheta\vec{e}_{\mathrm{y}} + \cos\vartheta\vec{e}_{\mathrm{z}}\\
	\vec{e}_{\upvartheta} &= \cos\vartheta\cos\varphi\vec{e}_{\mathrm{x}} + \cos\vartheta\sin\varphi\vec{e}_{\mathrm{y}} - \sin\vartheta\vec{e}_{\mathrm{z}}.
\end{align*}
For details of this solution see Ihlenburg~\cite[p. 28]{Ihlenburg1998fea}. Since this example has been used in~\cite{Gerdes1999otp} and~\cite{Simpson2014aib}, we may compare our results to the results found in these papers. We start by comparing the results found in~\cite{Simpson2014aib} by considering $k=2$ (low frequencies), and the construction of NURBS meshes illustrated in \Cref{Fig2:SphericalShellMeshes}. We send the incident wave along the $z$-axis (instead of the $x$-axis) and align the symmetry of the NURBS parametrization along the $y$-axis (instead of the $z$-axis). The results should obviously remain unchanged. We shall use $N=3$, which will practically neglect the error from the infinite element implementation on the coarse meshes considered. For low frequencies and the usage of the PGU formulation, it seems to be advantageous to set the artificial boundary very close to the surface of the sphere. We find the optimal radius to be around $r_{\mathrm{a}}=0.51$. When comparing with BEM, we typically have more liberty of adding degrees of freedom in the radial direction without destroying the fairness of the comparison. This is because the computational time of solving an BEM system of equations is higher than the corresponding IGA/IEM system of equations. However, it is very hard to compare the two methods without running both methods on the same computers. In~\Cref{Fig2:scatteringRigidSphereErrorNearField} we plot the absolute relative error in the modulus of the scattered field at $r=5$ (as was done in~\cite{Simpson2014aib}). Comparing with the results in~\cite{Simpson2014aib} we observe that BEM has the advantage on the coarsest mesh, but IGA/IEM produce the best results on finer meshes. 
%In~\Cref{Fig2:SphericalShellErrorMesh1}, \Cref{Fig2:SphericalShellErrorMesh2} and \Cref{Fig2:SphericalShellErrorMesh3} we visualize the error at the artificial boundary $\Gamma_{\mathrm{a}}$ both in the scalar field and the normed gradient field for mesh 1, 2 and 3, respectively. The gradient is used to evaluate far field points, so it is of interest to study this error as well. Interestingly, we observe larger errors in the gradient where the basis functions have lower continuity (which occurs at the mesh lines).
\begin{figure}
	\centering
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh1_2_0}
		\caption{Mesh 1}
    \end{subfigure}
    ~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh2_2_0}
		\caption{Mesh 2}
		\label{Fig2:SphericalShellMeshes2}
    \end{subfigure}
    ~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh3_2_0}
		\caption{Mesh 3}
		\label{Fig2:SphericalShellMeshes3}
    \end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Meshes. The knot $\zeta=0.5$ has been inserted in $\Zeta$ for mesh 2 while the knots $\zeta = 0.25, 0.5, 0.75$ has been inserted in $\Zeta$ for mesh 3 (from the original mesh 1, with NURBS data found in \Cref{Sec2:NURBSdata}).}
	\label{Fig2:SphericalShellMeshes}
\end{figure}

\tikzsetnextfilename{scatteringRigidSphereErrorNearField} 
\begin{figure}
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.94\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed}, % 3
				{ntnublue}, % 2
				{myGreen}, % 3
			},
			xtick={0, 45, ..., 360},
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={aspect angle $\alpha$},
			ylabel={$\frac{\big||p_{\mathrm{rs}}| - \left|p_h\right|\big|}{|p_{\mathrm{rs}}|}$},
			%ymax=100
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh1_180_0_formul_PGU_error.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh2_180_0_formul_PGU_error.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh3_180_0_formul_PGU_error.dat};
			\addlegendentry{Mesh 1}
			\addlegendentry{Mesh 2}
			\addlegendentry{Mesh 3}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} The relative error for the near field  $k=2$. The near field is plotted over all aspect angles $\alpha$ at $r=5$.}
	\label{Fig2:scatteringRigidSphereErrorNearField}
\end{figure}

Finally, we follow~\cite{Gerdes1999otp} in presenting the results on the pollution effect by comparing the results to the so-called best approximation BA. The BA solution represent the best possible solution in the solution space, and it is found by solving:
\begin{equation*}
	\text{Find}\quad p_h^{\mathrm{ba}}\in \calV_h(\Omega_{\mathrm{a}})\quad \text{such that} \quad \left(p_h^{\mathrm{ba}},q_h\right)_{H^1(\Omega_{\mathrm{a}})} = \left(p_{\mathrm{rs}}, q_h\right)_{H^1(\Omega_{\mathrm{a}})},\quad \forall q_h\in\calV_h(\Omega_{\mathrm{a}})
\end{equation*}
where $\left(p,q\right)_{H^1(\Omega_{\mathrm{a}})}$ is the $H^1$-inner product
\begin{equation*}
	\left(p,q\right)_{H^1(\Omega_{\mathrm{a}})} = \int_{\Omega_{\mathrm{a}}}\nabla p\cdot\nabla \bar{q} + p \bar{q}\idiff\Omega.
\end{equation*}
We denote by
\begin{equation}\label{Eq2:H1relError}
	E_h = \frac{\left\|p_{\mathrm{rs}}-p_h\right\|_{H^1(\Omega_{\mathrm{a}})}}{\left\|p_{\mathrm{rs}}\right\|_{H^1(\Omega_{\mathrm{a}})}},
\end{equation}
the absolute relative error with corresponding formula for $p_h^{\mathrm{ba}}$. We shall replicate the problem setup by Gerdes and Ihlenburg~\cite{Gerdes1999otp} which uses $N=6$ radial basis function in the infinite elements, places the artificial boundary at $r_{\mathrm{a}} = 1$ (the radius of the scatterer is as before $R=0.5$) and truncate \Cref{Eq2:rigidScattering_p} at $n=6$ to eliminate the error originating from the artificial boundary.

\begin{figure}
	\centering        
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh2_3_0}
		\caption{Mesh $2_3^0$.}
		\label{Fig2:SphericalShellMesh2_3_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh2_3_2}
		\caption{Mesh $2_3^2$.}
		\label{Fig2:SphericalShellMesh2_3_2}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh2_4_0}
		\caption{Mesh $2_4^0$.}
		\label{Fig2:SphericalShellMesh2_4_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh2_4_3}
		\caption{Mesh $2_4^3$.}
		\label{Fig2:SphericalShellMesh2_4_3}
	\end{subfigure}
	\par\bigskip  
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh3_3_0}
		\caption{Mesh $3_3^0$.}
		\label{Fig2:SphericalShellMesh3_3_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh3_3_2}
		\caption{Mesh $3_3^2$.}
		\label{Fig2:SphericalShellMesh3_3_2}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh3_4_0}
		\caption{Mesh $3_4^0$.}
		\label{Fig2:SphericalShellMesh3_4_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShell/sphericalShellMesh3_4_3}
		\caption{Mesh $3_4^3$.}
		\label{Fig2:SphericalShellMesh3_4_3}
	\end{subfigure}
	\caption{Illustration of the angular NURBS parametrization (parametrized with the $\xi$ and $\eta$ parameters) used in the numerical examples. The sub script index denotes the common angular NURBS degree $\check{p}_\upxi=\check{p}_\upeta$, and the super script index indicates the continuity of the angular parametrization over inserted knots. We insert $2^{s-1}-1$ knots in the original NURBS mesh (with data from \Cref{Sec2:NURBSdata}) for each knot interval in the $\xi$- and $\eta$-direction with $s=2,3$ for mesh $2_{\check{p}_\upxi}^0$ and mesh $3_{\check{p}_\upxi}^0$, respectively, for $\check{p}_\upxi=3,4$. Each internal knot is then repeated $\check{p}_\upxi=\check{p}_\upeta$ times to obtain $C^0$ continuity. To match the same degree of freedom for higher continuity meshes (mesh $2_{\check{p}_\upxi}^{\check{p}_\upxi-1}$ and mesh $3_{\check{p}_\upxi}^{\check{p}_\upxi-1}$) we must insert $\check{p}_\upxi\cdot 2^{s-1}-\check{p}_\upxi$ knots in the original NURBS mesh for each knot interval. The corresponding FEM meshes, mesh $2_{\check{p}_\upxi}^{\textsc{fem}}$ and $3_{\check{p}_\upxi}^{\textsc{fem}}$, are visually indistinguishable from mesh $2_{\check{p}_\upxi}^0$ and mesh $3_{\check{p}_\upxi}^0$, respectively.}
	\label{Fig2:SphericalShellMesh23_p}
\end{figure}

\Cref{Fig2:SphericalShellMesh23_p} illustrates the angular NURBS parametrization used to obtain the IGA results. In order to compare classical FEM and IGA on the scattering problem, we shall transform the NURBS mesh to a classical FEM mesh. We use the technique described in \Cref{Sec2:NURBStransformation} to get a isoparametric B-spline approximation of the geometry. Mesh $2_{\check{p}_\upxi}^{\textsc{fem}}$ will here be constructed from mesh $2_{\check{p}_\upxi}^0$ and mesh $3_{\check{p}_\upxi}^{\textsc{fem}}$ will be constructed from mesh $3_{\check{p}_\upxi}^0$. 

Let $\mathrm{noSurfDofs}()$ be a function counting the number of degrees of freedom on the surface of a given mesh. Then
\begin{align*}
	\mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_3^{\textsc{fem}}\right) &= \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_3^0\right) = \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_3^2\right) = 226,\\
	\mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_4^{\textsc{fem}}\right) &= \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_4^0\right) = \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}2_4^3\right) = 482,\\
	\mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_3^{\textsc{fem}}\right) &= \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_3^0\right) = \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_3^2\right) = 1106,\\
	\mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_4^{\textsc{fem}}\right) &= \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_4^0\right) = \mathrm{noSurfDofs}\left(\mathrm{Mesh\,}3_4^3\right) = 1986.
\end{align*}
The corresponding numbers for the prismatic isoparametric meshes used in~\cite{Gerdes1999otp} is 110, 194, 434 and 786 (``Mesh $H$'' with angular degree 3 and 4, and ``Mesh $h$'' with angular degree 3 and 4, respectively). The fact that these number differ from another is the reason we include our own FEM results to have a more fair comparison. It should be noted that the FEM analysis will then use the Bernstein basis instead of the classical Lagrange basis. However, both of these set of functions spans the same spaces, such that the results should be identical. We report the results in \Cref{Tab2:p3q2} - \Cref{Tab2:p4q3} and for illustrative purposes, we also plot the data sets of these tables in \Cref{Fig2:plot_p3q2} - \Cref{Fig2:plot_p4q3}, respectively. We firstly observe that the BA solution indeed yields the best results, but also the fact that the numerical results is quite close to this solution. Moreover, we generally observe the presence of the pollution effect; for higher wave numbers we obtain less accurate results. We also observe the curves to level off (especially for lower frequencies) which is due to under resolution in the angular directions. The FEM simulation yields a some reduction in the accuracy compared to the corresponding IGA $C^0$ counterpart. However, as we can see, this reduction is of less significance when higher order prismatic finite elements are used. A final general remark is the fact that we always obtain better results with higher continuity (with fixed number of dofs). 

The pollution effect is best observed in \Cref{Fig2:plot_p3q2mesh2} (where the least amount of dofs has been used). We here observe that the solution for $k=5$ quickly reach the optimal solution for the given resolution in the angular direction, whereas the same optimality lags behind for higher frequencies. The same tendency is observed in~\Cref{Fig2:plot_p4q2mesh3} where we increase the number of angular elements. The difference is observed in the fact that we get better results and we may use more dofs in the radial direction before we reach the optimal solution. A more extreme version of these two first figures may be observed in~\Cref{Fig2:plot_p4q3mesh2} and \Cref{Fig2:plot_p4q3mesh3} where we increase the radial polynomial degree. The figures in \Cref{Fig2:plot_p4q2} and \Cref{Fig2:plot_p4q3} increases the angular polynomial order of the preceding figures by one. We may then begin to observe the expected optimal convergence order, as the main source of error comes from the low resolution in the radial direction (that is, inserting more elements in the angular direction will not improve the result notably for a low amount of dofs in the radial direction). In \Cref{Fig2:plot_p4q2mesh3} we have the largest ratio of the dofs in the angular direction and the dofs in the radial direction. For this reason, the FEM results and the IGA $C^0$ results are visually indistinguishable.

\begin{itemize}
\item The convergence analysis is done on spherical shells.
\item Benchmarks for the spherical shell in BeTSSi-format: %
\begin{table}
	\centering%
	\begin{tabular}{l l l l}
		\toprule
		 & S1 & S2 & S3 \\
		\midrule
		$R_0$ & $0.5\unit{m}$ & $1\unit{m}$ & $5\unit{m}$\\
		$t$ & $50\unit{mm}$ & $20\unit{mm}$ & $8\unit{mm}$\\
		Fill & air & air & water\\
		\bottomrule
	\end{tabular}
	\caption{Parameters for S1, S2 and S3.}%
\end{table}
\item As for M1, M2 and M3, one can combine these models to get S13 and S23.
\item In all these cases (including combined models) analytic solutions exist (Jenserud $\sim$1990).
\end{itemize}%
\begin{table}
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for IGA (using different continuities) and FEM with their corresponding best approximation (BA). The meshes are found in \Cref{Fig2:SphericalShellMesh23_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:p3q2}
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 3 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p3q2mesh3}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 226\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $2_3^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $2_3^0$} 	&& \multicolumn{2}{c}{Mesh $2_3^2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p3q2mesh2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 4 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p3q2mesh4}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 1106\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_3^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $3_3^0$} 	&& \multicolumn{2}{c}{Mesh $3_3^2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p3q2mesh3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
\end{table}


\begin{table}
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for IGA (using different continuities) and FEM with their corresponding best approximation (BA). The meshes are found in \Cref{Fig2:SphericalShellMesh23_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:p3q3}
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 3 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p3q3mesh3}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 226\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $2_3^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $2_3^0$} 	&& \multicolumn{2}{c}{Mesh $2_3^2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p3q3mesh2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 4 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p3q3mesh4}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 1106\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_3^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $3_3^0$} 	&& \multicolumn{2}{c}{Mesh $3_3^2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p3q3mesh3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
\end{table}

\begin{table}
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for IGA (using different continuities) and FEM with their corresponding best approximation (BA). The meshes are found in \Cref{Fig2:SphericalShellMesh23_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:p4q2}
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 3 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=4$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p4q2mesh3}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 482\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $2_4^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $2_4^0$} 	&& \multicolumn{2}{c}{Mesh $2_4^3$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p4q2mesh2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 4 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=4$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p4q2mesh4}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 1986\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_4^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $3_4^0$} 	&& \multicolumn{2}{c}{Mesh $3_4^3$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p4q2mesh3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
\end{table}


\begin{table}
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for IGA (using different continuities) and FEM with their corresponding best approximation (BA). The meshes are found in \Cref{Fig2:SphericalShellMesh23_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:p4q3}
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 3 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=4$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p4q3mesh3}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 482\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $2_4^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $2_4^0$} 	&& \multicolumn{2}{c}{Mesh $2_4^3$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p4q3mesh2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 4 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=4$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p4q3mesh4}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 1986\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_4^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $3_4^0$} 	&& \multicolumn{2}{c}{Mesh $3_4^3$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis4/IGAIGA_p4q3mesh3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
\end{table}

\begin{figure}
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p3q2mesh2} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=129
			]
			% k = 5		
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k5Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh2k40Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $2_3^0$ in \Cref{Fig2:SphericalShellMesh2_3_0} and the $C^2$-results uses mesh $2_3^2$ in \Cref{Fig2:SphericalShellMesh2_3_2}.}
	\label{Fig2:plot_p3q2mesh2}
	\end{subfigure}

	\par\bigskip
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p3q2mesh3} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=129
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k5Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q2mesh3k40Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $3_3^0$ in \Cref{Fig2:SphericalShellMesh3_3_0} and the $C^2$-results uses mesh $3_3^2$ in \Cref{Fig2:SphericalShellMesh3_3_2}.}
	\label{Fig2:plot_p3q2mesh3}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q2} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$). All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q2}
\end{figure}
\begin{figure}
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p3q3mesh2}  
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=193
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k5Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh2k40Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $2_3^0$ in \Cref{Fig2:SphericalShellMesh2_3_0} and the $C^2$-results uses mesh $2_3^2$ in \Cref{Fig2:SphericalShellMesh2_3_2}.}
	\label{Fig2:plot_p3q3mesh2}
	\end{subfigure}

	\par\bigskip
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p3q3mesh3} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=193
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k5Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p3q3mesh3k40Case3.dat};
			\addlegendentry{BA IGA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $3_3^0$ in \Cref{Fig2:SphericalShellMesh3_3_0} and the $C^2$-results uses mesh $3_3^2$ in \Cref{Fig2:SphericalShellMesh3_3_2}.}
	\label{Fig2:plot_p3q3mesh3}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q3} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=3$). All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q3}
\end{figure}

\begin{figure}
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p4q2mesh2} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=129
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k5Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=5$}
			\addlegendentry{IGA $C^3$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh2k40Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=40$}
			\addlegendentry{IGA $C^3$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $2_4^0$ in \Cref{Fig2:SphericalShellMesh2_4_0} and the $C^3$-results uses mesh $2_4^3$ in \Cref{Fig2:SphericalShellMesh2_4_3}.}
	\label{Fig2:plot_p4q2mesh2}
	\end{subfigure}

	\par\bigskip
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p4q2mesh3}
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=129
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k5Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=5$}
			\addlegendentry{IGA $C^3$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q2mesh3k40Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=40$}
			\addlegendentry{IGA $C^3$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $3_4^0$ in \Cref{Fig2:SphericalShellMesh3_4_0} and the $C^3$-results uses mesh $3_4^3$ in \Cref{Fig2:SphericalShellMesh3_4_3}.}
	\label{Fig2:plot_p4q2mesh3}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p4q2} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$). All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p4q2}
\end{figure}
\begin{figure}
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p4q3mesh2} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=193
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k5Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=5$}
			\addlegendentry{IGA $C^3$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh2k40Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=40$}
			\addlegendentry{IGA $C^3$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $2_4^0$ in \Cref{Fig2:SphericalShellMesh2_4_0} and the $C^3$-results uses mesh $2_4^3$ in \Cref{Fig2:SphericalShellMesh2_4_3}.}
	\label{Fig2:plot_p4q3mesh2}
	\end{subfigure}
	
	\par\bigskip
	\begin{subfigure}{\textwidth}
	\tikzsetnextfilename{plot_p4q3mesh3} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{ntnublue, dashed, mark=triangle*}, % 2
				{ntnublue, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
				{ntnublue, dashed, mark=*}, % 2
				{ntnublue, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=193
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k5Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=5$}
			\addlegendentry{IGA $C^3$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis4/plot_p4q3mesh3k40Case3.dat};
			\addlegendentry{BA IGA $C^3$, $k=40$}
			\addlegendentry{IGA $C^3$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{The $C^0$-results uses mesh $3_4^0$ in \Cref{Fig2:SphericalShellMesh3_4_0} and the $C^3$-results uses mesh $3_4^3$ in \Cref{Fig2:SphericalShellMesh3_4_3}.}
	\label{Fig2:plot_p4q3mesh3}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p4q3} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$). All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p4q3}
\end{figure}

\clearpage
\subsection{Plane wave scattered by an elastic spherical shell}
We now turn to the acoustic-structure interaction (ASI) problem on a spherical shell where we want to compare classical FEM and IGA. This example has been thoroughly analysed by Ihlenburg in~\cite{Ihlenburg1998fea} using classical FEM and IEM. Once again, we choose to compare with our own FEM results for fair comparisons.

In~\cite[pp. 12-20]{Chang1994voa} the exact 3D elasticity solution for the spherical shell is presented. We shall repeat the final formulas needed for the scattered pressure.
Let the plane wave
\begin{equation*}
	p_{\textrm{inc}}(r,\vartheta) = P_{\mathrm{inc}}\euler^{\imag kz} = P_{\mathrm{inc}}\euler^{\imag kr\cos\vartheta}
\end{equation*}
be scattered on a elastic spherical shell with inner radius $R_1$ and outer radius $R_0$. The scattered pressure is then\footnote{Here, $P_n(x)$ denotes the $n^{\mathrm{th}}$ Legendre polynomial, $j_n(x)$ and $y_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Bessel function of first and second kind, respectively, and $h_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Hankel function of the first kind.}  (elastic scattering)
\begin{equation}\label{Eq2:exact3DscatteringSphericalShellSol}
	p_{\mathrm{es}}(r,\vartheta) = p_{\mathrm{rs}}(r,\vartheta) + \frac{P_{\mathrm{inc}}\rho_{\mathrm{f}} c_{\mathrm{f}}}{(kR_0)^2}\sum_{n=0}^\infty \frac{\imag^n(2n+1)P_n(\cos\vartheta)h_n(kr)}{[h_n'(kR_0)]^2(Z_n+z_n)}
\end{equation}
where $p_{\mathrm{rs}}$ is defined in \Cref{Eq2:rigidScattering_p}, and $z_n$ (\textit{specific acoustic impedance}) and $Z_n$ (\textit{mechanical impedance}) are defined by
\begin{equation*}
	z_n = \imag\rho_{\mathrm{f}} c_{\mathrm{f}}\frac{h_n(kR_0)}{h_n'(kR_0)}
\end{equation*}
and
\begin{equation*}
	Z_n =\frac{R_0}{-\imag\omega\left[C_n^{(1)} D_{1,n}^{(1)}(b_1 R_0) + C_n^{(2)} D_{2,n}^{(1)}(b_2 R_0) + C_n^{(3)} D_{1,n}^{(2)}(b_1 R_0) + C_n^{(4)} D_{2,n}^{(2)}(b_2 R_0)\right]},
\end{equation*}
where 
\begin{equation*}
	D_{1,n}^{(i)}(x) = nA_n^{(i)}(x)-xA_{n+1}^{(i)}(x),\quad\text{and}\quad	D_{2,n}^{(i)}(x) = n(n+1)A_n^{(i)}(x),
\end{equation*}
and the coefficients $C_n^{(1)}$, $C_n^{(2)}$, $C_n^{(3)}$ and $C_n^{(4)}$ are given by
\begin{equation*}
	C_0^{(1)} = \frac{\frac{R_0^2}{2\mu}B_{1,n}^{(2)}(b_1 R_1)}{\nabla^2_0},\quad C_0^{(2)}=0,\quad	C_0^{(3)} = -\frac{\frac{R_0^2}{2\mu}B_{1,n}^{(1)}(b_1 R_1)}{\nabla^2_0},\quad C_0^{(4)}=0,
\end{equation*}
for $n=0$ where
\begin{equation*}
	\nabla^2_0=\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_0) & B_{1,n}^{(2)}(b_1 R_0)\\
		B_{1,n}^{(1)}(b_1 R_1) & B_{1,n}^{(2)}(b_1 R_1)
	\end{vmatrix},
\end{equation*}
and by
\begin{equation*}
	C_n^{(1)} = \frac{\nabla^2_{1,n}}{\nabla^2_n},\quad C_n^{(2)} = \frac{\nabla^2_{2,n}}{\nabla^2_n},\quad C_n^{(3)} = \frac{\nabla^2_{3,n}}{\nabla^2_n},\quad C_n^{(4)} = \frac{\nabla^2_{4,n}}{\nabla^2_n},
\end{equation*}
for $n>0$ where the following notations has been used
\begin{equation*}
	\nabla^2_n = \begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_0) & B_{2,n}^{(1)}(b_2 R_0) & B_{1,n}^{(2)}(b_1 R_0) & B_{2,n}^{(2)}(b_2 R_0)\\
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix},
\end{equation*}
\begin{equation*}
	\nabla^2_{1,n} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix},
\end{equation*}
\begin{equation*}
	\nabla^2_{2,n} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix},
\end{equation*}
\begin{equation*}
	\nabla^2_{3,n} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix},
\end{equation*}
\begin{equation*}
	\nabla^2_{4,n} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1)
	\end{vmatrix},
\end{equation*}
\begin{align*}
	B_{1,n}^{(i)}(x) &= \left[n^2-n-\frac{1}{2}\left(\frac{b_2}{b_1}\right)^2 x^2\right] A_n^{(i)}(x) + 2xA_{n+1}^{(i)}(x),\\
	B_{2,n}^{(i)}(x) &= n(n+1)\left[(n-1)A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\right],\\
	B_{3,n}^{(i)}(x) &= (n-1) A_n^{(i)}(x) - xA_{n+1}^{(i)}(x),\\
	B_{4,n}^{(i)}(x) &= \left(n^2-1-\frac{1}{2}x^2\right) A_n^{(i)}(x) + xA_{n+1}^{(i)}(x),
\end{align*}
%\begin{align*}
%	B_9^{(i)}(x) &= \left[-n^2-\frac{1}{2}\left(\frac{b_2}{b_1}\right)^2 x^2+x^2\right] A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\\
%	B_7^{(i)}(x) &= -(n^2+n)\left[n A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\right] \\
%	B_5^{(i)}(x) &= \left[n-\frac{1}{2}x^2+\left(\frac{b_1}{b_2}\right)^2 x^2\right] A_n^{(i)}\left(\frac{b_1}{b_2}x\right) - \frac{b_1}{b_2}x A_{n+1}^{(i)}\left(\frac{b_1}{b_2}x\right)\\
%	B_6^{(i)}(x) &= n(n+1)A_n^{(i)}(x)\\
%\end{align*}
\begin{equation*}
	A_{n}^{(1)}(x) = j_n(x),\qquad A_{n}^{(2)}(x) = y_n(x),
\end{equation*}
\begin{equation*}
	b_1=\frac{\omega}{c_1},\quad b_2=\frac{\omega}{c_2},\quad c_1 = \sqrt{\frac{\lambda+2\mu}{\rho_s}},\quad c_2 = \sqrt{\frac{\mu}{\rho_s}}.
\end{equation*}
Here, the parameters $c_1$ and $c_2$ are called the longitudinal wave velocity and shear wave velocity, respectively. Moreover, $\lambda$ and $\mu$ are the Lam{\'e} parameters which can be defined by the Young's modulus, $E$, and Poisson's ratio, $\nu$, as
\begin{equation*}
	\lambda = \frac{\nu E}{(1+\nu)(1-2\nu)}\quad\text{and}\quad \mu = \frac{E}{2(1+\nu)}.
\end{equation*}
The material parameters are found in \Cref{Tab2:sphericalShellParameters}, and we shall use $r_{\mathrm{a}}=6$ and $N=3$ radial shape functions in the infinite elements. Moreover, we shall use the PGU formulation for the infinite elements. For each experiment we use the same NURBS order everywhere. Denote by $\check{p}_\upxi = p_{\upxi,\mathrm{f}} = p_{\upxi,\mathrm{s}}$ the common NURBS order in the fluid and the solid in the $\xi$-direction. Similarly $\check{p}_\upeta = p_{\upeta,\mathrm{f}} = p_{\upeta,\mathrm{s}}$ and $\check{p}_\upzeta = p_{\upzeta,\mathrm{f}} = p_{\upzeta,\mathrm{s}}$. For each experiment we will use $\check{p}_\upxi = \check{p}_\upeta = \check{p}_\upzeta$.

\begin{table}
	\centering
	\caption[Parameters for spherical shell]{\textbf{Scattering on spherical shell:} Parameters.}
	\label{Tab2:sphericalShellParameters}
	\begin{tabular}{l l}
		\toprule
		Parameter & Description\\
		\midrule
		$E = 2.07\cdot 10^{11}\unit{Pa}$ & Young's modulus\\
		$\rho_{\mathrm{s}} = 7669\unit{kg/m^3}$ & Density of solid\\
		$\rho_{\mathrm{f}} = 1000\unit{kg/m^3}$ & Density of fluid\\
		$\nu = 0.3$ & Poisson's ratio\\
		$c_{\mathrm{f}} = 1524\unit{m/s}$ & Fluid speed of sound\\
		$t_{\mathrm{s}} = 0.15\unit{m}$ & Thickness of the shell\\
		$R = 5\unit{m}$ & Radius of the midsurface of the shell\\
		$R_1 = 4.925\unit{m}$ & Inner radius of the shell\\
		$R_0 = 5.075\unit{m}$ & Outer radius of the shell\\
		$P_{\mathrm{inc}} = 1\unit{Pa}$ & Amplitude of incident wave\\
		\bottomrule
	\end{tabular}
\end{table}
The structure of the angular parametrization is equal for both the finite fluid domain (inside $\Gamma_{\mathrm{a}}$) and the solid domain (same structure as the meshes in \Cref{Fig2:SphericalShellMesh23_p}). We use $n_{\upzeta, \mathrm{f}}=4\check{p}_\upzeta+1$ basis functions in the radial direction for the finite fluid domain and $n_{\upzeta, \mathrm{s}}=2\check{p}_\upzeta+1$ basis functions in the radial direction for the solid domain

%For mesh $3_2^{\textsc{fem}}$ and mesh $3_2^0$, mesh $3_2^1$, mesh $3_3^0$ and mesh $3_3^2$, it is used $n_{\upzeta, \mathrm{f}}=2\check{p}_\upzeta+1$ basis functions in the radial direction for the finite fluid domain and $n_{\upzeta, \mathrm{s}}=\check{p}_\upzeta+1$ basis functions in the radial direction for the solid domain. For mesh $4_2^{\textsc{fem}}$ and mesh $4_2^0$, mesh $4_2^1$, mesh $4_3^0$ and mesh $4_3^2$, the corresponding numbers are $n_{\upzeta, \mathrm{f}}=4\check{p}_\upzeta+1$ and $n_{\upzeta, \mathrm{s}}=2\check{p}_\upzeta+1$, respectively.
%In~\Cref{Fig2:compFEMandIGAmesh3p2}, \Cref{Fig2:compFEMandIGAmesh3p3}, \Cref{Fig2:compFEMandIGAmesh4p2}, \Cref{Fig2:compFEMandIGAmesh4p3} we compare the far field pattern of the exact solution and the numerical solution on different meshes using different polynomial degrees. The most informative plots are found in the corresponding error plots in~\Cref{Fig2:compFEMandIGAmesh3p2_error}, \Cref{Fig2:compFEMandIGAmesh3p3_error}, \Cref{Fig2:compFEMandIGAmesh4p2_error} and \Cref{Fig2:compFEMandIGAmesh4p3_error} where we evaluate the error using

In~\Cref{Fig2:compFEMandIGAmesh4p2} and \Cref{Fig2:compFEMandIGAmesh4p3} we compare the far field pattern of the exact solution and the numerical solution on different meshes using different polynomial degrees. The most informative plots are found in the corresponding error plots in~\Cref{Fig2:compFEMandIGAmesh4p2_error} and \Cref{Fig2:compFEMandIGAmesh4p3_error} where we evaluate the error using
\begin{equation}\label{Eq2:relError}
	\tilde{E}_h = \frac{\left|p_\infty(\vec{P}_{\mathrm{ffp}})-p_{\infty,h}(\vec{P}_{\mathrm{ffp}})\right|}{\left|p_\infty(\vec{P}_{\mathrm{ffp}})\right|}
\end{equation}
where $p_{\infty,h}$ is found (using the numerical solution $p_h$) by \Cref{Eq2:farfieldFormula} and \Cref{Eq2:FarFieldDef}. On such a fine mesh the error from the inexact representation of the geometry in the FEM simulation is of less significance. However, we observe that an increase in the regularity of the basis functions reduces the error.

\tikzsetnextfilename{compFEMandIGAmesh3p2} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $3_2^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_2^0$}
			\addlegendentry{IGA $C^1$, mesh $3_2^1$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=2$ with meshes found in \Cref{Fig2:SphericalShellMesh23_p}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The far-field pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh3p2}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh3p3} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $3_3^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_3^0$}
			\addlegendentry{IGA $C^2$, mesh $3_3^2$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=3$ with meshes found in \Cref{Fig2:SphericalShellMesh23_p}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The far-field pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh3p3}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p2} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $4_2^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_2^0$}
			\addlegendentry{IGA $C^1$, mesh $4_2^1$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=2$ with meshes found in \Cref{Fig2:SphericalShellMesh23_p}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The far-field pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh4p2}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p3} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $4_3^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_3^0$}
			\addlegendentry{IGA $C^2$, mesh $4_3^2$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=3$ with meshes found in \Cref{Fig2:SphericalShellMesh23_p}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The far-field pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh4p3}
\end{figure}

\tikzsetnextfilename{compFEMandIGAmesh3p2_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p2_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $3_2^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_2^0$}
			\addlegendentry{IGA $C^1$, mesh $3_2^1$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh3p2} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh3p2_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh3p3_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh3_p3_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $3_3^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_3^0$}
			\addlegendentry{IGA $C^2$, mesh $3_3^2$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh3p3} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh3p3_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p2_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p2_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $4_2^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_2^0$}
			\addlegendentry{IGA $C^1$, mesh $4_2^1$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh4p2} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh4p2_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p3_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{myRed},
				{ntnublue},
				{myGreen},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis2/mesh4_p3_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $4_3^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_3^0$}
			\addlegendentry{IGA $C^2$, mesh $4_3^2$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh4p3} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh4p3_error}
\end{figure}

==> contents/resultsAnsDiscussion_old.tex <==
\section{Numerical examples} 
\label{Sec2:resultsDisc}
We start by investigating the pollution effect for the scattering problem on a rigid sphere, and then continue with the acoustic structure interaction (ASI) problem on the spherical shell. Rigid scattering on a sphere and elastic scattering on a spherical shell are often used to verify the methods because both cases admits analytic solutions. The latter case is the only known problem which admits such an analytic solution for the ASI scattering problem in 3D, and is thus especially valuable. Moreover, these cases has been used as a benchmark example for many methods and one is then able to compare the performance of each method on this problem.

The multipole layers for the infinite elements will be placed at $r_n=nr_{\mathrm{a}}$ for $n=1,\dots,N$ (this is suggested by Burnett in~\cite{Burnett1994atd}). Moreover, unless otherwise stated, we shall use the PGU formulation by default for the infinite elements.

\subsection{Plane wave scattered by a rigid sphere}
Let the plane wave (with $\vec{k}=[0, 0, k]^\transpose$)
\begin{equation*}
	p_{\textrm{inc}}(r,\vartheta) = P_{\mathrm{inc}}\euler^{\imag kz} = P_{\mathrm{inc}}\euler^{\imag kr\cos\vartheta}
\end{equation*}
be scattered on a sphere with radius $R=0.5$. That is, we once more send the wave along the $z$-axis (and we shall also align the symmetry axis of the NURBS parametrization along the $y$-axis). The resulting scattered wave is then\footnote{Here, $P_n(x)$ denotes the $n^{\mathrm{th}}$ Legendre polynomial, $j_n(x)$ and $y_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Bessel function of first and second kind, respectively, and finally $h_n(x)$ denotes the $n^{\mathrm{th}}$ spherical Hankel function of the first kind.} (rigid scattering)
\begin{equation}\label{Eq2:rigidScattering_p}
	p_{\mathrm{rs}} (r,\vartheta) = -P_{\mathrm{inc}}\sum_{n=0}^\infty \imag^n (2n+1) P_n(\cos\vartheta)\frac{j_n'(kR)}{h_n'(kR)} h_n(kr).
\end{equation}
For details of this solution see Ihlenburg~\cite[p. 28]{Ihlenburg1998fea}. Since this example has been used in~\cite{Gerdes1999otp} and~\cite{Simpson2014aib}, we may compare our results to other methods on the same problem. We start by comparing the results found in~\cite{Simpson2014aib} by considering $k=2$ (low frequencies), and the construction of NURBS meshes illustrated in \Cref{Fig2:SphericalShellMeshes}. We send the incident wave along the $z$-axis (instead of the $x$-axis) and align the symmetry of the NURBS parametrization along the $y$-axis (instead of the $z$-axis). The results should obviously remain unchanged. We shall use $N=3$, which will practically neglect the error from the infinite element implementation on the coarse meshes considered. For low frequencies and the usage of the PGU formulation, it seems to be advantageous to set the artificial boundary very close to the surface of the sphere. We find the optimal radius to be around $r_{\mathrm{a}}=0.51$. When comparing with BEM, we typically have more liberty of adding degrees of freedom in the radial direction without destroying the fairness of the comparison. This is because the computational time of solving an BEM system of equations is higher than the corresponding IGA/IEM system of equations. It is thus very hard to compare the two methods without running both methods on the same computers. In~\Cref{Fig2:scatteringRigidSphereErrorNearField} we plot the absolute relative error in the scattered field at $r=5$ (as was done in~\cite{Simpson2014aib}). Comparing with the results in~\cite{Simpson2014aib} we observe that BEM has the advantage on the coarsest mesh, but IGA/IEM produce the best results on finer meshes. 
%In~\Cref{Fig2:SphericalShellErrorMesh1}, \Cref{Fig2:SphericalShellErrorMesh2} and \Cref{Fig2:SphericalShellErrorMesh3} we visualize the error at the artificial boundary $\Gamma_{\mathrm{a}}$ both in the scalar field and the normed gradient field for mesh 1, 2 and 3, respectively. The gradient is used to evaluate far field points, so it is of interest to study this error as well. Interestingly, we observe larger errors in the gradient where the basis functions have lower continuity (which occurs at the mesh lines).
\begin{figure}
	\centering
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh1_Zaxis}
		\caption{Mesh 1}
    \end{subfigure}
    ~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh2_Zaxis}
		\caption{Mesh 2}
		\label{Fig2:SphericalShellMeshes2}
    \end{subfigure}
    ~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_Zaxis}
		\caption{Mesh 3}
		\label{Fig2:SphericalShellMeshes3}
    \end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Meshes. The knot $\zeta=0.5$ has been inserted in $\Zeta$ for mesh 2 while the knots $\zeta = 0.25, 0.5, 0.75$ has been inserted in $\Zeta$ for mesh 3 (from the original mesh 1, with NURBS data found in \Cref{Sec2:NURBSdata}).}
	\label{Fig2:SphericalShellMeshes}
\end{figure}

\tikzsetnextfilename{scatteringRigidSphereErrorNearField} 
\begin{figure}
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.94\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow}, % 1
				{mycolor}, % 2
				{myGreen}, % 3
				{myCyan}, % 4
			},
			xtick={0, 45, ..., 360},
			legend style={
				at={(0.97,0.03)},
				anchor=south east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={aspect angle $\alpha$},
			ylabel={$\frac{\big||p_{\mathrm{rs}}| - \left|p_h^N\right|\big|}{|p_{\mathrm{rs}}|}$},
			%ymax=100
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh1_180_0_formul_PGU_error.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh2_180_0_formul_PGU_error.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/simpsonExample/k_2_mesh3_180_0_formul_PGU_error.dat};
			\addlegendentry{Mesh 1}
			\addlegendentry{Mesh 2}
			\addlegendentry{Mesh 3}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} The relative error for the near field  $k=2$. The near field is plotted over all aspect angles $\alpha$ at $r=5$.}
	\label{Fig2:scatteringRigidSphereErrorNearField}
\end{figure}
%\begin{figure}
%	\centering
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis1Error}
%		\caption{Relative error in the scattered field}
%    \end{subfigure}
%	\par\bigskip	
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis1ErrorGradient}
%		\caption{Relative error in the gradient of the scattered field}
%    \end{subfigure}
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Relative errors for mesh 1 (not in percentage). The direction of the incident wave is given by $\alpha_{\mathrm{s}} = 180^\circ$.}
%	\label{Fig2:SphericalShellErrorMesh1}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis2Error}
%		\caption{Relative error in the scattered field}
%    \end{subfigure}
%	\par\bigskip	
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis2ErrorGradient}
%		\caption{Relative error in the gradient of the scattered field}
%    \end{subfigure}
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Relative errors for mesh 2 (not in percentage). The direction of the incident wave is given by $\alpha_{\mathrm{s}} = 180^\circ$.}
%	\label{Fig2:SphericalShellErrorMesh2}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis3Error}
%		\caption{Relative error in the scattered field}
%    \end{subfigure}
%	\par\bigskip	
%	\begin{subfigure}{\textwidth}
%		\centering
%		\includegraphics[scale=0.16]{../../graphics/sphericalShellMeshYaxis3ErrorGradient}
%		\caption{Relative error in the gradient of the scattered field}
%    \end{subfigure}
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Relative errors for mesh 3 (not in percentage). The direction of the incident wave is given by $\alpha_{\mathrm{s}} = 180^\circ$.}
%	\label{Fig2:SphericalShellErrorMesh3}
%\end{figure}

Finally, we present the results from IGA on the pollution effect by comparing the IGA results to the so-called best approximation. We shall follow~\cite{Gerdes1999otp} in comparing the IGA results with the so-called best approximation (BA). This solution represent the best possible solution in the solution space. The BA solution is found by solving: Find $p_h^{\mathrm{ba}}\in \calV_h(\Omega_{\mathrm{a}})$ such that
\begin{equation*}
	\left(p_h^{\mathrm{ba}},q_h\right)_{H^1(\Omega_{\mathrm{a}})} = \left(p, q_h\right)_{H^1(\Omega_{\mathrm{a}})}
\end{equation*}
where $\left(p,q\right)_{H^1(\Omega_{\mathrm{a}})}$ is the $H^1$-inner product
\begin{equation*}
	\left(p,q\right)_{H^1(\Omega_{\mathrm{a}})} = \int_{\Omega_{\mathrm{a}}}\nabla p\cdot\nabla \bar{q} + p \bar{q}\idiff\Omega.
\end{equation*}
We denote by
\begin{equation}\label{Eq2:H1relError}
	E_h^N = \frac{\left\|p_{\mathrm{rs}}-p_h^N\right\|_{H^1(\Omega_{\mathrm{a}})}}{\left\|p_{\mathrm{rs}}\right\|_{H^1(\Omega_{\mathrm{a}})}},
\end{equation}
the absolute relative error with corresponding formula for $p_h^{\mathrm{ba}}$. We shall replicate the problem setup by Gerdes and Ihlenburg~\cite{Gerdes1999otp} which uses $N=6$ radial basis function in the infinite elements, and truncate \Cref{Eq2:rigidScattering_p} at $n=6$ to eliminate the error originating from the artificial boundary.

%For convenience we duplicate the results in~\cite{Gerdes1999otp} in table \Cref{Tab2:gerdesIhlenburgTableResults_p4} and \Cref{Tab2:gerdesIhlenburgTableResults_p3}. The corresponding IGA results are reported in \Cref{Tab2:p4} and \Cref{Tab2:p3}. What we generally observe is that the difference between the IGA results and the BA results is smaller than the corresponding results from FEA. This suggest that IGA handles the pollution effect better then the classical FEA.

In \Cref{Fig2:SphericalShellMesh34_p} we illustrate the surface structure of the mesh used in the analysis. Let $\mathrm{noSurfDofs}()$ be a function counting the number of degrees of freedom on the surface of a given mesh. If the surface NURBS order is 2, then 
\begin{align*}
	\mathrm{noSurfDofs}(\mathrm{Mesh }3_0) &= \mathrm{noSurfDofs}(\mathrm{Mesh }3_1) = 482\\
	\mathrm{noSurfDofs}(\mathrm{Mesh }4_0) &= \mathrm{noSurfDofs}(\mathrm{Mesh }4_1) = 1986.
\end{align*}
If the surface NURBS order is 3, then 
\begin{align*}
	\mathrm{noSurfDofs}(\mathrm{Mesh }3_0) &= \mathrm{noSurfDofs}(\mathrm{Mesh }3_2) = 1106\\
	\mathrm{noSurfDofs}(\mathrm{Mesh }4_0) &= \mathrm{noSurfDofs}(\mathrm{Mesh }4_2) = 4514.
\end{align*}
We report the results in \Cref{Tab2:BAresults} and for illustrative purposes, we also plot this data in \Cref{Fig2:plot_p2q2mesh3}, \Cref{Fig2:plot_p2q2mesh4}, \Cref{Fig2:plot_p2q3mesh3}, \Cref{Fig2:plot_p2q3mesh4}, \Cref{Fig2:plot_p3q2mesh3}, \Cref{Fig2:plot_p3q2mesh4}, \Cref{Fig2:plot_p3q3mesh3} and \Cref{Fig2:plot_p3q3mesh4}. We firstly observe that the BA solution indeed yields the best results, but also the fact that the numerical results is quite close to this solution. In~\cite{Gerdes1999otp} Gerdes and Ihlenburg reports a far greater difference between the BA and the FEM solution. This can only come from the fact we here use exact geometry. To the extent that one may compare the two methods and the data which has been given, one should conclude that IGA performs much better than classical FEM. Moreover, we generally observe the presence of the pollution effect; for higher wave numbers we obtain less accurate results. A final general remark is the fact that we always obtain better results with higher continuity. 

The pollution effect is observed in \Cref{Fig2:plot_p2q2mesh3} (where the least amount of dofs has been used). We here observe that the solution quickly reach the optimal solution for a given set of radial basis function, whereas the same optimality lags behind for higher frequencies. The same tendency is observed in~\Cref{Fig2:plot_p2q2mesh4} where we increase the number of angular elements. The difference is observed in the fact that we get better results and we may use more dofs in the radial direction before we reach the optimal solution. A more extreme version of these two first figures may be observed in~\Cref{Fig2:plot_p2q3mesh3} and \Cref{Fig2:plot_p2q3mesh4} where we increase the radial polynomial degree in these two cases. The finale four figures only increases the angular polynomial order of the preceding four figures by one. We may then begin to observe the expected optimal convergence order as the main source of error comes from the low resolution in the radial direction (that is, inserting more elements in the angular direction will not improve the result notably). 


%\begin{table}
%	\tiny
%	\centering
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and FEA with angular degree $p=4$ collected from~\cite{Gerdes1999otp}. Mesh 2 and 3 are depicted in~\cite[Figure 3a]{Gerdes1999otp} and~\cite[Figure 3b]{Gerdes1999otp}, respectively. Other mesh parameters include the radial NURBS order $q$ and the number of element layers in radial direction $n_\upzeta$. As usual, $k$ is the wave number. The errors are measured in the normalized $H^1$-norm given in percentage.}
%	\label{Tab2:gerdesIhlenburgTableResults_p4}
%	\bgroup
%	\def\arraystretch{1.1}
%	\begin{tabular}{l l S S S S S S S S S S S}
%		\hline
%		\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\check{p}_\upzeta=2$} 							&& \multicolumn{5}{c}{$\check{p}_\upzeta=3$}\\ 
%		\cline{3-7} \cline{9-13}
%		\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh 2} 	&& \multicolumn{2}{c}{Mesh 3} 	&& \multicolumn{2}{c}{Mesh 2} && \multicolumn{2}{c}{Mesh 3}\\ 
%		\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
%		$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEA} 		&& {BA} 		& {FEA} 		&& {BA} 		& {FEA} 		&& {BA} 		& {FEA}		\\
%		\hline
%		\input{../../matlab/plotData/pollutionAnalysis/gerdesIhlenburgTableResults_p4}
%	    \hline
%	\end{tabular}
%	\egroup
%
%	\par\bigskip		
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and FEA with angular degree $\check{p}_\upxi=3$ collected from~\cite{Gerdes1999otp}\protect\footnotemark. Mesh 2 and 3 are depicted in~\cite[Figure 3a]{Gerdes1999otp} and~\cite[Figure 3b]{Gerdes1999otp}, respectively. Other mesh parameters include the radial NURBS order $q$ and the number of element layers in radial direction $n_\upzeta$. As usual, $k$ is the wave number. The errors are measured in the normalized $H^1$-norm given in percentage.}
%	\label{Tab2:gerdesIhlenburgTableResults_p3}
%	\bgroup
%	\def\arraystretch{1.1}
%	\begin{tabular}{l l S S S S S S S S S S S}
%		\hline
%		\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\check{p}_\upzeta=2$} 							&& \multicolumn{5}{c}{$\check{p}_\upzeta=3$}\\ 
%		\cline{3-7} \cline{9-13}
%		\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh 2} 	&& \multicolumn{2}{c}{Mesh 3} 	&& \multicolumn{2}{c}{Mesh 2} && \multicolumn{2}{c}{Mesh 3}\\ 
%		\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
%		$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEA} 		&& {BA} 		& {FEA} 		&& {BA} 		& {FEA} 		&& {BA} 		& {FEA}		\\
%		\hline
%		\input{../../matlab/plotData/pollutionAnalysis/gerdesIhlenburgTableResults_p3}
%	    \hline
%	\end{tabular}
%\egroup
%\end{table}
%
%\footnotetext{A typo has been assumed to have occurred in~\cite{Gerdes1999otp} in the three last rows for $n_\upzeta$; \\It should be 2, 4 and 8 instead of 1, 2 and 4.}
%\begin{table}
%	\tiny
%	\centering
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and IGA with angular NURBS order $p=4$. Mesh 2 and 3 are depicted in \Cref{Fig2:SphericalShellMeshes2} and \Cref{Fig2:SphericalShellMeshes3}, respectively. Other mesh parameters include the radial NURBS order $q$ and the number of element layers in radial direction $n_\upzeta$. As usual, $k$ is the wave number. The errors are measured in the normalized $H^1$-norm given in percentage.}
%	\label{Tab2:p4}
%	\bgroup
%	\def\arraystretch{1.1}
%	\begin{tabular}{l l S S S S S S S S S S S}
%		\hline
%		\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\check{p}_\upzeta=2$} 							&& \multicolumn{5}{c}{$\check{p}_\upzeta=3$}\\ 
%		\cline{3-7} \cline{9-13}
%		\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh 2} 	&& \multicolumn{2}{c}{Mesh 3} 	&& \multicolumn{2}{c}{Mesh 2} && \multicolumn{2}{c}{Mesh 3}\\ 
%		\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
%		$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
%		\hline
%		\input{../../matlab/plotData/pollutionAnalysis/p4}
%	    \hline
%	\end{tabular}
%	\egroup
%	
%	\par\bigskip		
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and IGA with angular degree $\check{p}_\upxi=3$. Mesh 2 and 3 are depicted in \Cref{Fig2:SphericalShellMeshes2} and \Cref{Fig2:SphericalShellMeshes3}, respectively. Other mesh parameters include the radial NURBS order $q$ and the number of element layers in radial direction $n_\upzeta$. As usual, $k$ is the wave number. The errors are measured in the normalized $H^1$-norm given in percentage.}
%	\label{Tab2:p3}
%	\bgroup
%	\def\arraystretch{1.1}
%	\begin{tabular}{l l S S S S S S S S S S S}
%		\hline
%		\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\check{p}_\upzeta=2$} 							&& \multicolumn{5}{c}{$\check{p}_\upzeta=3$}\\ 
%		\cline{3-7} \cline{9-13}
%		\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh 2} 	&& \multicolumn{2}{c}{Mesh 3} 	&& \multicolumn{2}{c}{Mesh 2} && \multicolumn{2}{c}{Mesh 3}\\ 
%		\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
%		$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
%		\hline
%		\input{../../matlab/plotData/pollutionAnalysis/p3}
%	    \hline
%	\end{tabular}
%	\egroup
%\end{table}
\begin{figure}
	\centering        
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_0}
		\caption{Mesh $3_0$.}
		\label{Fig2:SphericalShellMesh3_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_1}
		\caption{Mesh $3_1$.}
		\label{Fig2:SphericalShellMesh3_1}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_2}
		\caption{Mesh $3_2$.}
		\label{Fig2:SphericalShellMesh3_2}
	\end{subfigure}
	\par\bigskip  
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_0}
		\caption{Mesh $4_0$.}
		\label{Fig2:SphericalShellMesh4_0}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_1}
		\caption{Mesh $4_1$.}
		\label{Fig2:SphericalShellMesh4_1}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_2}
		\caption{Mesh $4_2$.}
		\label{Fig2:SphericalShellMesh4_2}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Illustration of the angular parametrization (parametrized with the $\xi$ and $\eta$ parameters). The sub index indicates the continuity of the angular parametrization over inserted knots. We insert $2^{s-1}-1$ knots for each knot interval in the $\xi$- and $\eta$-direction using $s=3,4$ for mesh $3_0$ and mesh $4_0$, respectively. To match the same degree of freedom for higher continuity meshes (mesh $3_1$, mesh $3_2$, mesh $4_1$ and mesh $4_2$) we must insert $\check{p}_\upxi\cdot 2^{s-1}-\check{p}_\upxi$ knots where $\check{p}_\upeta=\check{p}_\upxi$ (recall that $\check{p}_\upxi$ is the NURBS order in the $\xi$ direction while $\check{p}_\upeta$ is the NURBS order in the $\eta$ direction).}
	\label{Fig2:SphericalShellMesh34_p}
\end{figure}

\begin{table}
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and IGA. The meshes are found in \Cref{Fig2:SphericalShellMesh34_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:BAresults}
	\begin{subtable}[t]{\linewidth}
		\caption{Results on mesh 3 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p2q2mesh3}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 482\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-10}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_0^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $3_0$} 	&& \multicolumn{2}{c}{Mesh $3_1$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis2/IGAIGA_p2q2mesh3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
%	\begin{subtable}[t]{\linewidth}
%		\caption{Results on mesh 4 with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$, respectively.}
%		\label{Tab2:p2q2mesh4}
%		\centering
%		\bgroup
%		\def\arraystretch{1.1}
%		\begin{tabular}{l l S S S S S S S S}
%			\hline
%			\multicolumn{2}{c}{}				& \multicolumn{8}{c}{$\mathrm{noDofs} = 1986\cdot (n_\upzeta+N-1)$}\\ 
%			\cline{3-10}
%			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $4_0^{\textsc{fem}}$} 	&& \multicolumn{2}{c}{Mesh $4_0$} 	&& \multicolumn{2}{c}{Mesh $4_1$}\\ 
%			\cline{3-4} \cline{6-7}\cline{9-10}
%			$k$ 						& $n_\upzeta$ 	& {BA} 		& {FEM} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}\\
%			\hline
%			\input{../../matlab/plotData/pollutionAnalysis2/IGAIGA_p2q2mesh4}
%		    \hline
%		\end{tabular}
%		\egroup
%	\end{subtable}
\end{table}

	
%
\begin{table}
	\tiny
	\centering
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Convergence results for the best approximation (BA) and IGA. The meshes are found in \Cref{Fig2:SphericalShellMesh34_p}. We denote by $n_\upzeta$, the number of NURBS basis functions in the radial direction. As usual, $k$ is the wave number. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Tab2:BAresults}
	\begin{subtable}[t]{\linewidth}
		\caption{Results with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p2q2}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\mathrm{noDofs} = 482\cdot (n_\upzeta+N-1)$} 							&& \multicolumn{5}{c}{$\mathrm{noDofs} = 1986\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-7} \cline{9-13}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_0$} 	&& \multicolumn{2}{c}{Mesh $3_1$} 	&& \multicolumn{2}{c}{Mesh $4_0$} && \multicolumn{2}{c}{Mesh $4_1$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis/IGAIGA_p2q2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\caption{Results with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p2q3}
		\begin{tabular}{l l S S S S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\mathrm{noDofs} = 482\cdot (n_\upzeta+N-1)$} 							&& \multicolumn{5}{c}{$\mathrm{noDofs} = 1986\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-7} \cline{9-13}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_0$} 	&& \multicolumn{2}{c}{Mesh $3_1$} 	&& \multicolumn{2}{c}{Mesh $4_0$} && \multicolumn{2}{c}{Mesh $4_1$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis/IGAIGA_p2q3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\caption{Results with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$, respectively.}
		\label{Tab2:p3q2}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\begin{tabular}{l l S S S S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\mathrm{noDofs} = 1106\cdot (n_\upzeta+N-1)$} 							&& \multicolumn{5}{c}{$\mathrm{noDofs} = 4514\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-7} \cline{9-13}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_0$} 	&& \multicolumn{2}{c}{Mesh $3_2$} 	&& \multicolumn{2}{c}{Mesh $4_0$} && \multicolumn{2}{c}{Mesh $4_2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis/IGAIGA_p3q2}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
	\par\bigskip
	
	\begin{subtable}[t]{\linewidth}
		\centering
		\bgroup
		\def\arraystretch{1.1}
		\caption{Results with angular and radial NURBS order $\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$, respectively.}
		\label{Tab2:p3q3}
		\begin{tabular}{l l S S S S S S S S S S S}
			\hline
			\multicolumn{2}{c}{}				& \multicolumn{5}{c}{$\mathrm{noDofs} = 1106\cdot (n_\upzeta+N-1)$} 							&& \multicolumn{5}{c}{$\mathrm{noDofs} = 4514\cdot (n_\upzeta+N-1)$}\\ 
			\cline{3-7} \cline{9-13}
			\multicolumn{2}{c}{}				& \multicolumn{2}{c}{Mesh $3_0$} 	&& \multicolumn{2}{c}{Mesh $3_2$} 	&& \multicolumn{2}{c}{Mesh $4_0$} && \multicolumn{2}{c}{Mesh $4_2$}\\ 
			\cline{3-4} \cline{6-7}\cline{9-10} \cline{12-13}
			$k$ 						& $n_\upzeta$ 	& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA} 		&& {BA} 		& {IGA}		\\
			\hline
			\input{../../matlab/plotData/pollutionAnalysis/IGAIGA_p3q3}
		    \hline
		\end{tabular}
		\egroup
	\end{subtable}
\end{table}

%\begin{figure}
%	\tikzsetnextfilename{plot_p2q2mesh3} 
%	\begin{tikzpicture}
%		\begin{loglogaxis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={
%				{myYellow, dashed}, % 1
%				{myYellow}, % 1
%				{mycolor, dashed}, % 2
%				{mycolor}, % 2
%				{myGreen, dashed}, % 1
%				{myGreen}, % 1
%				{myRed, dashed}, % 2
%				{myRed}, % 2
%			},
%			%xtick={0, 45, ..., 360},
%			xtick={3, 5, 9, 17, 33},
%			xticklabels={3, 5, 9, 17, 33},
%			enlarge x limits = true,
%			legend style={
%				at={(0.97,0.97)},
%				anchor=north east,
%				legend columns=1,
%				%cells={anchor=west},
%				font=\footnotesize,
%				rounded corners=2pt
%			},
%			%width=0.45*350pt,
%			%height=0.5*250pt,
%			xlabel={Number of basis function in radial direction, $n_\upzeta$},
%			ylabel=Absolute relative error (\%),
%			xmax=75
%			]Fig:plot_p2q2mesh3
%			% k = 5			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k5reduceCont1.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k5reduceCont1.dat};
%			\addlegendentry{BA $C^0$, $k=5$}
%			\addlegendentry{IGA $C^0$, $k=5$}
%			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k5reduceCont0.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k5reduceCont0.dat};
%			\addlegendentry{BA $C^2$, $k=5$}
%			\addlegendentry{IGA $C^2$, $k=5$}
%			
%			
%			% k = 40
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k40reduceCont1.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k40reduceCont1.dat};
%			\addlegendentry{BA $C^0$, $k=40$}
%			\addlegendentry{IGA $C^0$, $k=40$}
%			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k40reduceCont0.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh3k40reduceCont0.dat};
%			\addlegendentry{BA $C^2$, $k=40$}
%			\addlegendentry{IGA $C^2$, $k=40$}
%		\end{loglogaxis}
%	\end{tikzpicture}
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q2} ($p=2$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $3_0$ in \Cref{Fig2:SphericalShellMesh3_0} and the $C^2$-results uses mesh $3_1$ in \Cref{Fig2:SphericalShellMesh3_1}. All results uses the same noDofs for a given $n_\upzeta$.}
%	\label{Fig2:plot_p2q2mesh3}
%
%	\par\bigskip
%	\tikzsetnextfilename{plot_p2q2mesh4}
%	\begin{tikzpicture}
%		\begin{loglogaxis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={
%				{myYellow, dashed}, % 1
%				{myYellow}, % 1
%				{mycolor, dashed}, % 2
%				{mycolor}, % 2
%				{myGreen, dashed}, % 1
%				{myGreen}, % 1
%				{myRed, dashed}, % 2
%				{myRed}, % 2
%			},
%			%xtick={0, 45, ..., 360},
%			xtick={3, 5, 9, 17, 33},
%			xticklabels={3, 5, 9, 17, 33},
%			enlarge x limits = true,
%			legend style={
%				at={(0.97,0.97)},
%				anchor=north east,
%				legend columns=1,
%				%cells={anchor=west},
%				font=\footnotesize,
%				rounded corners=2pt
%			},
%			%width=0.45*350pt,
%			%height=0.5*250pt,
%			xlabel={Number of basis function in radial direction, $n_\upzeta$},
%			ylabel=Absolute relative error (\%),
%			xmax=75
%			]
%			% k = 5			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont1.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont1.dat};
%			\addlegendentry{BA $C^0$, $k=5$}
%			\addlegendentry{IGA $C^0$, $k=5$}
%			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont0.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont0.dat};
%			\addlegendentry{BA $C^2$, $k=5$}
%			\addlegendentry{IGA $C^2$, $k=5$}
%			
%			
%			% k = 40
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont1.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont1.dat};
%			\addlegendentry{BA $C^0$, $k=40$}
%			\addlegendentry{IGA $C^0$, $k=40$}
%			
%			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont0.dat};
%			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont0.dat};
%			\addlegendentry{BA $C^2$, $k=40$}
%			\addlegendentry{IGA $C^2$, $k=40$}
%		\end{loglogaxis}
%	\end{tikzpicture}
%	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q2} ($p=2$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $4_0$ in \Cref{Fig2:SphericalShellMesh4_0} and the $C^2$-results uses mesh $4_1$ in \Cref{Fig2:SphericalShellMesh4_1}. All results uses the same noDofs for a given $n_\upzeta$.}
%	\label{Fig2:plot_p2q2mesh4}
%\end{figure}
\begin{figure}
	\tikzsetnextfilename{plot_p2q2mesh3} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{mycolor, dashed, mark=triangle*}, % 2
				{mycolor, mark=triangle*}, % 2
				{myGreen, dashed, mark=triangle*}, % 1
				{myGreen, mark=triangle*}, % 1
				{myRed, dashed, mark=triangle*}, % 2
				{myRed, mark=triangle*}, % 2
				{mycolor, dashed, mark=*}, % 2
				{mycolor, mark=*}, % 2
				{myGreen, dashed, mark=*}, % 1
				{myGreen, mark=*}, % 1
				{myRed, dashed, mark=*}, % 2
				{myRed, mark=*}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=5$}
			\addlegendentry{FEM $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k5Case3.dat};
			\addlegendentry{BA IGA $C^1$, $k=5$}
			\addlegendentry{IGA $C^1$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case1.dat};
			\addplot table[x=l,y=FEM] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case1.dat};
			\addlegendentry{BA FEM $C^0$, $k=40$}
			\addlegendentry{FEM $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case2.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case2.dat};
			\addlegendentry{BA IGA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA]  {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case3.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis2/plot_p2q2mesh3k40Case3.dat};
			\addlegendentry{BA IGA $C^1$, $k=40$}
			\addlegendentry{IGA $C^1$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q2} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $3_0$ in \Cref{Fig2:SphericalShellMesh3_0} and the $C^1$-results uses mesh $3_1$ in \Cref{Fig2:SphericalShellMesh3_1}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p2q2mesh3}

	\par\bigskip
	\tikzsetnextfilename{plot_p2q2mesh4} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k5reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=5$}
			\addlegendentry{IGA $C^1$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q2mesh4k40reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=40$}
			\addlegendentry{IGA $C^1$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q2} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $4_0$ in \Cref{Fig2:SphericalShellMesh4_0} and the $C^1$-results uses mesh $4_1$ in \Cref{Fig2:SphericalShellMesh4_1}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p2q2mesh4}
\end{figure}
\begin{figure}
	\tikzsetnextfilename{plot_p2q3mesh3} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k5reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=5$}
			\addlegendentry{IGA $C^1$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh3k40reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=40$}
			\addlegendentry{IGA $C^1$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q3} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=3$). The $C^0$-results uses mesh $3_0$ in \Cref{Fig2:SphericalShellMesh3_0} and the $C^1$-results uses mesh $3_1$ in \Cref{Fig2:SphericalShellMesh3_1}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p2q3mesh3}

	\par\bigskip
	\tikzsetnextfilename{plot_p2q3mesh4} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k5reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=5$}
			\addlegendentry{IGA $C^1$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p2q3mesh4k40reduceCont0.dat};
			\addlegendentry{BA $C^1$, $k=40$}
			\addlegendentry{IGA $C^1$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p2q3} ($\check{p}_\upxi=\check{p}_\upeta=2$ and $\check{p}_\upzeta=3$). The $C^0$-results uses mesh $4_0$ in \Cref{Fig2:SphericalShellMesh4_0} and the $C^1$-results uses mesh $4_1$ in \Cref{Fig2:SphericalShellMesh4_1}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p2q3mesh4}
\end{figure}

\tikzsetnextfilename{plot_p3q2mesh3} 
\begin{figure}
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=75
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k5reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh3k40reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q2} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $3_0$ in \Cref{Fig2:SphericalShellMesh3_0} and the $C^2$-results uses mesh $3_2$ in \Cref{Fig2:SphericalShellMesh3_2}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q2mesh3}

	\par\bigskip
	\tikzsetnextfilename{plot_p3q2mesh4} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={3, 5, 9, 17, 33},
			xticklabels={3, 5, 9, 17, 33},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=75
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k5reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q2mesh4k40reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q2} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=2$). The $C^0$-results uses mesh $4_0$ in \Cref{Fig2:SphericalShellMesh4_0} and the $C^2$-results uses mesh $4_2$ in \Cref{Fig2:SphericalShellMesh4_2}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q2mesh4}
\end{figure}
\tikzsetnextfilename{plot_p3q3mesh3} 
\begin{figure}
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k5reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh3k40reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q3} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$). The $C^0$-results uses mesh $3_0$ in \Cref{Fig2:SphericalShellMesh3_0} and the $C^2$-results uses mesh $3_2$ in \Cref{Fig2:SphericalShellMesh3_2}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q3mesh3}
	
	\par\bigskip
	\tikzsetnextfilename{plot_p3q3mesh4} 
	\begin{tikzpicture}
		\begin{loglogaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={
				{myYellow, dashed}, % 1
				{myYellow}, % 1
				{mycolor, dashed}, % 2
				{mycolor}, % 2
				{myGreen, dashed}, % 1
				{myGreen}, % 1
				{myRed, dashed}, % 2
				{myRed}, % 2
			},
			%xtick={0, 45, ..., 360},
			xtick={4, 7, 13, 25, 49},
			xticklabels={4, 7, 13, 25, 49},
			enlarge x limits = true,
			legend style={
				at={(0.97,0.97)},
				anchor=north east,
				legend columns=1,
				%cells={anchor=west},
				font=\footnotesize,
				rounded corners=2pt
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			xlabel={Number of basis function in radial direction, $n_\upzeta$},
			ylabel=Absolute relative error (\%),
			xmax=115
			]
			% k = 5			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k5reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k5reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=5$}
			\addlegendentry{IGA $C^0$, $k=5$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k5reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k5reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=5$}
			\addlegendentry{IGA $C^2$, $k=5$}
			
			
			% k = 40
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k40reduceCont1.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k40reduceCont1.dat};
			\addlegendentry{BA $C^0$, $k=40$}
			\addlegendentry{IGA $C^0$, $k=40$}
			
			\addplot table[x=l,y=BA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k40reduceCont0.dat};
			\addplot table[x=l,y=IGA] {../../matlab/plotData/pollutionAnalysis/plot_p3q3mesh4k40reduceCont0.dat};
			\addlegendentry{BA $C^2$, $k=40$}
			\addlegendentry{IGA $C^2$, $k=40$}
		\end{loglogaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by a rigid sphere:} Plot of the results reported in \Cref{Tab2:p3q3} ($\check{p}_\upxi=\check{p}_\upeta=3$ and $\check{p}_\upzeta=3$). The $C^0$-results uses mesh $4_0$ in \Cref{Fig2:SphericalShellMesh4_0} and the $C^2$-results uses mesh $4_2$ in \Cref{Fig2:SphericalShellMesh4_2}. All results uses the same noDofs for a given $n_\upzeta$. The errors are found using \Cref{Eq2:H1relError} and are given in percentage.}
	\label{Fig2:plot_p3q3mesh4}
\end{figure}

\clearpage
\subsection{Plane wave scattered by an elastic spherical shell}
We now turn to the acoustic-structure interaction (ASI) problem on a spherical shell where we want to compare classical FEM and IGA.

In~\cite[pp. 12-20]{Chang1994voa} the exact 3D elasticity solution for the spherical shell is presented. We shall repeat the final formulas needed for the scattered pressure.
Let the plane wave
\begin{equation*}
	p_{\textrm{inc}}(r,\vartheta) = P_{\mathrm{inc}}\euler^{\imag kz} = P_{\mathrm{inc}}\euler^{\imag kr\cos\vartheta}
\end{equation*}
be scattered on a elastic spherical shell with inner radius $R_1$ and outer radius $R_0$. The scattered pressure is then (elastic scattering)
\begin{equation}\label{Eq2:exact3DscatteringSphericalShellSol}
	p_{\mathrm{es}}(r,\vartheta) = p_{\mathrm{rs}}(r,\vartheta) + \frac{P_{\mathrm{inc}}\rho_{\mathrm{f}} c_{\mathrm{f}}}{(kR_0)^2}\sum_{n=0}^\infty \frac{\imag^n(2n+1)P_n(\cos\vartheta)h_n(kr)}{[h_n'(kR_0)]^2(Z_n+z_n)}
\end{equation}
where $p_{\mathrm{rs}}$ is defined in \Cref{Eq2:rigidScattering_p}, and $z_n$ (\textit{specific acoustic impedance}) and $Z_n$ (\textit{mechanical impedance}) are defined by
\begin{equation*}
	z_n = \imag\rho_{\mathrm{f}} c_{\mathrm{f}}\frac{h_n(kR_0)}{h_n'(kR_0)}
\end{equation*}
and
\begin{equation*}
	Z_n =\frac{R_0}{-\imag\omega\left[C_n^{(1)} D_{1,n}^{(1)}(b_1 R_0) + C_n^{(2)} D_{2,n}^{(1)}(b_2 R_0) + C_n^{(3)} D_{1,n}^{(2)}(b_1 R_0) + C_n^{(4)} D_{2,n}^{(2)}(b_2 R_0)\right]}
\end{equation*}
where 
\begin{equation*}
	D_{1,n}^{(i)}(x) = nA_n^{(i)}(x)-xA_{n+1}^{(i)}(x),\qquad	D_{2,n}^{(i)}(x) = n(n+1)A_n^{(i)}(x)	
\end{equation*}
and the coefficients $C_n^{(1)}$, $C_n^{(2)}$, $C_n^{(3)}$ and $C_n^{(4)}$ are given by
\begin{equation*}
	C_0^{(1)} = \frac{\frac{R_0^2}{2\mu}B_{1,n}^{(2)}(b_1 R_1)}{\nabla^2_0},\quad C_0^{(2)}=0,\quad
	C_0^{(3)} = -\frac{\frac{R_0^2}{2\mu}B_{1,n}^{(1)}(b_1 R_1)}{\nabla^2_0},\quad C_0^{(4)}=0
\end{equation*}
for $n=0$ where
\begin{equation*}
	\nabla^2_0=\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_0) & B_{1,n}^{(2)}(b_1 R_0)\\
		B_{1,n}^{(1)}(b_1 R_1) & B_{1,n}^{(2)}(b_1 R_1)
	\end{vmatrix},
\end{equation*}
and by
\begin{equation*}
	C_n^{(1)} = \frac{\nabla^2_{1,n}}{\nabla^2_n},\quad C_n^{(2)} = \frac{\nabla^2_{2,n}}{\nabla^2_n},\quad C_n^{(3)} = \frac{\nabla^2_{3,n}}{\nabla^2_n},\quad C_n^{(4)} = \frac{\nabla^2_{4,n}}{\nabla^2_n}
\end{equation*}
for $n>0$ where the following notations has been used
\begin{equation*}
	\nabla^2_n = \begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_0) & B_{2,n}^{(1)}(b_2 R_0) & B_{1,n}^{(2)}(b_1 R_0) & B_{2,n}^{(2)}(b_2 R_0)\\
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{1,n} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{2,n} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{1,n}^{(2)}(b_1 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{3,n}^{(2)}(b_1 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{3,n}^{(2)}(b_1 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{3,n} = \frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{2,n}^{(2)}(b_2 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{4,n}^{(2)}(b_2 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{4,n}^{(2)}(b_2 R_1)
	\end{vmatrix}
\end{equation*}
\begin{equation*}
	\nabla^2_{4,n} = -\frac{R_0^2}{2\mu}\begin{vmatrix}
		B_{1,n}^{(1)}(b_1 R_1) & B_{2,n}^{(1)}(b_2 R_1) & B_{1,n}^{(2)}(b_1 R_1)\\
		B_{3,n}^{(1)}(b_1 R_0) & B_{4,n}^{(1)}(b_2 R_0) & B_{3,n}^{(2)}(b_1 R_0)\\
		B_{3,n}^{(1)}(b_1 R_1) & B_{4,n}^{(1)}(b_2 R_1) & B_{3,n}^{(2)}(b_1 R_1)
	\end{vmatrix}.
\end{equation*}
\begin{align*}
	B_{1,n}^{(i)}(x) &= \left[n^2-n-\frac{1}{2}\left(\frac{b_2}{b_1}\right)^2 x^2\right] A_n^{(i)}(x) + 2xA_{n+1}^{(i)}(x)\\
	B_{2,n}^{(i)}(x) &= n(n+1)\left[(n-1)A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\right]\\
	B_{3,n}^{(i)}(x) &= (n-1) A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\\
	B_{4,n}^{(i)}(x) &= \left(n^2-1-\frac{1}{2}x^2\right) A_n^{(i)}(x) + xA_{n+1}^{(i)}(x)
\end{align*}
%\begin{align*}
%	B_9^{(i)}(x) &= \left[-n^2-\frac{1}{2}\left(\frac{b_2}{b_1}\right)^2 x^2+x^2\right] A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\\
%	B_7^{(i)}(x) &= -(n^2+n)\left[n A_n^{(i)}(x) - xA_{n+1}^{(i)}(x)\right] \\
%	B_5^{(i)}(x) &= \left[n-\frac{1}{2}x^2+\left(\frac{b_1}{b_2}\right)^2 x^2\right] A_n^{(i)}\left(\frac{b_1}{b_2}x\right) - \frac{b_1}{b_2}x A_{n+1}^{(i)}\left(\frac{b_1}{b_2}x\right)\\
%	B_6^{(i)}(x) &= n(n+1)A_n^{(i)}(x)\\
%\end{align*}
\begin{equation*}
	A_{n}^{(1)}(x) = j_n(x),\quad\text{and}\quad A_{n}^{(2)}(x) = y_n(x),
\end{equation*}
\begin{equation*}
	b_1=\frac{\omega}{c_1},\quad b_2=\frac{\omega}{c_2},\quad c_1 = \sqrt{\frac{\lambda+2\mu}{\rho_s}},\quad c_2 = \sqrt{\frac{\mu}{\rho_s}}.
\end{equation*}
Here, the parameters $c_1$ and $c_2$ are called the longitudinal wave velocity and shear wave velocity, respectively. Moreover, $\lambda$ and $\mu$ are the Lam{\'e} parameters which can be defined by the Young's modulus, $E$, and Poisson's ratio, $\nu$, as
\begin{equation*}
	\lambda = \frac{\nu E}{(1+\nu)(1-2\nu)}\quad\text{and}\quad \mu = \frac{E}{2(1+\nu)}.
\end{equation*}
The material parameters are found in \Cref{Tab2:sphericalShellParameters}, and we shall use $r_{\mathrm{a}}=6$ and $N=3$ radial shape functions in the infinite elements. Moreover, we shall use the PGU formulation for the infinite elements. For each experiment we use the same NURBS order everywhere. Denote by $\check{p}_\upxi = p_{\upxi,\mathrm{f}} = p_{\upxi,\mathrm{s}}$ the common NURBS order in the fluid and the solid in the $\xi$-direction. Similarly $\check{p}_\upeta = p_{\upeta,\mathrm{f}} = p_{\upeta,\mathrm{s}}$ and $\check{p}_\upzeta = p_{\upzeta,\mathrm{f}} = p_{\upzeta,\mathrm{s}}$. For each experiment we will use $\check{p}_\upxi = \check{p}_\upeta = \check{p}_\upzeta$.

\begin{table}
	\centering
	\caption[Parameters for spherical shell]{\textbf{Scattering on spherical shell:} Parameters.}
	\label{Tab2:sphericalShellParameters}
	\begin{tabular}{l l}
		\toprule
		Parameter & Description\\
		\midrule
		$E = 2.07\cdot 10^{11}\unit{Pa}$ & Young's modulus\\
		$\rho_{\mathrm{s}} = 7669\unit{kg/m^3}$ & Density of solid\\
		$\rho_{\mathrm{f}} = 1000\unit{kg/m^3}$ & Density of fluid\\
		$\nu = 0.3$ & Poisson's ratio\\
		$c_{\mathrm{f}} = 1524\unit{m/s}$ & Fluid speed of sound\\
		$t_{\mathrm{s}} = 0.15\unit{m}$ & Thickness of the shell\\
		$R = 5\unit{m}$ & Radius of the midsurface of the shell\\
		$R_1 = 4.925\unit{m}$ & Inner radius of the shell\\
		$R_0 = 5.075\unit{m}$ & Outer radius of the shell\\
		$P_{\mathrm{inc}} = 1$ & Amplitude of incident wave\\
		\bottomrule
	\end{tabular}
\end{table}

In order to compare classical FEM and IGA on the scattering problem on the spherical shell, we shall transform the NURBS mesh to a classical FEM mesh. In~\Cref{Fig2:SphericalShellMesh34_p_FSI} we add the equivalent FEM meshes which contain the same noDofs as the IGA meshes, respectively. These new meshes are still NURBS parametrizations, and are created by repeating every knot in the IGA mesh such that every internal knot has multiplicity $m=\check{p}_\upxi$ in the $\xi$-direction and correspondingly in the other two directions. Moreover, to get the polygon elements, we simply project every control point which does not lie on the surface, to the surface of its corresponding polygon element. Finally, all weights are set to be 1. It should be noted that the FEM analysis will then use the Bernstein basis instead of the classical Lagrange basis. However, both of these set of functions spans the same spaces, such that the results should be identical.
\begin{figure}
	\centering        
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_0_FEM}
		\caption{Mesh $3_0^{\textsc{fem}}$.}
		\label{Fig2:SphericalShellMesh3_0_FEM}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_0}
		\caption{Mesh $3_0$.}
		\label{Fig2:SphericalShellMesh3_0_FSI}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_1}
		\caption{Mesh $3_1$.}
		\label{Fig2:SphericalShellMesh3_1_FSI}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh3_2}
		\caption{Mesh $3_2$.}
		\label{Fig2:SphericalShellMesh3_2_FSI}
	\end{subfigure}
	\par\bigskip  
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_0_FEM}
		\caption{Mesh $4_0^{\textsc{fem}}$.}
		\label{Fig2:SphericalShellMesh4_0_FEM}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_0}
		\caption{Mesh $4_0$.}
		\label{Fig2:SphericalShellMesh4_0_FSI}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_1}
		\caption{Mesh $4_1$.}
		\label{Fig2:SphericalShellMesh4_1_FSI}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{../../graphics/sphericalShellMesh4_2}
		\caption{Mesh $4_2$.}
		\label{Fig2:SphericalShellMesh4_2_FSI}
	\end{subfigure}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell:} Illustration of the angular parametrization (parametrized with the $\xi$ and $\eta$ parameters). The sub index indicates the continuity of the parametrization over inserted knots. The structure of the angular parametrization is equal for both the finite fluid domain (inside $\Gamma_{\mathrm{a}}$) and the solid domain. For mesh $3_0^{\textsc{fem}}$ and mesh $3_i$, $i=0,1,2$, it is used $n_{\upzeta, \mathrm{f}}=2\check{p}_\upzeta+1$ basis functions in the radial direction for the finite fluid domain and $n_{\upzeta, \mathrm{s}}=\check{p}_\upzeta+1$ basis functions in the radial direction for the solid domain. For mesh $4_0^{\textsc{fem}}$ and mesh $4_i$, $i=0,1,2$, the corresponding numbers are $n_{\upzeta, \mathrm{f}}=4\check{p}_\upzeta+1$ and $n_{\upzeta, \mathrm{s}}=2\check{p}_\upzeta+1$, respectively.}
	\label{Fig2:SphericalShellMesh34_p_FSI}
\end{figure}

In~\Cref{Fig2:compFEMandIGAmesh3p2}, \Cref{Fig2:compFEMandIGAmesh3p3}, \Cref{Fig2:compFEMandIGAmesh4p2}, \Cref{Fig2:compFEMandIGAmesh4p3} we compare the far field pattern of the exact solution and the numerical solution on different meshes using different polynomial degrees. The most informative plots are found in the corresponding error plots in~\Cref{Fig2:compFEMandIGAmesh3p2_error}, \Cref{Fig2:compFEMandIGAmesh3p3_error}, \Cref{Fig2:compFEMandIGAmesh4p2_error} and \Cref{Fig2:compFEMandIGAmesh4p3_error} where we evaluate the error using
\begin{equation}\label{Eq2:relError}
	E_h = \frac{\left|p_\infty(\vec{P}_{\mathrm{ffp}})-p_{\infty,h}(\vec{P}_{\mathrm{ffp}})\right|}{\left|p_\infty(\vec{P}_{\mathrm{ffp}})\right|}.
\end{equation}
where $p_{0,h}$ is found (using the numerical solution $p_h^N$) by \Cref{Eq2:farfieldFormula} and \Cref{Eq2:FarFieldDef}. Once again, we not only observe a significant improvement using the exact geometry, but also when using higher continuity of the basis functions. We observe that if we increase the difference in the continuity between two simulations (which uses the same nodofs), we get a greater difference in the resulting error.

\tikzsetnextfilename{compFEMandIGAmesh3p2} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $3_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_0$}
			\addlegendentry{IGA $C^1$, mesh $3_1$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=2$ with meshes found in \Cref{Fig2:SphericalShellMesh34_p_FSI}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The farfield pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh3p2}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh3p3} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $3_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_0$}
			\addlegendentry{IGA $C^2$, mesh $3_2$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=3$ with meshes found in \Cref{Fig2:SphericalShellMesh34_p_FSI}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The farfield pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh3p3}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p2} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $4_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_0$}
			\addlegendentry{IGA $C^1$, mesh $4_1$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=2$ with meshes found in \Cref{Fig2:SphericalShellMesh34_p_FSI}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The farfield pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh4p2}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p3} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel={$|p_\infty(\alpha_{\mathrm{f}},0)|$},
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case1_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case2_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case3_num.dat};
			\addplot table[x=theta,y=F_k] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case3_exact.dat};
			\addlegendentry{FEM $C^0$, mesh $4_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_0$}
			\addlegendentry{IGA $C^2$, mesh $4_2$}
			\addlegendentry{Exact}
		\end{axis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Results using $p=q=3$ with meshes found in \Cref{Fig2:SphericalShellMesh34_p_FSI}. The exact solution is given in \Cref{Eq2:exact3DscatteringSphericalShellSol}. The farfield pattern $|p_\infty(\alpha_{\mathrm{f}},\beta_{\mathrm{f}})|$ at aspect angle $\alpha_{\mathrm{f}}$ and elevation angle $\beta_{\mathrm{f}}$ is defined in \Cref{Eq2:FarFieldDef}.}
\label{Fig2:compFEMandIGAmesh4p3}
\end{figure}

\tikzsetnextfilename{compFEMandIGAmesh3p2_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p2_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $3_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_0$}
			\addlegendentry{IGA $C^1$, mesh $3_1$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh3p2} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh3p2_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh3p3_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh3_p3_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $3_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $3_0$}
			\addlegendentry{IGA $C^1$, mesh $3_2$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh3p3} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh3p3_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p2_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p2_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $4_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_0$}
			\addlegendentry{IGA $C^1$, mesh $4_1$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh4p2} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh4p2_error}
\end{figure}
\tikzsetnextfilename{compFEMandIGAmesh4p3_error} 
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{semilogyaxis}[
			width = 0.95\textwidth,
			height = 0.3\paperheight,
			cycle list={%
				{mycolor},
				{myGreen},
				{myRed},
				{black},
			},
			xtick={0, 45, ..., 360},
			legend style={
			at={(0.97,0.97)},
			anchor=north east
			},
			%width=0.45*350pt,
			%height=0.5*250pt,
			%xtick={0.2, 0.25, 0.3, 0.35, 0.4, 0.45, 0.5},
			xlabel={$\alpha_{\mathrm{f}}$},
			ylabel=Absolute relative error (in \%),
%			xmin=0.2,
%			xmax=0.525,
%			ymax=25
			]
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case1.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case2.dat};
			\addplot table[x=theta,y=error] {../../matlab/plotData/FEMvsIGAanalysis/mesh4_p3_Case3.dat};
			\addlegendentry{FEM $C^0$, mesh $4_0^{\textsc{fem}}$}
			\addlegendentry{IGA $C^0$, mesh $4_0$}
			\addlegendentry{IGA $C^1$, mesh $4_2$}
		\end{semilogyaxis}
	\end{tikzpicture}
	\caption{\textbf{Plane wave scattered by an elastic spherical shell}: Same results as in \Cref{Fig2:compFEMandIGAmesh4p3} in terms of the error (in percentage) given by \Cref{Eq2:relError}.}
\label{Fig2:compFEMandIGAmesh4p3_error}
\end{figure}


%\subsection{Scattering on BeTSSi model 3}3
%We shall present both bistatic and monostatic results of scattering on BeTSSi model 3. The main theme in the results will be the pollution effect as the results become less accurate for high frequencies using the same mesh. It will illustrate the importance of mesh refinement for the increase in the frequency.
%
%In all results, we have set the elevation angle of the incident wave and the far field point to be zero, that is $\beta_{\mathrm{s}}=0$ and $\beta_{\mathrm{f}}=0$. 
%
%Most of the results will be compared with results obtained from Ilkka Karasalo and Martin Østberg at FOI\footnote{FOI, Totalförsvarets forskningsinstitut, is the Swedish Defence Research Agency.}. They have proposed several methods for solving the scattering problems including the boundary element method (FOI4). For BeTSSi model 3, they exploit the axisymmetry to reduce the computational time, such that the obtained results may not be compared to the obtained results in this thesis when conserning computational time. However, we shall use the results from FOI as reference solutions.
%
%
%\subsubsection{The near field}
%For illustrative purposes we start by plotting (the real part of) the near field for $f=500\unit{Hz}$ and $f=1\unit{kHz}$, and for the aspect angles $\alpha_{\mathrm{s}} = 240^\circ$ and $\alpha_{\mathrm{s}}=300^\circ$. In \Cref{Fig2:mesh5bistatic_f_500alpha240} and \Cref{Fig2:mesh5bistatic_f_500alpha300} we consider $f=500\unit{Hz}$ with the aspect angles $\alpha_{\mathrm{s}} = 240^\circ$ and $\alpha_{\mathrm{s}}=300^\circ$, respectively. The incident wave at aspect angle $\alpha_{\mathrm{s}}=240^\circ$ arrives normal to the surface of BeTSSi model 3 only at one point, namely a point on the larger hemisphere. From here the scattered waves form a locally spherical wave pattern, as expected. What is peculiar about these plots is the ``shadow'' area behind BeTSSi model 3 where one should expect lower pressure. Instead we see waves forming with higher amplitude compared to the other scattered wave. This is because these waves do not represent the total pressure field\footnote{Which we here define to be the superposition of the incident field and the scattered pressure.}, rather they represents the canceling part of the incident wave such that the total field indeed is reduced in this area. We call this area the shadow area, as the model casts a shadow behind itself. All of these effects are also observed when $\alpha_{\mathrm{s}}=300^\circ$ in \Cref{Fig2:mesh5bistatic_f_500alpha300}. The corresponding two plots for $f=1\unit{kHz}$ in \Cref{Fig2:mesh5bistatic_f_1000alpha240} and \Cref{Fig2:mesh5bistatic_f_1000alpha300} shows the same behavior, with a doubling in the number of waves. However, for higher frequencies, special lines of diffraction patterns emerges in the shadow area.
%\begin{figure}
%	\centering
%	\tikzsetnextfilename{mesh5bistatic_f_500alpha240} 
%	\begin{tikzpicture}
%		\def\scalingFact{41.4}
%			\node[anchor=north west,inner sep=0] at (0,0) {\includegraphics[width=0.8425\textwidth]{../../graphics/mesh5bistatic_f_500alpha240}};
%		    \draw[dashed] (2.23,-1.6) -- (3.23,0.4);
%		    \draw[dashed] (11.85,-2) -- (13.05,0.4);
%		    \draw[dashed] (3.23,0.4) -- (13.05,0.4) node [midway,fill=white] {Shadow area};
%		    
%	  		\def\dy{0.1}
%		    \draw (1,-4) -- (3,-5);
%		    \draw (1+\dy,-4+2*\dy) -- (3+\dy,-5+2*\dy);
%		    \draw (1+2*\dy,-4+2*2*\dy) -- (3+2*\dy,-5+2*2*\dy);
%		    \draw[<-] (2.3,-3.9) -- (1.8,-4.9) node[below left]{$p_{\mathrm{inc}}$};
%	\end{tikzpicture}
%	\caption[Near field of BeTSSi model 3 with $f=500\unit{Hz}$ and $\alpha_{\mathrm{s}}=240^\circ$]{\textbf{Scattering on BeTSSi model 3}: The near field of BeTSSi model 3 with $f=500\unit{Hz}$ on mesh 5. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. Mesh 5 is illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:mesh5bistatic_f_500alpha240}
%	
%	
%	\vspace{2cm}
%	\tikzsetnextfilename{mesh5bistatic_f_500alpha300} 
%	\begin{tikzpicture}
%		\def\scalingFact{41.4}
%			\node[anchor=north west,inner sep=0] at (0,0) {\includegraphics[width=0.8425\textwidth]{../../graphics/mesh5bistatic_f_500alpha300}};
%		    
%	  		\def\dy{0.1}
%		    \draw (10,-5) -- (12,-4);
%		    \draw (10-\dy,-5+2*\dy) -- (12-\dy,-4+2*\dy);
%		    \draw (10-2*\dy,-5+2*2*\dy) -- (12-2*\dy,-4+2*2*\dy);
%		    \draw[<-] (10.6,-3.7) -- (11.1,-4.7) node[below right]{$p_{\mathrm{inc}}$};
%	\end{tikzpicture}
%	\caption[Near field of BeTSSi model 3 with $f=500\unit{Hz}$ and $\alpha_{\mathrm{s}}=300^\circ$]{\textbf{Scattering on BeTSSi model 3}: The near field of BeTSSi model 3 with $f=500\unit{Hz}$ on mesh 5. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. Mesh 5 is illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:mesh5bistatic_f_500alpha300}
%\end{figure} 
%\begin{figure}
%	\centering
%	\tikzsetnextfilename{mesh5bistatic_f_1000alpha240} 
%	\begin{tikzpicture}
%		\def\scalingFact{41.4}
%			\node[anchor=north west,inner sep=0] at (0,0) {\includegraphics[width=0.8425\textwidth]{../../graphics/mesh5bistatic_f_1000alpha240}};
%		    
%	  		\def\dy{0.1}
%		    \draw (1,-4) -- (3,-5);
%		    \draw (1+\dy,-4+2*\dy) -- (3+\dy,-5+2*\dy);
%		    \draw (1+2*\dy,-4+2*2*\dy) -- (3+2*\dy,-5+2*2*\dy);
%		    \draw[<-] (2.3,-3.9) -- (1.8,-4.9) node[below left]{$p_{\mathrm{inc}}$};
%	\end{tikzpicture}
%	\caption[Near field of BeTSSi model 3 with $f=1\unit{kHz}$ and $\alpha_{\mathrm{s}}=240^\circ$]{\textbf{Scattering on BeTSSi model 3}: The near field of BeTSSi model 3 with $f=1\unit{kHz}$ on mesh 5. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. Mesh 5 is illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:mesh5bistatic_f_1000alpha240}
%	
%	
%	\vspace{2cm}
%	\tikzsetnextfilename{mesh5bistatic_f_1000alpha300} 
%	\begin{tikzpicture}
%		\def\scalingFact{41.4}
%			\node[anchor=north west,inner sep=0] at (0,0) {\includegraphics[width=0.8425\textwidth]{../../graphics/mesh5bistatic_f_1000alpha300}};
%		    
%	  		\def\dy{0.1}
%		    \draw (10,-5) -- (12,-4);
%		    \draw (10-\dy,-5+2*\dy) -- (12-\dy,-4+2*\dy);
%		    \draw (10-2*\dy,-5+2*2*\dy) -- (12-2*\dy,-4+2*2*\dy);
%		    \draw[<-] (10.6,-3.7) -- (11.1,-4.7) node[below right]{$p_{\mathrm{inc}}$};
%	\end{tikzpicture}
%	\caption[Near field of BeTSSi model 3 with $f=1\unit{kHz}$ and $\alpha_{\mathrm{s}}=300^\circ$]{\textbf{Scattering on BeTSSi model 3}: The near field of BeTSSi model 3 with $f=1\unit{kHz}$ on mesh 5. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. Mesh 5 is illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:mesh5bistatic_f_1000alpha300}
%\end{figure} 
%
%
%\subsubsection{Bistatic scattering}
%Bistatic scattering consist of analyzing a single incident wave on the obstacle, and measure the scattered pressure in a series of far-field points. We shall consider bistatic scattering for incident waves with aspect angles $\alpha_{\mathrm{s}}=240^\circ$ and $\alpha_{\mathrm{s}}=300^\circ$, and for the frequencies $100\unit{Hz}$, $500\unit{Hz}$ and $1\unit{kHz}$. For all these 6 cases we compare with the results obtained by FOI.
%
%In \Cref{Fig2:M3_240_100} and \Cref{Fig2:M3_300_100} we consider the two cases for $f=100\unit{Hz}$. At such a low frequency, we observe very good results. Even mesh 1 yields a tolerable result. However, increasing the frequency to $500\unit{Hz}$ we see in \Cref{Fig2:M3_240_100} and \Cref{Fig2:M3_300_100} that a corresponding increase in the number of elements is needed. In the final increase of the frequency to $1\unit{kHz}$ the accuracy of the results fall correspondingly. This seems to be dominant in the area $\alpha_{\mathrm{f}}\in[120^\circ, 300^\circ]$. The angle $\alpha_{\mathrm{s}}$ lies in this interval, and as we shall see, the monostatic analysis on the same frequency reveals the same loss of accuracy for the full set of angles $\alpha_{\mathrm{s}}$. In other words, using the chosen set of parameters (mesh, polynomial order, etc.), considering the same aspect angle for the incident wave and the far-field point yields slower convergence. Note that mesh 5 is the most refined mesh available for a direct solver with the equipment at hand.
%
%\tikzsetnextfilename{M3_240_100} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{black}, % FOI
%			},
%			legend style={
%			at={(0.5,0.97)},
%			anchor=north
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%			ymax = 30,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh1_240.dat};
%			\addlegendentry{Mesh 1}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh2_240.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh3_240.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh4_240.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f100_240.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=240^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_240_100}
%	\vspace{2cm}
%\tikzsetnextfilename{M3_300_100} 
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{black},
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%			ymax = 30,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh1_300.dat};
%			\addlegendentry{Mesh 1}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh2_300.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh3_300.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_100_mesh4_300.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f100_300.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%		\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=300^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_300_100}
%\end{figure} 
%\tikzsetnextfilename{M3_240_500} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 5
%				{black},
%			},
%			legend style={
%			at={(0.5,0.97)},
%			anchor=north
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh1_240.dat};
%			\addlegendentry{Mesh 1}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh2_240.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh3_240.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh4_240.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh5_240.dat};
%			\addlegendentry{Mesh 5}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f500_240.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=500\unit{Hz}$ and $\alpha_{\mathrm{s}}=240^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=500\unit{Hz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_240_500}
%	\vspace{2cm}
%\tikzsetnextfilename{M3_300_500} 
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 5
%				{black},
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh1_300.dat};
%			\addlegendentry{Mesh 1}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh2_300.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh3_300.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh4_300.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_500_mesh5_300.dat};
%			\addlegendentry{Mesh 5}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f500_300.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=500\unit{Hz}$ and $\alpha_{\mathrm{s}}=300^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=500\unit{Hz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_300_500}
%\end{figure} 
%\tikzsetnextfilename{M3_240_1000} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 5
%				{black},
%			},
%			legend style={
%			at={(0.5,0.97)},
%			anchor=north
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%							
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh2_240.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh3_240.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh4_240.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh5_240.dat};
%			\addlegendentry{Mesh 5}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f1000_240.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=1\unit{kHz}$ and $\alpha_{\mathrm{s}}=240^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=1\unit{kHz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. Mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:M3_240_1000}
%\end{figure} 
%\tikzsetnextfilename{M3_300_1000} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{mycolor}, 
%				{myGreen}, 
%				{myCyan},
%				{myRed},
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{f}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh2_300.dat};
%			\addlegendentry{Mesh 2}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh3_300.dat};
%			\addlegendentry{Mesh 3}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh4_300.dat};
%			\addlegendentry{Mesh 4}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/f_1000_mesh5_300.dat};
%			\addlegendentry{Mesh 5}
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_BI/FOI_f1000_300.dat};
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=1\unit{kHz}$ and $\alpha_{\mathrm{s}}=300^\circ$]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=1\unit{kHz}$. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. Mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:M3_300_1000}
%\end{figure} 
%Finally, for illustration purposes, we plot the bistatic pressure also for a set of angles $\beta_{\mathrm{s}}$ which then results in a 3D plot. In \Cref{Fig2:M3_240_100_3D} we consider $\alpha_{\mathrm{s}}=240^\circ$ and add the geometry of BeTSSi model 3 as a location reference (this geometry is scaled up in order to make it visible). In \Cref{Fig2:M3_240_100_3Dfull} we plot the full set of elevation angles $\beta_{\mathrm{f}}$. The similar case for $\alpha_{\mathrm{s}}=300^\circ$ are depicted in \Cref{Fig2:M3_300_100_3D} and \Cref{Fig2:M3_300_100_3Dfull}.
%\begin{figure}
%	\centering
%	\includegraphics[scale=1.3]{../../graphics/BeTSSi_M3_HWBC_f100_240_20}	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=240^\circ$ 3D~plot]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$ on mesh 1. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. The plot spans elevation angles $\beta_{\mathrm{f}}$ from $-20^\circ$ to $20^\circ$ and the whole range of aspect angles in steps of $0.25^\circ$ (results in $232,001$ evaluation points). Mesh 1 is illustrated in \Cref{Fig2:Mesh1NonUniform}.}
%	\label{Fig2:M3_240_100_3D}
%	\vspace{2cm}
%	\includegraphics[scale=1.3]{../../graphics/BeTSSi_M3_HWBC_f100_240_90}	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=240^\circ$ 3D~plot]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$ on mesh 1. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=240^\circ$. The plot spans the whole range of elevation angles and of aspect angles in steps of $0.25^\circ$ (results in $1,038,961$ evaluation points). Mesh 1 is illustrated in \Cref{Fig2:Mesh1NonUniform}.}
%	\label{Fig2:M3_240_100_3Dfull}
%\end{figure} 
%\begin{figure}
%	\centering
%	\includegraphics[scale=1.3]{../../graphics/BeTSSi_M3_HWBC_f100_300_20}	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=300^\circ$ 3D~plot]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$ on mesh 1. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. The plot spans elevation angles $\beta_{\mathrm{f}}$ from $-20^\circ$ to $20^\circ$ and the whole range of aspect angles in steps of $0.25^\circ$ (results in $232,001$ evaluation points). Mesh 1 is illustrated in \Cref{Fig2:Mesh1NonUniform}.}
%	\label{Fig2:M3_300_100_3D}
%	\vspace{2cm}
%	\includegraphics[scale=1.3]{../../graphics/BeTSSi_M3_HWBC_f100_300_90}	
%	\caption[Bistatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$ and $\alpha_{\mathrm{s}}=300^\circ$ 3D~plot]{\textbf{Bistatic scattering on BeTSSi model 3}: The bistatic TS of BeTSSi model 3 with $f=100\unit{Hz}$ on mesh 1. The aspect angle for the incident wave is $\alpha_{\mathrm{s}}=300^\circ$. The plot spans the whole range of elevation angles and of aspect angles in steps of $0.25^\circ$ (results in $1,038,961$ evaluation points). Mesh 1 is illustrated in \Cref{Fig2:Mesh1NonUniform}.}
%	\label{Fig2:M3_300_100_3Dfull}
%\end{figure} 
%\clearpage
%
%\subsubsection{Monostatic scattering}
%In monostatic scattering we consider the case $\alpha_{\mathrm{f}}=\alpha_{\mathrm{s}}$ and $\beta_{\mathrm{f}}=\beta_{\mathrm{s}}$. Due to the geometry of BeTSSi model 3, one expects peaks at incident waves which hits the scatterer normal to the broadsides (as noted in~\cite{Nolte2014btb}). A simple trigonometric calculation then reveals these angles to be
%\begin{align*}
%	\alpha_{\mathrm{s},\mathrm{max}}^{(1)} &= \frac{\pi}{2}-\tan^{-1}\left(\frac{R_{\mathrm{o}1}-R_{\mathrm{o}2}}{L-R_{\mathrm{o}1}-R_{\mathrm{o}2}}\right) = 1.522054475 = 87.20729763^\circ,\\
%	\alpha_{\mathrm{s},\mathrm{max}}^{(2)} &= \frac{3\pi}{2}+\tan^{-1}\left(\frac{R_{\mathrm{o}1}-R_{\mathrm{o}2}}{L-R_{\mathrm{o}1}-R_{\mathrm{o}2}}\right) = 4.761130832 = 272.7927024^\circ,
%\end{align*}
%where $R_{\mathrm{o}1}=5$ and $R_{\mathrm{o}2}=3$ is the outer radius of the larger and smaller hemisphere, respectively, and $L=49$ is the total length of BeTSSi model 3 (including the hemispheres). Both of these predictions are verified in the results. 
%
%In \Cref{Fig2:M3_MS_100} we consider monostatic scattering with $f=100\unit{Hz}$. For such a low frequencies we obtain very good results, even for mesh 1. Increasing the frequency to $f=500\unit{Hz}$, we observe in \Cref{Fig2:M3_MS_500} that we need a corresponding increase in the number of elements to reach the same accuracy. Unfortunately we have no data sets from FOI to compare with for these two cases. Finally, increasing the frequency to $1\unit{kHz}$ we can compare the results to FOI (\Cref{Fig2:M3_MS_1000}), and we do not reach convergence on mesh 5. It is assumed that the resolution of the mesh is too low to obtain good results at this frequency. That is, our results suffers from the pollution effect.
%\tikzsetnextfilename{M3_MS_100} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 4
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{s}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_100_mesh1.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_100_mesh2.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_100_mesh3.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_100_mesh4.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_100_mesh5.dat};
%			
%			\addlegendentry{mesh 1}
%			\addlegendentry{mesh 2}
%			\addlegendentry{mesh 3}
%			\addlegendentry{mesh 4}
%			\addlegendentry{mesh 5}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Monostatic scattering on BeTSSi model 3 with $f=100\unit{Hz}$]{\textbf{Monostatic scattering on BeTSSi model 3}: The monostatic TS of BeTSSi model 3 with $f=100\unit{Hz}$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_MS_100}
%\end{figure} 
%\tikzsetnextfilename{M3_MS_500} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myYellow}, % 1
%				{mycolor}, % 2
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 5
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{s}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_500_mesh1.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_500_mesh2.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_500_mesh3.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_500_mesh4.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_500_mesh5.dat};
%			
%			\addlegendentry{mesh 1}
%			\addlegendentry{mesh 2}
%			\addlegendentry{mesh 3}
%			\addlegendentry{mesh 4}
%			\addlegendentry{mesh 5}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Monostatic scattering on BeTSSi model 3 with $f=500\unit{Hz}$]{\textbf{Monostatic scattering on BeTSSi model 3}: The monostatic TS of BeTSSi model 3 with $f=500\unit{Hz}$. Mesh 1 and mesh 2, 3, 4 and 5 are illustrated in \Cref{Fig2:Mesh1NonUniform} and \Cref{Fig2:model3Meshes}, respectively.}
%	\label{Fig2:M3_MS_500}
%\end{figure} 
%\tikzsetnextfilename{M3_MS_1000} 
%\begin{figure}
%	\centering
%	\begin{tikzpicture}
%		\begin{axis}[
%			width = 0.95\textwidth,
%			height = 0.3\paperheight,
%			cycle list={%
%				{myGreen}, % 3
%				{myCyan}, % 4
%				{myRed}, % 5
%				{black}, % FOI
%			},
%			legend style={
%			at={(0.97,0.97)},
%			anchor=north east
%			},
%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%			%yticklabels={},
%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%			%xmin=80, 
%			%xmax=100000, 
%%				ymin = -24,
%%				ymax = 25,
%			ylabel={TS},
%			xlabel={Aspect angle $\alpha_{\mathrm{s}}$}
%			]
%			
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_1000_mesh3.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_1000_mesh4.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/f_1000_mesh5.dat};
%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_HWBC_MS/FOI4.dat};
%			
%			\addlegendentry{Mesh 3}
%			\addlegendentry{Mesh 4}
%			\addlegendentry{Mesh 5}
%			\addlegendentry{FOI4}
%		\end{axis}
%	\end{tikzpicture} 	
%	\caption[Monostatic scattering on BeTSSi model 3 with $f=1\unit{kHz}$]{\textbf{Monostatic scattering on BeTSSi model 3}: The monostatic TS of BeTSSi model 3 with $f=1\unit{kHz}$. Mesh 3, 4 and 5 are illustrated in \Cref{Fig2:model3Meshes}.}
%	\label{Fig2:M3_MS_1000}
%\end{figure} 
%
%
%\subsection{General remarks}
%In~\cite{Burnett1994atd} Burnett suggest that the artificial boundary $\Gamma_{\mathrm{a}}$ should be placed (on average) $\frac{\lambda}{2}$ away from the object. That is, he suggest that this boundary to be placed closer at higher frequencies. This rule would be hard to impose on BeTSSi model 3 simply because BeTSSi model 3 differs to much from a prolate spheroid. This is a drawback, as it could be easy to draw a convex surface around BeTSSi model 3 which would nearly be a constant distance from the object surface $\Gamma$. The promising method of PML (Perfectly matched layers) after Bérenger (in~\cite{Berenger1994apm} and~\cite{Berenger1996pml}) manages to do just that, create a perfectly matched layer of fluid between $\Gamma_{\mathrm{a}}$ and $\Gamma$. In principle, this should be possible for the infinite element method (as long as $\Gamma_{\mathrm{a}}$ is made convex). However, this requires the use of a more general coordinate system (rather then the prolate spheroidal coordinate system). This topic has been somewhat investigated in \Cref{subsubsubsec:infElementsOnGeneralizedCoordSyst}.
%
%As we did not achieve completely satisfactory accuracy in the numerical simulation of the BeTSSi model 3 using HWBC, we did not make anyattempt to do the full FSI problem of this model. This problem consist of BeTSSi model 3 being filled with water, such that we have a interaction between fluid and the solid both inside and outside the shell. We must thus not only add structural elements, but also fluid elements inside the shell. The number of elements for mesh 5 (M3) then easily rises above one million, and will thus be outside the capacity of our direct solver.
%
%%In \Cref{Fig2:M3_RBC_TS} various results from different companies illustrate the additional complexity of introducing FSI. This plot illustrates that the shadow area is reduced. In fact, the waves penetrates the model so well as to create a second peak around $90^\circ$ (and correspondingly around $270^\circ$).
%%\tikzsetnextfilename{M3_RBC_TS} 
%%\begin{figure}
%%	\centering
%%	\begin{tikzpicture}
%%		\begin{axis}[
%%			width = 0.95\textwidth,
%%			height = 0.3\paperheight,
%%			cycle list={%
%%				{BeTSSiII_2}, % BHT
%%				{BeTSSiII_11}, % DCNS
%%				{BeTSSiII_3}, % DRDC&LR
%%				{BeTSSiII_4}, % DSTO
%%				{BeTSSiII_5}, % FOI1
%%				{BeTSSiII_5, dashed},  % FOI2
%%				{BeTSSiII_6}, % FWG
%%				{BeTSSiII_7}, % Kockums
%%				{BeTSSiII_9}, % TKMS
%%				{BeTSSiII_13}, % TNO
%%			},
%%			legend style={
%%			at={(0.97,0.97)},
%%			anchor=north east
%%			},
%%			%xtick={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14},
%%%			ytick={0, 0.02, 0.04, 0.06, 0.08, 0.1},
%%			%yticklabels={},
%%			%xticklabels={2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 13'},
%%			%xmin=80, 
%%			%xmax=100000, 
%%%				ymin = -24,
%%			%ymax = 60,
%%			ylabel={TS},
%%			xlabel={Aspect angle}
%%			]
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/BHT.dat};
%%			\addlegendentry{BHT}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/DCNS.dat};
%%			\addlegendentry{DCNS}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/DRDCLR.dat};
%%			\addlegendentry{DRDC\&LR}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/DSTO.dat};
%%			\addlegendentry{DSTO}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/FOI1.dat};
%%			\addlegendentry{FOI1}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/FOI2.dat};
%%			\addlegendentry{FOI2}
%%							
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/FWG.dat};
%%			\addlegendentry{FWG}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/Kockums.dat};
%%			\addlegendentry{Kockums}
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/TKMS.dat};
%%			\addlegendentry{TKMS}
%%			
%%			
%%			\addplot table[x=theta,y=TS] {../../matlab/plotData/BeTSSi_M3_RBC_MS_0_1/TNO.dat};
%%			\addlegendentry{TNO}
%%			
%%		\end{axis}
%%	\end{tikzpicture} 
%%	
%%	\caption[Monostatic scattering on BeTSSi model 3 with RBC]{\textbf{Monostatic scattering on BeTSSi model 3 with RBC}: Plot of the TS of the model 3 with RBC (Realistic Boundary Conditions) and frequency $f=1\unit{kHz}$. A description of each company was given in \Cref{se:background}.}
%%	\label{Fig2:M3_RBC_TS}
%%\end{figure} 
%
%The simulation using mesh 5 with HWBC has been using a server with 256GB available memory. With $700,000$ elements (mesh 5), about 50\% of this memory is used. The memory consumption is very expensive as the system of linear equation is solved by a direct solver. In MATLAB, a LU-factorization is made, and this is very memory consuming. An iterative iterative solver should be implemented to solve the issue. Not only will the memory consumption problem be eliminated, but we should also be able to speed up the solution process, as we do not require machine epsilon precision of the solution (after all, a 1\% error in the result is considered to be very good). For classical elasticity problems on bounded domain, the global matrix is symmetric and positive definite (SPD). However, when introducing the infinite elements, the mass matrix is no longer positive definite, and neither is the resulting global matrix. This is the reason we may not use Cholesky factorization as a direct method. Moreover, this is the reason we we may not use the conjugate gradient (CG) method as this method also requires the matrix to be SPD. We must therefore go to other more general iteration techniques which typically have slower convergence rates. MATLAB has a built in routine for the GMRES method, which is designed for large sparse systems. Although CG cannot be used, there exist CG similar methods which does not require the matrix to be positive definite. Some of these methods are compared in~\cite{Clemens2002imf}, BiCGStab is also a natural choice to be investigated. The global matrix often turns out to be badly conditioned for iterative techniques. One should apply some preconditioning to this matrix before applying for instance GMRES. This typically results in a comprehensive analysis, which we shall suggest as future work.
%


==> contents/sourceCode.tex <==
\section{Source code}
The complete source code is far to comprehensive to be included in this thesis. However, we shall present the implementation of the NURBS routine in some detail as this is a fundamental function of the analysis. In addition we add the routine which create global matrices. We shall here not go into details. The source code, alongside instruction of how to use, may be given on request.

\subsection{B-spline implementation}
When we want to evaluate a B-spline at a fixed $\xi$ it is important to note that it is very redundant to evaluate all $n$ basis function. This is due to the small support of each function. In fact, it turns out that only (at most) $p+1$ basis functions are non-zero at $\xi$. It is then important to only use these function to have an efficient code. One typically implements a function which finds the knot span corresponding to a given $\xi$. Due to the ordering of the knot vector, we may use a binary search algorithm for finding this span. The span will be defined by the index $i$ corresponding to the last basis function which is non-zero at $\xi$. The following listing represents the algorithm called \mcode{findKnotSpan} and is listed in \Cref{Listings:findKnotSpan}.

As an example, if $p=2$ and $n=8$ and we want to evaluate a B-spline with the knot vector $\Xi = \{0, 0, 0, 0.1, 0.5, 0.5, 0.8, 0.9, 1, 1, 1\}$, we get the index $i=3$ if $\xi = 0.09$, $i=6$ if $\xi=0.5$ and $i=n=8$ if $\xi=0.9$ or $\xi = 1$.

We are now ready to implement a program which evaluates B-splines using the previous routine. When the recursion formula is used to evaluate the $p+1$ functions which are non-zero at $\xi$, the function $N_{i,0}$ is the only function of order zero which is non-zero at $\xi$. Everything is thus build from this function, such that we get the graph in \Cref{Fig2:BsplinesEvalGraph}.
\tikzsetnextfilename{BsplinesEvalGraph}  
\begin{figure}
	\centering
	\ifplotData
	\begin{tikzpicture}[>=triangle 60]
	  \matrix[matrix of math nodes,column sep={70pt,between origins},row
	    sep={40pt,between origins},nodes={asymmetrical rectangle}] (s)
	  {
	    	 |[name=aa]| N_{i,0} 		& |[name=ba]| N_{i-1,1} & |[name=ca]| N_{i-2,2} &  |[name=da]| \cdots 	&  |[name=ea]| \textcolor{myRed}{N_{i-p+1,p-1}} 	&  |[name=fa]| N_{i-p,p}  	\\	
	    	 					 		& |[name=bb]| N_{i,1}   & |[name=cb]| N_{i-1,2} &  |[name=db]| \cdots 	&  |[name=eb]| \textcolor{myRed}{N_{i-p+2,p-1}} 	&  |[name=fb]| N_{i-p+1,p}  \\	
	    	 					 		& 			 		    & |[name=cc]| N_{i,2}   &  |[name=dc]| \cdots 	&  |[name=ec]| \textcolor{myRed}{N_{i-p+3,p-1}} 	&  |[name=fc]| N_{i-p+2,p}  \\	
	    	 					 		& 			 		    & 					  	&  |[name=dd]| \ddots 	&  |[name=ed]| \vdots 							&  |[name=fd]|\vdots  \\	
	    	 					 		& 						& 						&  				 		&  |[name=ee]| \textcolor{myRed}{N_{i,p-1}} 		&  |[name=fe]| N_{i-1,p}  	\\	
	    	 							& 						& 						&  					  	&  									 			&  |[name=ff]| N_{i,p}  	\\	
	  };
	  \draw[->] (aa) edge (ba)
	  			(ba) edge (ca)
	  			(ca) edge (da)
	  			(da) edge (ea)
	  			(ea) edge (fa)
	  			
	  			(bb) edge (cb)
	  			(cb) edge (db)
	  			(db) edge (eb)
	  			(eb) edge (fb)
	  			
	  			(cc) edge (dc)
	  			(dc) edge (ec)
	  			(ec) edge (fc)
	  			
	  			(ee) edge (fe)
	  			
	  			(aa) edge (bb)
	  			(bb) edge (cc)
	  			(cc) edge (dd)
	  			(dd) edge (ee)
	  			(ee) edge (ff)
	  			
	  			(ba) edge (cb)
	  			(cb) edge (dc)
	  			
	  			(ca) edge (db)
	  			(db) edge (ec)
	  			
	  			(da) edge (eb)
	  			(eb) edge (fb)
	  			
	  			(ea) edge (fb);
	\end{tikzpicture}
	\fi
	\caption[B-splines evaluation graph]{B-splines evaluation graph when the $p+1$ non-zero basis functions are to be evaluated at a given $\xi$. The values colored \textcolor{myRed}{red} is used to calculate the nonzero derivatives at the same $\xi$.}
	\label{Fig2:BsplinesEvalGraph}
\end{figure}

It is then clear that we need two loops. The outer loop should iterate over the columns of this graph and the inner loop should iterate over the rows. The output of the function \mcode{Bspline_basis} is simply an array \mcode{N} which contains the $p+1$ functions which are evaluated at $\xi$. To save memory one should also store the intermediate values $N_{i-j+k, j-1}$ in this same array. Thus, we need to store \mcode{N(k-1)} to compute \mcode{N(k)} (which we store in the variable \mcode{saved}). Here, $j$ is the loop index of the outer loop, while $k$ is the loop index of the inner loop. The first iteration (when $p=0$) should be done separate.

We will finally need to compute the corresponding derivatives. Once again, only $p+1$ derivatives will be nonzero at $\xi$. Let \mcode{N_tilde} be an array containing the \textcolor{myRed}{red} values in the previous graph. The full function is found in \Cref{Listings:Bspline_basisDers}.

\subsection{NURBS implementation}
We may now insert all of this into a routine which computes the nonzero NURBS basis functions at a given point $(\xi,\eta,\zeta)$ and the corresponding nonzero derivatives. This function is called \mcode{NURBS3DBasisDers}. After finding the nonzero B-spline functions and their corresponding derivatives as discussed above, it continues by first finding the function $W$ and its corresponding derivatives. 

Note the use of the index \mcode{A} which is convenient when weights is located in an long array (which is the format we shall use when doing the IGA analysis). Finally, the function can now compute the NURBS basis alongside the corresponding derivatives.

Note the use of the intermediate variables \mcode{fac} and \mcode{NML} which is used to avoid redundant computations. The index \mcode{counter} loops over the $n_{\mathrm{en}}=(p+1)\cdot(q+1)\cdot(r+1)$ nonzero functions. The full function is found in \Cref{Listings:NURBS3DBasis}.

\subsection{Building global matrices}
The function \mcode{buildGlobalMatrices} builds any fluid or solid matrix used in this thesis. When dynamics is considered, the mass matrix will also be computed. Finally, if any bodyforces are applied, a corresponding loading vector will be constructed. As an example of use, consider any analysis concerning finding eigenvalues for elasticity problems. Then we use the function as follows.
\begin{lstlisting}
options = {'operator', 'linearElasticity',...
           'fieldDimension', 3,...
           'buildMassMatrix', 1};
[K, M, ~] = buildGlobalMatrices(varCol, options);
\end{lstlisting}
The partial differential equation resulting in the global matrix is the linear elasticity equation. Hence, we set \mcode{'operator'} to be \mcode{'linearElasticity'}. If the Helmholtz equation was to be solved, the \mcode{'operator'} is set to be \mcode{'Laplace'}. The option \mcode{'fieldDimension'} is only added for generality if other operators where to be implemented. Indeed, the solution for the linear elasticity operator is always vector valued (in 2D/3D), while the solution for the Laplace operator is scalar valued. Finally, we ask the function to build the mass matrix, as eigenvalues concerns with dynamics. The struct \mcode{varCol} simply collects all variables associated with the NURBS mesh. The full function is listed in \Cref{Listings:buildGlobal}
\raggedbottom
\lstinputlisting[caption = {\mcode{findKnotSpan.m}}, label = {Listings:findKnotSpan}]{../../data/NURBS/findKnotSpan.m}
\newpage
\lstinputlisting[caption = {\mcode{Bspline_basisDers.m}}, label = {Listings:Bspline_basisDers}]{../../data/NURBS/Bspline_basisDers.m}
\lstinputlisting[caption = {\mcode{NURBS3DBasis.m}}, label = {Listings:NURBS3DBasis}]{../../data/NURBS/NURBS3DBasis.m}
\lstinputlisting[caption = {\mcode{buildGlobalMatrices.m}}, label = {Listings:buildGlobal}]{../../data/IGAfunctions/buildGlobalMatrices.m}

==> contents/test2.tex <==
\tikzsetnextfilename{physicalProblem}
\begin{figure}
	\centering
	\begin{tikzpicture}[scale = 1,font=\small]
	\draw [water, fill = water] (2,0) ellipse (4cm and 2cm);
	%\draw [gray!50]  (0,0) -- (1,1) -- (2,1) -- (3,0)  -- (2,-1) -- cycle;
	\draw [myRed, fill = solid] plot [smooth cycle] coordinates {(0,0) (1,0.5) (1.2,1) (2,1) (3,0) (2,-1)};
	\draw [<-, below right] (2,-0.5) -- (2.9,-2.2) node{Elastic material};
	\draw [<-, below] (0,-1) -- (-1,-2.2) node{Homogeneous fluid};
	\draw [below right] (3,0) node{$\color{myRed} \Gamma$};
	\draw [water, fill = water] (-2.6, 0) circle(0.05cm);
	\draw [water, fill = water] (-2.4, 0) circle(0.05cm);
	\draw [water, fill = water] (-2.2, 0) circle(0.05cm);
	\draw [water, fill = water] (6.6, 0) circle(0.05cm);
	\draw [water, fill = water] (6.4, 0) circle(0.05cm);
	\draw [water, fill = water] (6.2, 0) circle(0.05cm);
	\draw [water, fill = water] (2, 2.2) circle(0.05cm);
	\draw [water, fill = water] (2, 2.4) circle(0.05cm);
	\draw [water, fill = water] (2, 2.6) circle(0.05cm);
	\draw [water, fill = water] (2, -2.2) circle(0.05cm);
	\draw [water, fill = water] (2, -2.4) circle(0.05cm);
	\draw [water, fill = water] (2, -2.6) circle(0.05cm);
	\def\dx{1};
	\def\dy{1};
	\def\x{-2};
	\def\y{2};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\def\x{-1.8};
	\def\y{1.8};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\def\x{-1.6};
	\def\y{1.6};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\draw [<-, above left] (-1.4+\dx/2, 1.4+\dy/2) -- (-2.2+\dx/2, 2.2+\dy/2) node{$\color{black}p_{\text{inc}}$};
	\def\dx{1};
	\def\dy{-0.5};
	\def\x{4};
	\def\y{3};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\def\x{4.1};
	\def\y{3.2};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\def\x{4.2};
	\def\y{3.4};
	\draw (\x,\y) -- (\x+\dx,\y+\dy);
	\draw [<-, below] (4.3+\dx/2, 3.6+\dy/2) -- (3.9+\dx/2, 2.8+\dy/2) node{$\color{black}p_{\mathrm{s}}$};
	
	\draw (2, 0) node{$\color{black}\Omega$};
	\draw (3, 1) node{$\color{black}\Omega^+$};
	
	%\draw [gray!50, xshift=4cm]  (0,0) -- (1,1) -- (2,-2) -- (3,0);
	%\draw [cyan, xshift=4cm] plot [smooth, tension=2] coordinates { (0,0) (1,1) (2,-2) (3,0)};
	\end{tikzpicture}
	\caption[Illustration of the physical problem]{Illustration of the physical problem.}
	\label{Fig2:physicalProblem}
\end{figure}

==> contents/vibrations.tex <==
\section{Isogeometric analysis of vibrations}
\label{Sec2:vibrations}
A fundamental mathematical assumption of this thesis, is the harmonic time dependency assumption (see \Cref{Eq2:periodicityAssumption}). When we transform our time dependent problem to a frequency dependent problem, it is advantageous to analyze the phenomena of vibrations (also named \textit{spectrum analysis}). As it turns out, there are examples where IGA is demonstrably better in this analysis compared to ordinary FEA. That is, one may wonder if the NURBS basis functions (with their smooth properties) serve a better basis than the typical Lagrange basis function which are commonly used in FEM. We shall illustrate this improvement by an example taken from~\cite{Cottrell2009iat}. The work in~\cite{hughes2009imi} and~\cite{Cottrell2006iao} investigates the improvement of IGA even further.

\subsection{Longitudinal vibrations of an elastic rod}
\label{subse:longVibElRod}
We shall consider an one dimensional rod of length $L$ such that our spatial domain is given by $\Omega = (0, L)$, where we apply homogeneous Dirichlet boundary conditions. That is, $u=0$ at $\Gamma = \partial\Omega = \{0, L\}$. In one dimension \Cref{Eq2:mainDiffEqn} reads
\begin{equation}\label{Eq2:elastic1Drod}
	E\pderiv[2]{u}{x} + \omega^2 \rho u = 0
\end{equation}
where it is assumed that $E$ and $\rho$ are constant throughout the domain. Proceeding in the usual way, we construct a solution space $\mathcal{S}=\{u|u\in H^1(\Omega), u|_\Gamma = 0\}$. As we have homogeneous Dirichlet boundary conditions, the weighted space $\mathcal{V}$ is identical to the solution space $\mathcal{S}$. We now multiply \Cref{Eq2:elastic1Drod} by an arbitrary $v\in \mathcal{V}$ and integrate the resulting equation over the domain.
\begin{equation*}
	\int_0^L  vE\pderiv[2]{u}{x} \idiff x + \omega^2\int_0^L v\rho u \idiff x = 0
\end{equation*}
Using partial integration we get
\begin{equation*}
	\left[vE\pderiv{u}{x} \right]_0^L - \int_0^L \pderiv{v}{x}E \pderiv{u}{x} \idiff x+ \omega^2\int_0^L v \rho u  \idiff x = 0
\end{equation*}
Exploiting now the fact that $v(0) = v(L) = 0$, the resulting weak form is given by
\begin{equation*}
	a(v,u) -\omega^2 (v,\rho u) = 0
\end{equation*}
where
\begin{align*}
	a(v,u) &= \int_0^L  \pderiv{v}{x} E\pderiv{u}{x} \idiff x\\
	( v,\rho u) &= \omega^2\int_0^L  v\rho u \idiff x
\end{align*}
Turning now to the Galerkin formulation, we restrict ourselves to solution of the form
\begin{equation*}
	u^h = \sum_{A = 1}^{n_{\mathrm{eq}}} N_A d_A\quad\text{and}\quad u^h = \sum_{B = 1}^{n_{\mathrm{eq}}} N_B d_B
\end{equation*}
such that our eigenvalue problem now becomes: Find $\omega^h\in\R^+$ and $u^h\in\mathcal{S}^h$ such that for all $v^h\in\mathcal{V}^h$ we have
\begin{equation*}
	a(v^h,u^h) -(\omega^h)^2 (u^h,\rho v^h) = 0
\end{equation*}
In the analysis we use a nonlinear parametrization of the rod such that the control points are uniformly placed in the physical space. As noted in~\cite{Cottrell2009iat}, this result in better results when studying structural vibrations. 

Using a finite number of NURBS basis functions\footnote{As all the weights are 1, we actually only get simple B-splines; a subset of NURBS functions.} ($n_{\mathrm{eq}}$), we will get the same number of eigenvalues $\omega_n^h$.

\pgfplotsset{
	legend style={
		at={(0.03,0.97)},
		anchor=north west,
		legend columns=1,
		%cells={anchor=west},
		font=\footnotesize,
		rounded corners=2pt
	}
}
\tikzsetnextfilename{longVibRodFEMIGAcomparison}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			xtick={0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1},
			xticklabels={0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1},
			%ytick={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
			%yticklabels={0.001,0.01, 0.1, 1.0, 10.0, 100.0},
			cycle list={%
				{myYellow}, 
				{mycolor}, 
				{mycolor, dashed}, 
				{myGreen}, 
				{myGreen,dashed}, 
				{myCyan},
				{myCyan,dashed},
				{myRed},
				{myRed,dashed}
			},
			width = 0.8\textwidth,
			height = 0.3\paperheight,
			%xticklabels={0.2, 0.15, 0.1, 0.05, 0},
			%xmin=80, 
			% ymin=0.0007,
			% xmax=200000, 
			xlabel=$n/n_{\mathrm{eq}}$,
			ylabel=$\omega_n^h/\omega_n$]
			
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodIGA/p1.dat};
			\addlegendentry{$p = 1$}
			
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodIGA/p2.dat};
			\addlegendentry{IGA: $p = 2$}
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodFEM/p2.dat};
			\addlegendentry{FEM: $p = 2$}
			
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodIGA/p3.dat};
			\addlegendentry{IGA: $p = 3$}
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodFEM/p3.dat};
			\addlegendentry{FEM: $p = 3$}
			
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodIGA/p4.dat};
			\addlegendentry{IGA: $p = 4$}
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodFEM/p4.dat};
			\addlegendentry{FEM: $p = 4$}
			
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodIGA/p5.dat};
			\addlegendentry{IGA: $p = 5$}
			\addplot table[x=n,y=omega,mark=none] {../../data/plotData/vibrationRodFEM/p5.dat};
			\addlegendentry{FEM: $p = 5$}
		\end{axis}
	\end{tikzpicture}
	\caption[IGA/FEM comparison of longitudinal vibrations of an elastic rod]{\textbf{Longitudinal vibrations of an elastic rod:} Comparison of FEM and IGA. Note that the basis functions for both FEM and IGA are equal in the case $p=1$. The results are thus identical in this case.}\label{Fig2:longVibRodFEMIGAcomparison}
\end{figure}

The solution of the \textit{eigenvalue problem} in \Cref{Eq2:elastic1Drod} is trigonometric equations. With the boundary conditions we get the eigenfunctions $u_n(x) = \sin \left(\sqrt{\frac{\rho}{E}}\omega_n x\right)$ and eigenvalues $\omega_n = \sqrt{\frac{E}{\rho}}\frac{n\pi}{L}$. We consider the case $L=1$, $\rho=1$, $E=1$ and $n_{\mathrm{eq}} = 999$. Then the eigenvalues are simply $\omega_n = n\pi$. We want to compare these analytic eigenvalues to our numerical eigenvalues $\omega_n^h$, by looking at the ratio $\omega_n/\omega_n^h$, which should tend to 1 as the numerical solution becomes better. In \Cref{Fig2:longVibRodFEMIGAcomparison} we plot this ratio against the ratio $n/n_{\mathrm{eq}}$ using standard Lagrange basis functions (FEM) and B-splines (IGA). A motivation for using IGA in stead of FEM in this thesis is quite apparent in this plot. It should be noted that the B-spline basis functions have larger support and the resulting matrix would then be less sparse. This will in turn increase the computational time for finding the eigenvalues. So the smooth results of IGA comes at some cost in computational time of solving the resulting system of equations. For a more detailed explanation of the different behaviors in \Cref{Fig2:longVibRodFEMIGAcomparison}, we refer to Cotterell et al.~\cite{Cottrell2009iat}. 


\subsection{Elastic vibration in 3D}
Moving on to three dimensions, we multiply each of the equations in \eqref{Eq:mainDiffEqn2} by a corresponding test functions $v_i\in\mathcal{S}_i$ and sum these three equations into one single equation given by
\begin{equation*}
	v_i\sigma_{ij,j} +\omega^2\rho_{\mathrm{s}} v_i u_i = 0.
\end{equation*}
Note that we have set $f_i=0$ as we shall not consider any body forces. 

Integration over the domain and using the same procedure as for the static linear elasticity case, get the linear form
\begin{equation*}
	L(\vec{v}) = \int_{\Gamma_N} v_i h_j\idiff\Gamma.
\end{equation*}
and the bilinear form
\begin{equation*}
	a(\vec{v},\vec{u}) = \int_\Omega v_{(i,j)}c_{ijkl}u_{(k,l)}\idiff\Omega - \omega^2\rho_{\mathrm{s}} \int_\Omega v_i u_i\idiff\Omega
\end{equation*}
where the only difference from before is the last term which will result in the \textit{mass matrix} $\vec{M}$. So if $\vec{K}$ is the same stiffness matrix as in the static linear elasticity case, we now have the following eigenvalue problem: Find natural frequency $\omega_k^h\in\R^+$ and eigenvectors $\vec{U}_k$ such that
\begin{equation*}
	(\vec{K}-[\omega_k^h]^2\vec{M})\vec{U}_k=\zerovec
\end{equation*}
where (using the same notation as before) the mass matrix is given by
\begin{equation*}
	\vec{M} = \left[M_{PQ}\right]
\end{equation*}
and
\begin{equation*}
	M_{PQ} = \rho_{\mathrm{s}} \vec{e}_i\int_\Omega R_A R_B\idiff\Omega\vec{e}_j.
\end{equation*}
As $\vec{e}_i\cdot \vec{e}_j = \delta_{ij}$ we may write
\begin{equation*}
	M_{PQ} = \rho_{\mathrm{s}} \delta_{ij}\int_\Omega R_A R_B\idiff\Omega.
\end{equation*}
In the same way the stiffness element matrix could be computed in one go, so can the \textit{element mass matrix}:
\begin{equation*}
	\vec{m}^e = \rho_{\mathrm{s}} \int_{\tilde{\Omega}^e}\mathrm{blkdiag}\left(\vec{R}^\transpose\vec{R},\vec{R}^\transpose\vec{R},\vec{R}^\transpose\vec{R}\right)|J_1||J_2| \idiff\tilde{\Omega}.
\end{equation*}
where (once again)
\begin{equation*}
	\vec{R}^\transpose = \begin{bmatrix}
		R_1, & R_2, & \dots, & R_{n_{\mathrm{en}}}
	\end{bmatrix}
\end{equation*}
and $\mathrm{blkdiag}()$ creates a block diagonal matrix with it's arguments on the diagonal.

\subsubsection{Circular plate vibrating in vacuum}
\begin{table}
	\centering
	\caption[Parameters for circular plate]{Parameters for circular plate.}
	\label{Tab2:circularPlateParameters}
	\begin{tabular}{l l}
		\toprule
		Parameter & Description\\
		\midrule
		$E = 30\cdot 10^9\unit{Pa}$ & Young's modulus\\
		$\rho = 2.32\cdot 10^3\unit{kg/m^3}$ & Density\\
		$\nu = 0.2$ & Poisson's ratio\\
		$t = 0.02\unit{m}$ & Thickness of the plate\\
		$R = 2\unit{m}$ & Radius of plate\\
		\bottomrule
	\end{tabular}
\end{table}
In~\cite[pp. 185-189]{Meirovitch1967ami} we find the exact Poisson-Kirchhoff solution to the clamped circular plate. One finds the eigenvalues by first solving
\begin{equation*}
	\imag^{-n}J_n(\imag x) J_{n-1}(\imag x) - \imag^{-n-1}J_n(x) J_{n-1}(\imag x) = 0,\quad n = 0,1,2,\dots
\end{equation*}
where $J_n$ are the mentioned Bessel functions of the first kind. This equation has infinitely many solution (as for the spherical shell), so we obtain a set of solutions $\{x_{nm}\}$. The eigenvalues are then given by $\beta_{nm} = x_{nm}/R$ such that the natural frequencies may be found by
\begin{equation}
	\omega_{nm} = \beta_{nm}^2\sqrt{\frac{D_E}{\rho t}},\quad D_E = \frac{E t^3}{12(1-\nu^2)}.
\end{equation}
In~\cite{Hughes2005iac} the notation $C_{nm} = x_{nm}/\pi$ has been used. In~\cite[p. 188]{Meirovitch1967ami} there is a misprint in the first eigenfrequency: $C_{01} = 1.015$ where the true value is $C_{01} = 1.0173886$. Hughes et al. copies this misprint in~\cite{Hughes2005iac} such that he compares his result with $\omega_{01} = 53.863$ when the true value is $\omega_{01} = 54.117$. Hence, in~\cite{Hughes2005iac} there seems to be convergence to the wrong result when this is not the case.
\begin{table}
	\centering
	\caption[Eigenvalues for circular plate]{\textbf{Circular plate:} Eigenvalues.}
	\label{Tab2:circularPlateFirstEigenValues}
	\pgfplotstableset{% global config, for example in the preamble
	% these columns/<colname>/.style={<options>} things define a style
	% which applies to <colname> only.
	columns/n/.style={int detect,column type=r,column name=\textsc{$n$}}, 
	columns/omega_n_0/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n1}$}},
	columns/omega_n_1/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n2}$}},
	columns/omega_n_2/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n3}$}},
	columns/omega_n_3/.style={/pgf/number format/fixed, sci sep align, column name=\textsc{$\omega_{n4}$}},
	every head row/.style={before row=\toprule,after row=\midrule},
	every last row/.style={after row=\bottomrule}
	}
	\pgfplotstabletypeset[fixed zerofill,precision=6, 1000 sep={\,},1000 sep in fractionals]{../../data/plotData/circularPlate/sortedEigenvalues.dat}
\end{table}
The NURBS data for the coarsest geometry of the plate shell may be found in \Cref{se:circularPlateNURBSdata}, here two parametrizations for the circular plate is presented (cf. \Cref{Fig2:circularPlate1_new} and \Cref{Fig2:circularPlate2_new}). In~\cite{Schmidt2010roa} better convergence results was shown for parametrization 2, but we shall restrict ourselves to the analysis on the first of these parametrizations as the main objective is to compare with the results in~~\cite{Cottrell2009iat}. Some deviation in the comparison of the results occured, but the main trend is the same.

In \Cref{Tab2:circlarPlateComputedEigenfrequencies} we show the $p$-convergence of the first 4 computed frequencies. The corresponding modes are shown in \Cref{Fig2:EigenModesCircularPlate}. We can here observe that for axisymmetric modes ($\omega_{0n}$, $n=0,1,2,\dots$) there is hardly any accuracy to be gained by increasing the polynomial order in the angular direction ($\xi$-direction).
\begin{table}
	\centering
	\caption[Convergence of computed eigenfrequencies for circular plate]{\textbf{Circular plate:} Convergence of computed eigenfrequencies.}
	\label{Tab2:circlarPlateComputedEigenfrequencies}
	\begin{tabular}{S S S S S S S}
		\toprule
		    {$p$} & {$q$} & {$r$} & {$\omega_{01}$} & {$\omega_{11}$} & {$\omega_{21}$} & {$\omega_{02}$}\\
		\midrule
						2 & 2 & 2 & 254.838 & 778.860 & 2569.078 & 3456.036\\	
						2 & 3 & 2 & 54.424 & 138.174 & 400.934 & 214.661\\	
						3 & 3 & 2 & 54.424 & 117.358 & 196.698 & 214.661\\	
						3 & 4 & 2 & 54.253 & 116.359 & 187.731 & 211.796\\	
						4 & 4 & 2 & 54.253 & 112.954 & 185.972 & 211.796\\	
						4 & 5 & 2 & 54.203 & 112.801 & 185.475 & 210.912\\	
						5 & 5 & 2 & 54.203 & 112.783 & 185.218 & 210.912\\	
						5 & 6 & 2 & 54.177 & 112.728 & 185.122 & 210.803\\	
		\multicolumn{3}{c}{exact} & 54.117 & 112.624 & 184.756 & 210.682\\	
	   %\multicolumn{3}{c}{exact} & 53.863 & 112.670 & {\textcolor{red}{??}} & 210.597\\	
		\bottomrule
	\end{tabular}
\end{table}
\begin{figure}
	\centering    
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.8\textwidth]{../../graphics/circularPlate_2}
		\caption{Parametrization 1.}
		\label{Fig2:circularPlate1_new}
	\end{subfigure}
	~ 
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.8\textwidth]{../../graphics/circularPlate2_2}
		\caption{Parametrization 2.}
		\label{Fig2:circularPlate2_new}
	\end{subfigure}
	\caption[Parametrizations of circular plate]{\textbf{Circular plate}: Example of parametrizations of the circular plate.}
\end{figure}

\begin{figure}
	\centering        
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrationCircularPlateMode1}
		\caption{Mode 1.}
	\end{subfigure}
	~
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrationCircularPlateMode2}
		\caption{Mode 2.}
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrationCircularPlateMode4}
		\caption{Mode 4.}
	\end{subfigure}
	~ 
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrationCircularPlateMode6}
		\caption{Mode 6.}
	\end{subfigure}
	\caption[Cibration modes of circular plate]{\textbf{Circular plate}: Four vibration modes using $p=6$, $q = 6$ and $r = 2$ with parametrization 1.}
	\label{Fig2:EigenModesCircularPlate}
\end{figure}

\subsubsection{Spherical shell vibrating in vacuum}
We shall repeat the analysis we did on the circular plate with the spherical shell with data from \Cref{Tab2:sphericalShellParameters}. The NURBS data for the coarsest geometry of the spherical shell may be found in \Cref{se:sphericalShellNURBSData}. In this analysis we shall insert the knots $\{\frac{1}{8}, \frac{3}{8}, \frac{5}{8}, \frac{7}{8}\}$ in the $\xi$-direction and $\{0.25, 0.75\}$ in the $\eta$-direction. We do not refine the mesh in $\zeta$-direction. This results in mesh 2 in \Cref{Fig2:shericalShellMesh2}. 

The results is shown in \Cref{Tab2:sphericalShellComputedEigenfrequencies} where the exact eigenfrequencies are collected from \Cref{Tab2:sphericalShellFirstEigenValues}. As the spherical shell is not clamped, the first 6 modes (3 from translation and 3 from rotation) will correspond to eigenvalue equal zero. The first interesting mode is thus vibration mode 7, which corresponds to $\omega_{21}$. Up to rotation, there is 4 identical other modes (identical eigenvalues), such that the next mode is vibration mode 12 which then corresponds to $\omega_{31}$. The first four unique modes up to rotation is shown in \Cref{Fig2:EigenModesSphericalShell}. We note that the accuracy decreases for modes with higher frequencies.
\begin{table}
	\centering
	\caption[Convergence of computed eigenfrequencies for spherical shell]{\textbf{Spherical shell:} Convergence of computed eigenfrequencies.}
	\label{Tab2:sphericalShellComputedEigenfrequencies}
	\begin{tabular}{S S S S S S S}
		\toprule
		{$p$} & {$q$} & {$r$} & {$\omega_{21}$} & {$\omega_{31}$} & {$\omega_{41}$} & {$\omega_{51}$}\\
		\midrule
		2 & 2 & 2 & 777.802 & 1019.834 & 1379.161 & 2159.979\\	
		3 & 3 & 2 & 764.428 & 913.290 & 1000.350 & 1235.107\\	
		4 & 4 & 2 & 764.175 & 908.693 & 976.975 & 1038.282\\	
		5 & 5 & 2 & 764.123 & 908.041 & 972.766 & 1021.684\\	
		\multicolumn{3}{c}{exact} & 764.121 & 907.967 & 972.169 & 1017.829\\	
		\bottomrule
	\end{tabular}
\end{table}
\begin{figure}
	\centering        
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/sphericalShellMesh1}
		\caption{Mesh 1.}
		\label{Fig2:shericalShellMesh2_1}
	\end{subfigure}
	~ 
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/sphericalShellMesh2}
		\caption{Mesh 2.}
	\end{subfigure}
	\caption[Meshes of a spherical shell]{\textbf{Spherical shell:} The first two meshes with, respectively, 8 and 32 elements.}
	\label{Fig2:shericalShellMesh2}
	\par\bigskip	
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrSphericalShell7}
		\caption{Mode 7 corresponding to $\omega_{21}$.}
	\end{subfigure}
	~
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrSphericalShell12}
		\caption{Mode 12 corresponding to $\omega_{31}$.}
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrSphericalShell19}
		\caption{Mode 19 corresponding to $\omega_{41}$.}
	\end{subfigure}
	~
	\begin{subfigure}{0.47\textwidth}
		\centering   
		\includegraphics[width=0.7\textwidth]{../../graphics/vibrSphericalShell28}
		\caption{Mode 28 corresponding to $\omega_{51}$.}
	\end{subfigure}
	\caption[Vibration modes of spherical shell]{\textbf{Spherical shell}: First four unique (up to rotation) vibration modes using $p=5$, $q=5$ and $r=2$. The colors corresponds to displacement in the radial direction.}
	\label{Fig2:EigenModesSphericalShell}
\end{figure}
